TinySDR: Low-Power SDR Platform for Over-the-Air Programmable IoT Testbeds

Wireless protocol design for IoT networks is an active area of research which has seen significant interest and developments in recent years. The research community is however handicapped by the lack of a flexible, easily deployable platform for prototyping IoT endpoints that would allow for ground up protocol development and investigation of how such protocols perform at scale. We introduce tinySDR, the first software-defined radio platform tailored to the needs of power-constrained IoT endpoints. TinySDR provides a standalone, fully programmable low power software-defined radio solution that can be duty cycled for battery operation like a real IoT endpoint, and more importantly, can be programmed over the air to allow for large scale deployment. We present extensive evaluation of our platform showing it consumes as little as 30 uW of power in sleep mode, which is 10,000x lower than existing SDR platforms. We present two case studies by implementing LoRa and BLE beacons on the platform and achieve sensitivities of -126 dBm and -94 dBm respectively while consuming 11% and 3% of the FPGA resources. Finally, using tinySDR, we explore the research question of whether an IoT device can demodulate concurrent LoRa transmissions in real-time, within its power and computing constraints.

==> acks.tex <==
\vspace{-10px}
\section{Acknowledgments.}
\vskip -0.15in
\textred{We thank Haitham Hassanieh, Vikram Iyer, Vamsi Talla, Justin Chan, Anran Wang, Rajalakshmi Nandakumar, and the anonymous reviewers for their helpful feedback on the paper. This work was funded in part by NSF awards CNS-1812554, CNS-1452494, CNS-1823148, Google Faculty Research Awards and a Sloan Fellowship.}



==> app-1.tex <==
\section{Applications}
In this section, we 
\subsection{IoT Protocol: LoRa}

\subsubsection{Transmitter}

\subsubsection{Receiver}

\subsection{LoRa Spectrum Sensing}

\subsection{Localization}

==> concurrent-0.tex <==
\section{Research Case Study}
An SDR that is geared for IoT endpoints and can provide I/Q transmission and reception capability opens up opportunities for addressing multiple research questions in IoT networks.

In this section, we focus on the following question: Can a {\it low-power IoT endpoint} device decode multiple concurrent LoRa transmissions at the same time? LoRa supports long range communication for IoT devices and is gaining popularity as a low-power wide area networking (LPWAN) standard. While it supports long ranges, it is also challenging since the range of these devices can be a few kilometers. This increases the number of collisions and probability of concurrent transmissions in a large scale city-scale deployment. While recent work~\cite{lorasigcomm17,netscatter} has explored the feasibility of enabling concurrent LoRa transmissions, they have been targeted for decoding on a gateway USRP device.  In fact, most concurrent transmission techniques in our community~\cite{zigzag, anc, lorasigcomm17} have been prototyped on USRPs and it is unclear if a low-power IoT endpoint device can decode concurrent transmissions in real-time within its stringent 1) power constraints, 2) computational constraints and 3)  resource constraints. TinySDR enables us to explore such questions and design MAC protocols for decoding concurrent transmissions  on IoT endpoints. 

{\bf Using orthogonal LoRa codes.} Here we explore a specific way of enabling concurrent transmissions in LoRa: using orthogonal codes.  Specifically, to allow multiple LoRa nodes to communicate at the same time, we exploit LoRa's support for orthogonal transmissions~\cite{lora_basics} which can occupy the same frequency channel without interfering with each other. Two chirp symbols are orthogonal when they have a different chirp slope. For a chirp with spreading factor of $SF$ and bandwidth of $BW$, the chirp slope is the bandwidth occupation of the chirp over time: $\frac{BW^{2}}{2^{SF}}$~\cite{netscatter}.

{\bf Decoding concurrent transmissions on \name.} We explore if we can demodulate multiple concurrent LoRa transmissions in real-time on a \name\ platform and evaluate its power consumption, computational resources and delay. 

In order to receive concurrent LoRa transmissions, \name\ must be able to demodulate LoRa upchirp symbols with different slopes. So say we have two LoRa transmissions that use different spreading factor and bandwidth configurations: $SF_1, BW_1$ and $SF_2, BW_2$. To decode them concurrently, we implement decoders for each of the chirp configurations in parallel on our FPGA. Specifically, we first generate a corresponding downchirp symbol for each configuration. We then correlate the received signals in the frequency domain with each of the downchirp symbols using time domain multiplication with the received signal. After correlation, we take an FFT of the result and identify the maximum to decode the symbol values. Fig.~\ref{sdsd} shows the decoding pipeline we use.

{\bf Evaluation.} We evaluate three key aspects of our design: 1) the  platform's effectiveness in decoding concurrent transmissions across a range of RSSI values, 2) the power consumption at the endpoint device while decoding concurrent transmissions and 3) the computational resources required and the resulting delay in decoding. 

We use two SX 1276 LoRa transceivers as our transmitters and set them to transmit continuously at two different settings: they both use a spreading factor of $SF=8$ but have two different bandwidth setups, $BW_1=125 kHz$ and $BW_2=250 kHz$. The transmitters are set to transmit random chirp symbols and are connected to a power combiner  and we connect the combined output to the RF input of \name\ through a variable attenuator. The \name\ platform decodes these two concurrent transmissions and computes the chirp symbol error rate for each of these transmissions. We evaluate three main scenarios: 1) when the two transmitters have a similar power level at the receiver, 2) when the first transmitter has a power level XX~dB higher than the second and 3) when the first transmitter has a power level xXX~dB lower than the second.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/8_lora_orthogonal_rx/lora_multiple.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf LoRa Orthogonal Demodulator Evaluation.}}}
	\label{fig:lora_multiple_rx}
    \vskip -0.15in
\end{figure}

Fig.~\ref{fig:lora_multiple_rx}(a)-(c) plot the measured the chirp symbol error rate vs received power and plot the results in Fig.~\ref{fig:lora_multiple_rx}. The results can be summarized as follows:
\squishlist
\item  This plot shows our implementation on \name achieves a sensitivity of -123~dBm for $SF=8$ and $BW=125kHz$. This is expected because XXX explain the. Explain the two extra graphs we are adding
\item Our parallel implementation in Fig.~\ref{sdds} uses only 11\% of the FPGAs resources. Yet it is able to perform the functionality of decoding two concurrent transmissions while also allowing the flexibility for further optimization.  Further the delayXXX.
\item Power conusmption XXX and compare it to a single one. XXX
\squishend
% Can Semtech chips 
%same fft
%provides programmable parallel %demodulation for different LoRa configurations. Here, 


Note that Semtech gateway solutions such as SX1308~\cite{sx1308} can receive multiple transmissions like our design. However it is a gateway solution and to the best of our knowledge we are the first to show that concurrent LoRa transmissions can be decoded on a IoT endpoint, which would have been difficult without \name.


==> design-0.tex <==
\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}

\section{System Design}

We design \name platform to fulfill the vision of an SDR based IoT testbed. In particular, \name system has flexible PHY and MAC layer, is capable of updating over the air (OTA) and low power. In this section, we explain the design of the \name system and present design choices and considerations. As shown in fig.~\ref{fig:system}, the system is divided to six different functional blocks: i) SDR, ii) OTA update system, iii) Power Management Unit (PMU), iv) storage devices and v) sensor interface.

\subsection{SDR}
% - Which radio chip?
% - Large area network --> longer range --> higher power --> need PA, which PA?
% - What FPGA?
%   - Memory
%   - DSP blocks/features
%   - SD card
Software-Defined Radio is a programmable PHY layer which converts bits to radio signals and vice versa. At a high level, SDR uses programmable I/Q radio which transforms RF signals to I/Q samples and vice versa. This radio exchanges data with the FPGA for modulation and demodulation. Our SDR is composed of multiple blocks: i) I/Q Radio, ii) Power Amplifier, iii) FPGA and iv) Memory.

% Radio
% What are its blocks?
% sampling rate
% ADC/DAC number of bits
% spectrum support
% cost
% power

\noindent{\bf I/Q Radio.} Current SDR systems use I/Q radio chips that are designed to cover a multi-GHz spectrum and have high ADC/DAC sampling rates to support large bandwidth. For example, AD9361~\cite{ad9361} series which is used in USRP and ADPluto can transmit from xxx MHz to xxx GHz and supports sampling rates as high as tens of MHz. Supporting a wide frequency spectrum with a low receiver noise figure and being to able to operate at tens of megahertz sampling rate, makes these radios power hungry on the order of watts. Moreover, as shown in Table~\ref{table:Radios}, almost all these radio chips costs more than XXX\$. To support IoT testbed vision, we need to use a radio that supports at least 900~MHz and 2.4~GHz ISM bands and is low-power and low-cost to be deployable. To this end, we selected AT86RF215~\cite{at86rf215} radio chip among all the choices. As we can see in Table~\ref{table:Radios}, this chip is the only one supporting both 900~MHz and 2.4~GHz ISM bands, costs less than 10\$ and consumes less than xxxx watts. MAX2831 and SX1257 are the only competitors in terms of cost. MAX2831 supports only 2.4~GHz, consumes twice the current and needs separate ADC and DAC. SX1257 supports only 900~MHz, has less bandwidth and consumes more current in TX mode. AT86RF215 integrates all the necessary blocks including LNA, programmable receive gain and low pass filter and ADC on the RX chain and including DAC to programmable PA with a maximum power of 14~dBm on the TX side. It supports three frequency bands of 389.5-510~MHz, 779-1020~MHz and 2400-2483.5~MHz and has two RF ports - one for sub-GHz and the other for 2.4~GHz. This chip utilizes two PLLs for sub-GHz and 2.4~GHz transceivers. Both PLLs use a shared 26~MHz crystal as reference and they can synthesize any frequencies with 198~Hz step size. Moreover, it has 13 bit ADC and DAC supporting up to 4~Msps of sampling rate for I and Q and hence 4~MHz of bandwidth which is more than the bandwidth of common IoT protocols. The RF front-end has 3-5~dB noise figure which is even lower than the noise figure of the front-end used in Semtech LoRa chipset, SX1276. Receiver/transmitter chain consumes around 28~mA/62mA nearly 5x lower than the current consumption of radio chips used in other SDR platforms~\cite{}. The receiver chain passes signal through an LNA with noise figure of 4.5 and then downconverts the signal using a mixer that is controlled by frequency synthesizer (PLL). In addition, this radio supports various modulations such as MR-FSK, MR-OFDM, MR-O-QPSK and O-QPSK. This allows us to bypass the FPGA entirely and enable greater power savings when we use standard modulations supported by this radio.
% What is FPGA doing?
% Why this FPGA?
% Duty-cycling
% 

\begin{figure}[t]
    \centering
	\includegraphics[width=1\linewidth]{figs/block_diagram/system.eps}
	\caption{\footnotesize{\name system block diagram. \textcolor{red}{We will revise this diagram based on new system design explanation. XXX}}}
	\label{fig:system}
\end{figure}


\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Existing off-the-shelf I/Q radios.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|C{2.4cm}|C{2.2cm}|c|c|}
         \hline
         \cellcolor{lightgray}{\bf I/Q Radio} & \cellcolor{lightgray}{\bf Frequency (MHz)} & \cellcolor{lightgray}{\bf Power} & \cellcolor{lightgray}{\bf Cost (\$)}\\
         \hline
         AD9361~\cite{ad9361} & 70$\sim$6000 & XXX & 282\\
         \hline
         Lms7002m~\cite{lms7002m} & 10$\sim$3500 & XXX & 110\\ 
         \hline
         MAX2831~\cite{max2831} & 2400$\sim$2500 & XXX & 9\\ 
         \hline
         SX1257~\cite{sx1257} & 862$\sim$1020 & XXX & 7.5\\ 
         \hline
         {\bf AT86RF215~\cite{at86rf215}} & {\bf 389.5$\sim$510 \newline 779$\sim$1020 \newline 2400$\sim$2483} & {\bf XXX} & {\bf 5.5}\\ 
         \hline
    \end{tabular}
    }
    \label{tab:radios}
\end{table}

\noindent{\bf FPGA.} The baseband I/Q signal is exchanged between I/Q radio and FPGA. The radio baseband I/Q interface is Low Voltage Differential Signalling (LVDS).
We use LFE5U-25F~\cite{latticeLFE5U} FPGA from Lattice Semiconductor for baseband processing which supports LVDS and has 24~k logic units which is comparable to other common SDR platforms including XXX, XXX and XXX. We use a small package of this FPGA on our design to decrease the platform physical size. Compared to FPGAs used in other existing platform this FPGA provides higher number of LUTs for the same cost. We use a 32~MHz clock oscillator as the reference clock for the FPGA. When radio operates in transmit mode, we use this clock reference to generate a 64~MHz clock reference for I/Q serial interface. However, when the I/Q operates in receive mode, we turn off this clock oscillator since the I/Q interface provides an clock reference and we use this reference for DSP operations in FPGA. 


% Why PA?
% Output power
% bypass and sleep current 
% 
\noindent{\bf Power amplifier.} Our vision is to design an SDR which can be used for a long-range IoT node implementation. To be able to support long ranges, we need to support high power transmitter. AT86RF215 can transmit maximum power of 14~dBm which is less than the maximum power allowed by FCC in 900~MHz and 2.4~GHz. To this end, we use SE2435L~\cite{SE2435L} 900~MHz module which has 30~dBm PA for sub-GHz RF port. This module has LNA and power amplifier which can be bypassed if needed. This gives us flexibility in different operations. For example, in receive mode we can either pass the incoming signal through the LNA and then connect it to the I/Q radio or completely bypass the LNA and connect the signal directly. The bypass current consumption is around xxx uA and the sleep current of these two power amplifiers is xxx uA. Similarly, in transmit operation we can pass the signal through the PA and amplify the signal or turn off the PA and just pass the signal directly to the antenna. If the required output power is less than 14~dBm, we would bypass the PA to decrease power consumption. We use similar module, SKY66112~\cite{SKY66112}, which can output 27~dBm at 2.4~GHz band with similar capabilities.


\subsection{Over-the-Air (OTA) update system}
Our goal in this paper is to design an IoT platform that is deployable and scalable in a wide area. To achieve this vision, we need to think about how to update these platform's firmware in a large network over time without the need of a wired infrastructure. In this section, we explain our OTA update system where we can update each \name node wirelessly. 

\noindent{\bf OTA wireless protocol.}
% - What protocol? Make table of protocols
% - RF switch
% - Flash, What size is needed?
% - MAC protocol?
Supporting wide area requires a long-range wireless protocol for the OTA. We used LoRa protocol for two reasons. First, LoRa gives high sensitivity and in turn kilometer ranges and also support a wide range of data rates from from XXX to XXX.
% For example with 30~dBm output power, $SF = xxx$, $BW = xxx$ and a 2~dBi antenna, we can achieve xxx~kbps at xxxx~km. 
Moreover, LoRa is becoming more and more wide-spread specially in the US. Table~\ref{tab:OTA_protocols} compares different long-range protocols and their corresponding data-rates. We use SX1276 Semtech chipset~\cite{sx1276} to implement LoRa protocol. As shown in Fig.~\ref{fig:OTA_XXX}, MCU receives the baseband bits from the SX1276 which has compressed firmware bitstream for both FPGA and MCU. Then, it stores this data in the external flash memory.XXXXX

% \noindent{\bf OTA MAC.} In \xref{sec:OTA}, we show that the update takes about 1 minute to finish depending on the update rate and the update bitstream file size. Moreover, we provision only one whole network firmware update per day. So, to update all the devices' firmware, each device goes to update mode at a certain time during the day. \textcolor{red}{explain the update MAC more}XXXX

%VI: moving to implementation section
%\noindent{\bf OTA MAC Design.} We design a MAC layer system for Lora protocol to update \name nodes in testbed network. Since we can update each node in a short time, XXXs as shown in Fig.~\ref{XXX}, we update each node separately. First, we send an update request including device ID in a LoRa packet from our access point (AP). Then, we the \name node process this packet, switches to update mode and send a ready message to access point. Then, the AP sends firmware updates with multiple LoRa packets and handles packet failures using acknowledge messages from the \name node. After PA sends all firmware data, it send another message representing end of firmware update. Finally, the \name node switch its state to normal operation.

\noindent{\bf Flash Memory.} We store the firmware update bitstream in an external flash memory. FPGA programming bitstream for our FPGA on \name has a size of 572~KB and MCU is XXX~KB. In our platform, we use 2~MB flash memory to be able to store multiple bitstreams for FPGA and MCU at the same time.

\subsection{Controller}
% - What needs to be controlled?
% - Which MCU?
% - Power management
Controller is the central brain of the system and is implemented on a low-power MCU. The MCU needs to have low sleep current, able to support multiple control interfaces, requires enough memory resources to support IoT MAC protocols and also able to run decompression algorithm. We used MSP432P401R~\cite{msp432P401R} a 32-Bit Cortex M4F MCU which has less than 1~uA sleep current, includes 64~KB SRAM and 256~KB flash memory. MCU controls I/Q radio parameters, backbone radio parameters, power amplifiers, RF switches, all the regulators and FPGA programming. By controlling the regulators, it does power-gating of different voltage domains and hence puts components supported by these domain to sleep or wakes them up. The sleep process which is controlled by the MCU is the following, it sets the timer, puts all the regulators to shut-down mode and then it goes to low power mode consuming only 550~nA.


% with floating point unit to control two I/Q and backbone transceiver, communicate with baseband processor and managing power on the platform. This MCU has 64~kB RAM along with 256~kB FLASH memory for programming and provides huge flexibility for performing compression algorithms, complex MAC layer implementation of IoT protocols and sensor reading applications. It supports up to eight SPI, four UART and four I2C interfaces. It can operate at low frequencies, such as 128~kHz, as well as high frequencies up to 48~MHz. It has two 32-bits timers and more importantly it supports different low-power modes. As an example, it supports LPM4.5 mode which only consumes 25~nA current. These features make this MCU a suitable choice for \name to operate at low-power and also perfomr accurate duty-cycling.


% The MAC layer controls channel access between different transceivers on the medium. In \name design, it is implemented on an MCU. Note that, since \name is designed for IoT protocols testing and implementation, it has relaxed latency requirements. This means there is no stringent timing requirement on the communication link between the PHY and MAC layer. MCU is the central controller of the system and in addition to hosting the MAC layer it controls sensor interfaces, OTA update process and all necessary functions to increase the battery life-time including duty-cycling and power-gating of different blocks.


\subsection{Power Management Unit}
In this section, we present the design of power management unit working with 4V xxxx battery with the goal of decreasing power consumption. Specifically, to be able to support long battery life we need to be able to duty-cycle and power-gate the the system. In addition, different components in the system have different supply voltage requirements. To minimize the power, we need to provide components with the lowest voltage possible. This means that to minimize power we need to support similar voltage components with the voltage domain supported by the same voltage regulator. Additionally, voltage of some of the components needs to be changed over time to get the desired performances like power efficiency. So, ideally we would want have separate controllable voltage regulator for each major power consuming component in the system. However, having many different voltage regulators and being able to control them increases the number of devices and in turn \name price significantly. Moreover, control signals routing and having different power planes on the PCB to support these voltage domains makes the PCB design exponentially complicated. Therefore, trade-off exists between the number of voltage domains and price and complexity of the design. Table~\ref{tab:voltages} shows the supply voltages needed for each component and the voltage domain supporting it. 

% Other than V1 which supplies the MCU, other voltage regulators would go to shut-down and wake-up. This means that V1 needs to have low quiesant current and others needs
\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Voltage domains in \name.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|C{2.4cm}|C{3cm}|c|}
         \hline
         \cellcolor{lightgray}{\bf Component} & \cellcolor{lightgray}{\bf Voltage (V)} & \cellcolor{lightgray}{\bf Voltage Domain}\\
         \hline
         MCU & 1.8 & V1\\
         \hline
         FPGA & 1.1, 1.8, 2.5, 1.8< V5 <3.6 & V2, V3, V4, V5\\
         \hline
         I/Q Radio & 1.8< V5 <3.6 & V5\\
         \hline
         Backbone Radio & 1.8< V5 <3.6 & V5\\
         \hline
         sub-GHz PA & 3.5 & V6\\
         \hline
         2.4~GHz PA & 1.8, 3.0 & V3, V7\\
         \hline
         FLASH Memory & 1.8 & V3\\
         \hline
         Micro SD Memory& 3.0 & V7\\
         \hline
    \end{tabular}
    }
    \vskip -0.2 in
    \label{tab:voltages}
\end{table}


\noindent{\bf Voltage domain V1.} We use linear regulator for V1 which supports MCU. Since MCU is the central controller, it needs to be powered at all times. Therefore, it is powered by a separate voltage domain. Moreover, to decrease the sleep current we need to use a voltage regulator that has low quiescent current. Although switching voltage regulator has higher voltage conversion efficiency when it is active, its high quiescent current prevents it from being used for V1. Considering a wake-up power consumption of 100~mW XXX and duty-cycles as high as 1000x, the sleep power consumption should be much lower than $\frac{100mW}{1000} = 100uW$ or $\frac{100uW}{5} = 20uW$. Having a battery voltage of 4V results in less than 5uA sleep current. We use XXX which is a linear regulator and has only XXX uA quiescent current.

\noindent{\bf Voltage domain V2.} This voltage domain supports FPGA core voltage which needs constant voltage of 1.1~V. Since the voltage difference between the battery voltage and this domain's voltage is high, we need to use switching voltage regulator to achieve high efficiency. Since we are using SRAM-based FPGA, it has high core and I/O leakage current. Therefore, in order to decrease sleep current, this voltage domain needs to be shut-down during sleep. This means that the regulator needs to have low shut-down current of less than 1~uA. We use TPS62240~\cite{TPS62240} to support this domain since it has high voltage conversion efficiency and low shut-down current.

\noindent{\bf Voltage domain V3, V4 and V7.} We need 1.8~V voltage supply for I/O banks and programming of the FPGA, digital supply of the 2.4~GHz PA and Flash memory and is provided by V3 voltage domain. In addition, FPGA I/O banks need a supply voltage of 2.5~V other than their main I/O supply voltage. V4 provides this supply voltage. Voltage regulators for these domains should have low shut-down current during sleep and high efficiency. We use 3~V voltage supply to power microSD card and analog supply of the 2.4~GHz PA. The voltage regulator for this domain needs to support currents as high as 120~mA for the 2.4~GHz PA in addition to having low shut-down current and high efficiency. Similar to V2, we use three TPS62240 switching voltage regulators for V3, V4 and V7 because of its low shut-down current, high efficiency and being able to provide as high as 300~mA current.

\noindent{\bf Voltage domain V5.} V5 is a shared voltage domain for I/Q radio, backbone LoRa radio and FPGA I/O bank connected to LVDS interface of the I/Q radio. This voltage domain is initially set to 1.8V to decrease the power consumption. If the output of the I/Q radio needs to increase, we would need to increase this voltage. Therefore, we need controllable voltage regulator for this voltage domain besides having high efficiency and low shut-down current. To this end, we use Semtech SC195ULTRT~\cite{SC195ULTRT} which provides a range from 1.8~V to 3.6~V.

\noindent{\bf Voltage domain V6.} This voltage domain supplies the 900~MHz PA. This PA consumes as high as 550~mA current when transmitting 30~dBm. Therefore, the voltage regulator for this domain needs to be able to supply this current while having high efficiency and low shut-down current. We use TPS62080~\cite{TPS62080} which is able to provide 1.2A while satisfying the other two requirements. Note that, since this PA can consumes as much as 2~W, we carefully design ground and power plane on PCB to support enough current and also avoid heating issues on the \name board.



% \subsection{System Implementation}
% \subsubsection{RF front end}
% - Radio architecture
% - Radio options/features and how to use them

% \subsubsection{Reading samples}
% - LVDS
%   - Explain differential signals
%   - Explain RX (serial, clk, etc)
%   - Explain TX
%   - PCB design concerns
  
% - Memory/buffer
%   - Explain interface to memory blocks
%   - Size
%   - Speed
  
% - DSP
%   - FFT
%   - Filters etc
  
% \subsubsection{Backbone}
% - Use LoRa
% - Compression, which algorithm and why?
% - Programming
%   - Flash interface
%   - FPGA modes
%   - Programming steps with flow diagram
%   - Multiple bitstreams





==> design-1.tex <==
\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}

\section{\name\ Platform}
Our IoT platform has low-power, supports a few MHz of bandwidth, achieves microsecond latency and includes over-the-air update of the wireless protocol it can run on its FPGA. Here, we first describe the different components in our hardware. We then present the interfaces between the different hardware components. Finally, we describe the over-the-air update protocol including the compression and decompression algorithm as well as over-the-air FPGA programming. 
\subsection{Hardware Design}
Building a platform that satisfies the above requirements needs a number of careful design considerations. Specifically, we seek to minimize power consumption and cost while still offering the flexibility of an SDR which can read and process raw samples. Here, we outline the system architecture along with a detailed analysis of our design decisions.

\subsubsection{Designing the Software Radio}
The core block on our platform is the software-defined radio, a programmable PHY layer that processes and converts bits to radio signals and vice versa. We begin by explaining our choices for the primary components of an SDR which are a radio chip that provides an interface for sending and receiving raw samples of an RF signal as well as an FPGA that can process these signals in real time. We then discuss the supporting peripherals for these devices such as a power amplifier (PA) to boost the output of the radio chip and non-volatile memory for the FPGA to read and write data from.


{\bf Choosing a Radio Chip.} 
We begin by choosing a radio chip as its specs define the requirements for the FPGA and other blocks. Our primary requirement is that the chip supports reading and writing raw complex I/Q samples of the RF signal. Current SDR systems use I/Q radio chips that are designed to cover a multi-GHz spectrum and have high ADC/DAC sampling rates to support large bandwidth. For example, AD93XX~\cite{XXX} series which is used in USRP and ADPluto can transmit from xxx MHz to xxx GHz and supports sampling rates as high as tens of MHz. Each of these spec, wide bandwidth, low noise figure, and high sampling rate represent fundamental trade offs of power for performance, and therefore consume watts of power. Moreover, almost all these radio chips costs more than \$XX. 

We instead take a different approach when designing \name: identify the minimum required specs and find a radio that supports them. Specifically, an IoT platform must be able to operate in at least the 900~MHz and 2.4~GHz ISM bands, have at least XX~MHz of bandwidth, while otherwise minimizing power and ideally costing less than \$10. We analyze all of the commercially available radio chips that provide these capabilities and list them in Table~\ref{table:Radios}. As shown, only the AT86RF215 supports all of our requirements. In addition to lower cost and support for both frequency bands, it also consumes less power than the MAX2831 and the SX1257. Moreover, the AT86RF215 integrates all the necessary blocks including LNA, programmable receive gain and low pass filter, ADC on the RX chain, as well as a DAC and programmable PA with a maximum power of 14~dBm on the TX side. This chip supports three frequency bands of 389.5-510~MHz, 779-1020~MHz and 2400-2483.5~MHz which includes major ISM bands and provides 4~MHz of bandwidth which meets our IoT protocol requirements.

Next, we evaluate its noise figure to determine whether it compromises performance to achieve these specs. For comparison, the RF front-end has 3-5~dB noise figure which is even better than the noise figure of the front-end used in Semtech SX1276 LoRa chipset, suggesting it should be able to achieve long range performance. At the same time it consumes 5x less power than the radios used on other SDRs~\cite{XXX} and has built in support for standard modulations such as MR-FSK, MR-OFDM, MR-O-QPSK and O-QPSK that can save FPGA resources or power by bypassing the FPGA entirely.

%The receiver chain passes signal through an LNA with noise figure of 4.5 and then downconverts the signal using a mixer that is controlled by frequency synthesizer (PLL).
\begin{figure}[t]
    \centering
	\includegraphics[width=1\linewidth]{figs/block_diagram/system.eps}
	\caption{\footnotesize{\name system block diagram.}}
	\label{fig:system}
\end{figure}


\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Existing off-the-shelf I/Q radios.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|C{2.4cm}|C{2.2cm}|c|c|}
         \hline
         \cellcolor{lightgray}{\bf I/Q Radio} & \cellcolor{lightgray}{\bf Frequency (MHz)} & \cellcolor{lightgray}{\bf Power} & \cellcolor{lightgray}{\bf Cost (\$)}\\
         \hline
         AD9361~\cite{ad9361} & 70$\sim$6000 & XXX & 282\\
         \hline
         LMS7002M~\cite{lms7002m} & 10$\sim$3500 & XXX & 110\\ 
         \hline
         MAX2831~\cite{max2831} & 2400$\sim$2500 & XXX & 9\\ 
         \hline
         SX1257~\cite{sx1257} & 862$\sim$1020 & XXX & 7.5\\ 
         \hline
         {\bf AT86RF215~\cite{at86rf215}} & {\bf 389.5$\sim$510 \newline 779$\sim$1020 \newline 2400$\sim$2483} & {\bf XXX} & {\bf 5.5}\\ 
         \hline
    \end{tabular}
    }
    \vskip -0.15in
    \label{tab:radios}
\end{table}

{\bf Picking an FPGA.} Now that we have chosen a radio chip, the next step in our design process is to find an FPGA that can interface with it. Aside from minimizing power, we would also like to maintain a small form factor, and so we also consider the physical package size of the FPGA. We use LFE5U-25F~\cite{latticeLFE5U} FPGA from Lattice Semiconductor for baseband processing which has 24~k logic units. This chip provides a greater number of LUTs than other SDR platforms such as the XXX and XXX but at lower cost. We also choose a small package of this FPGA to decrease the platform's size.

% Maybe add a comparison of the Microsemi FPGA you used on V1?

{\bf Adding a power amplifier.} AT86RF215 only supports a maximum transmit power of 14~dBm that is traditionally used by IoT radios but which is less than the 30~dBm allowed by the FCC for transmissions in ISM bands. To provide flexibility, we add a PA to maximize range within FCC constraints. Considering the high cost and power requirements of wide-band PAs that could operate at both 900~MHz and 2.4~GHz we instead select two different chips: the SE2435L~\cite{SE2435L} for 900~MHz and SKY66112~\cite{SKY66112} for 2.4~GHz. Our 900~MHz PA supports up to 30~dBm output power, and the 2.4~GHz PA can output up to 27~dBm. Both chips also include an LNA for receive mode and include a built in circuit to bypassing either of these components for maximum flexibility and power savings. For example, in receive mode we can either pass the incoming signal through the LNA and then connect it to the I/Q radio or completely bypass the LNA and connect the signal directly. The bypass current consumption is a negligible xxx uA and the sleep current of both two power amplifiers is xxx uA. Similarly, in transmit operation we can pass the signal through the PA and amplify the signal or turn off the PA and just pass the signal directly to the antenna if we need to transmit less than 14~dBm.


\subsubsection{Designing hardware for Over-the-Air (OTA) update system.}
Designing a wireless IoT platform that is useful for research and performing experiments presents a practical issue: how can we send firmware updates to these nodes with new IoT protocols to run? While all of the discussion above enables a small, low power, low cost SDR for easy deployment, FPGAs and microcontrollers typically require a wired interface for reprogramming. To make a large scale network practical we develop an OTA update system to reconfigure and program \name nodes wirelessly. 

{\bf OTA wireless chipset.} A key question when designing an OTA update system is, what wireless protocol should be used? Considering our goal is to support wide area networking, we focus on protocols designed for long range operation. We analyze all of the available long range protocols and select LoRa for our OTA system for a number of reasons. First, LoRa receivers have a high sensitivity which enables kilometer ranges. LoRa also support a wide range of data rates from XXX to XXX which allows us to trade off rate for range depending on the deployment scenario. Moreover, LoRa is becoming more and more wide-spread in the US. We use the SX1276 Semtech chipset~\cite{sx1276} which is available for only \$XX, minimizing the cost overhead.


% For example with 30~dBm output power, $SF = xxx$, $BW = xxx$ and a 2~dBi antenna, we can achieve xxx~kbps at xxxx~km. 
% \noindent{\bf OTA MAC.} In \xref{sec:OTA}, we show that the update takes about 1 minute to finish depending on the update rate and the update bitstream file size. Moreover, we provision only one whole network firmware update per day. So, to update all the devices' firmware, each device goes to update mode at a certain time during the day. \textcolor{red}{explain the update MAC more}XXXX

{\bf Flash Memory.} While our FPGA achieves good performance at low power, size and cost, it is SRAM based and does not include onboard non-volatile memory for storing programming data. We instead store the firmware bitstream on a separate flash memory chip. The FPGA programming bitstream is 572~KB and the MCU programs require up to XXX~KB. When choosing a flash chip we select the XXX which has 2~MB of memory. Although this is far more than the minimum size required, it allows for \name to store multiple bitstreams and MCU programs to quickly switch between stored protocols or configurations without re-sending the programming data over the air.

\subsubsection{Picking the microcontroller}
So far we explained how to assemble a highly flexible and low power SDR design with wireless update capabilities. To control all of these individual chips and toggle all of these power saving options, we use a low-power microcontroller (MCU). 

What are the requirements for our MCU? In addition to having a low sleep current it must be able to support multiple control interfaces, requires enough memory resources to support IoT MAC protocols and also able to run a  decompression algorithm for our OTA system. We select the MSP432P401R~\cite{msp432P401R} a 32-Bit Cortex M4F MCU which meets all of our requirements with its less than 1~uA sleep current, and 64~KB of onboard SRAM and 256~KB of onboard flash memory.  In addition to controlling the I/Q radio parameters and backbone radio parameters, and reprogramming of the FPGA, the MCU performs the important function of power management. It is responsible or toggling on and off the power amplifiers, as well as performing power-gating by turning ON and OFF different voltage regulators to turn various components in our system ON or OFF. 

%The sleep process which is controlled by the MCU is the following, it sets the timer, puts all the regulators to shut-down mode and then it goes to low power mode consuming only 550~nA.


% with floating point unit to control two I/Q and backbone transceiver, communicate with baseband processor and managing power on the platform. This MCU has 64~kB RAM along with 256~kB FLASH memory for programming and provides huge flexibility for performing compression algorithms, complex MAC layer implementation of IoT protocols and sensor reading applications. It supports up to eight SPI, four UART and four I2C interfaces. It can operate at low frequencies, such as 128~kHz, as well as high frequencies up to 48~MHz. It has two 32-bits timers and more importantly it supports different low-power modes. As an example, it supports LPM4.5 mode which only consumes 25~nA current. These features make this MCU a suitable choice for \name to operate at low-power and also perfomr accurate duty-cycling.


% The MAC layer controls channel access between different transceivers on the medium. In \name design, it is implemented on an MCU. Note that, since \name is designed for IoT protocols testing and implementation, it has relaxed latency requirements. This means there is no stringent timing requirement on the communication link between the PHY and MAC layer. MCU is the central controller of the system and in addition to hosting the MAC layer it controls sensor interfaces, OTA update process and all necessary functions to increase the battery life-time including duty-cycling and power-gating of different blocks.


% Should this part move to a different section?
\subsubsection{Designing the Power Management Unit}
Next, we present the design of our power management unit which seeks to maximize the system lifetime when running off of a 3.7~V Lithium battery. To enable long battery lifetimes we need to be able to duty-cycle our system and toggle each of the above blocks ON and OFF when they are not used. Further, different components have different supply voltage requirements and we wish to provide each one with the lowest voltage possible to minimize power usage. 

Ideally we would want separate controllable voltage regulator for each major power consuming component in the system. However, having many different voltage regulators and being able to control all of them significantly increases the complexity and number of components which in turn increases price. Moreover, it complicates the PCB design requiring many control signals to be routed and a multitude of power planes. Therefore, there exists a trade-off between the granularity of power control and the price/complexity of a design. To better understand the needs of our system, we outline the supply voltages needed for each component and the voltage domain supporting it in Table~\ref{tab:voltages}. We describe each of these voltage domains and how we group components to balance power optimization with complexity below. 

% Other than V1 which supplies the MCU, other voltage regulators would go to shut-down and wake-up. This means that V1 needs to have low quiesant current and others needs
\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Voltage domains in \name.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|c|c|c|}
         \hline
         Component & Voltage [V] & Voltage Domain\\
         \hline
         MCU & 1.8V & V1\\
         \hline
         FPGA & 1.1, 1.8, 2.5, Vlvds & V2, V3, V4, V5\\
         \hline
         I/Q Radio & 1.8< V5 <3.6 & V5\\
         \hline
         Backbone Radio & 1.8< V5 <3.6 & V5\\
         \hline
         sub-GHz PA & 3.5V & V6\\
         \hline
         2.4~GHz PA & 1.8, 3.0 & V3, V7\\
         \hline
         FLASH Memory & 1.8 & V3\\
         \hline
         Micro SD Memory& 3.0 & V7\\
         \hline
    \end{tabular}
    }
    \vskip -0.2 in
    \label{tab:voltages}
\end{table}


{\bf Voltage domain V1 (MCU).} Since MCU is the central controller which implements power management, it needs to be powered at all times and therefore has its own voltage domain. Moreover, to decrease the sleep current we need to use a voltage regulator with a low quiescent current. Although switching voltage regulator designs have higher conversion efficiency when active, they also have high quiescent currents. So we instead use  a linear regulator. When choosing these components we want to make sure this regulator and the microcontroller sleep power do not dominate the sleep power of the whole systemt. Since our system consumes around 100~mW when active and duty-cycling of IoT devices can be as much as 1000x, our sleep power consumption should be much lower than $\frac{100mW}{1000} = 100uW$; we target $20uW$. Having a battery voltage of 3.7 V results in around 5uA sleep current. We therefore choose the XXX which is a linear regulator with a quiescent current of XXX uA.

{\bf Voltage domain V2.} This voltage domain supports the FPGA core voltage which needs to be a constant 1.1~V. Since the voltage difference between the battery voltage and this domain's voltage is high and the FPGA can be power gated when not in use, we use a switching voltage regulator to achieve high efficiency. Because our FPGA is SRAM-based, it has a relatively high core and I/O leakage current, therefore wasting power even in sleep mode. In order to decrease the overall sleep power of our system, we shut down this voltage domain during sleep. This means that the regulator needs to have low shut-down current of less than 1~uA. We use TPS62240~\cite{TPS62240} here since it has high voltage conversion efficiency and low shut-down current.

{\bf Voltage domains V3, V4 and V7.} We need a 1.8~V supply for the I/O banks and programming of the FPGA, the digital supply of the 2.4~GHz PA and flash memory which are all provided by V3 voltage domain. In addition, the FPGA I/O banks need a supply voltage of 2.5~V given by V4 in addition to V3. Considering these components will all be turned off when not operating the voltage regulators for these domains should have low shut-down current during sleep and high efficiency. Additionally, we need a 3~V voltage supply provided by V7 to power the microSD card and analog supply of the 2.4~GHz PA. The voltage regulator for V7 has the additional requirement of supporting currents as high as 120~mA when the 2.4~GHz PA is active. Similar to V2, we use three TPS62240 switching voltage regulators which can be set to output each of the required voltages for V3, V4 and V7 because of its low shut-down current, high efficiency and ability to provide up to 300~mA of current.

{\bf Voltage domain V5.} V5 is a shared voltage domain for I/Q radio, backbone LoRa radio and FPGA I/O bank connected to the I/Q radio. This voltage domain is initially set to 1.8V to minimize power consumption, however components such as the radio chips can require higher voltage to achieve maximum power output. Therefore, in addition to high efficiency and low shut-down current as with the others, this domain should be programmable as well. To this end, we use Semtech SC195ULTRT~\cite{SC195ULTRT} which provides an adjustable output that can be set from 1.8~V to 3.6~V.

{\bf Voltage domain V6.} This voltage domain supplies the 900~MHz PA. This PA consumes as much as 550~mA current when transmitting at 30~dBm.  We use TPS62080~\cite{TPS62080} which is able to provide 1.2A. Note that,  we carefully design the ground and power plane on PCB to support enough current while minimizing heat dissipation issues. We also note that in normal operations the PA is turned off since IoT protocols do not such high transmit powers.



==> discussion-0.tex <==
\section{Conclusion and Discussion}
This paper presents the first SDR  platform specifically tailored to the needs of  IoT endpoints that can be used for large scale IoT network deployments. The goal of \name  is to provide a platform that can catalyze research  in  IoT networks. 

{\bf Research on PHY/MAC protocols.} \Name  presents an opportunity for researchers to avoid the time consuming endeavor of building their own custom IoT evaluation platforms and instead focus on PHY/MAC protocol innovations for the unique challenges of IoT networks. These include the fact that protocols trade-off data rate for range resulting in long packets during which channels may change significantly. What is the trade-off between packet length and overall throughput? Are there benefits of rate adaptation? We could also explore other questions like whether we can develop systems that support concurrent transmissions or creating multi-hop IoT PHY/MAC innovations, which have not been explored well given the lack of a flexible platform.

{\bf Research on IoT localization.} \Name could also be used to build localization systems as it gives access to the raw signals and therefore phase information across 2.4~GHz and 900~MHz bands, which forms the basis for many localization algorithms. In addition to exploring novel techniques such as distributed localization solutions where we could combine the phase information across a distributed set of sensors to create a large MIMO sensing system, \name presents an opportunity to evaluate and verify existing techniques on a common platform and understand how they would perform within the power and computation constraints of an IoT device.

{\bf Machine learning on IoT devices.} The FPGA on \name  opens up exciting opportunities for exploring machine learning algorithms on-board. This would allow researchers to explore trade-offs between the power overhead of running an on-board classifier versus repeatedly turning on the radio to send data to the cloud. This could also enable use of high bandwidth sensors such as cameras and microphones in which the time and therefore power bottleneck may be communication rather than sensing, as well as the ability to immediately act on sensor data during network outages for example to sound a local alert or alarm.

In addition to IoT research opportunities, below we outline ways in which we can improve our platform.

{\bf Improving OTA programming.}
Currently, \name  uses a simple MAC protocol for programming with a focus on using minimal system resources to allow for other custom software. However sequentially updating each node, could present significant overhead for systems with >100 nodes. Potential research directions involve exploring modified MAC protocols to reduce this time by exploiting the wireless broadcast nature, as well as a distributed update system in which nodes could help propagate update packets through the network.

% Based on Anran's feedback
{\bf Programming interface.}
TinySDR currently requires users to write Verilog or VHDL to program the FPGA and C code for programming the microcontroller. Future versions can incorporate a pipeline to use high level synthesis tools or integration with GNUradio for easy prototyping.

==> eval-1.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Single Tone Transmitter Power Consumption.} We show the total power consumption of \name in single transmitter mode at different output power.}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}


\section{Benchmarks and Evaluation}\label{eval}
% - power consumption in different modes, tx(single tone) rx(record raw IQ)
% - power in sleep mode
% - duty cycle system, wake-up time and power consumption
% - size on fpga for rx(raw IQ) and tx(single tone)
% - 
In this section, we characterize \name platform while it is running different operations. 
% We use two basic operations to evaluate receiver and transmitter capabilities of our platform. Following, we first describe scenarios that we used to evaluate our platform and then we show the results for different evaluations.

\begin{figure}[t]
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/rx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{{\bf I/Q Receiver.}}}
        \label{fig:rx_block}
    \end{subfigure}
	\begin{subfigure}{\linewidth}
	    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/tx_block.eps}
        \caption{\footnotesize{{\bf Single Tone Transmitter.}}}
        \label{fig:tx_block}
    \end{subfigure}
    \vskip -0.15in
    \caption{\footnotesize{{\bf FPGA Block Diagrams.} XXX}}
    \label{fig:fpga_blocks}
\end{figure}

\subsection{Single Tone Transmitter}
One of the basic operations of an SDR platform is transmitting a single tone wave. We program the radio front-end to transmit I/Q samples. Then, we use FPGA architecture, shown in Fig.~\ref{fig:tx_block} block diagram, to generate single tone wave and interface with radio front-end. This block diagram includes the basic architecture for any transmitting operation on \name platform. This block diagram includes a PLL module, clock divider, modulator, IQ Serializer and two LVDS modules. We use PLL to convert 50~MHz clock oscillator to 64~MHz clock that is required to interface with radio front-end serial interface. We divide this 64~MHz clock to 4~MHz clock that is the maximum sampling rate of the radio. Then we use this clock frequency to generate I/Q samples in signal modulator which in this example is a single tone modulator. We design an I/Q serializer module to convert parallel samples to serial. Then we connect serial output alongside the 64~MHz serial clock to LVDS modules to interface with radio font-end.

We set our radio to operate at following settings; Sampling rate of 4~MHz, power amplifier (PA) DC voltage of $2.4V$. We sweep the power output of the radio by changing PA index power and record the total power consumption of our platform. Fig.~\ref{fig:bench_tx_power} shows the power consumption of \name operating at 900~MHz and 2.4~GHz ISM bands. This plot shows XXXX.

In addition, we evaluate the area size of the single tone transmitter design on FPGA to show XXX.


\subsection{I/Q Receiver}
Next, we evaluate our platform in receive mode. To do this, we design a simple I/Q receiver on FPGA which receives I/Q samples from radio front-end and stores them in FPGA memory. Fig.~\ref{fig:rx_block} shows the FPGA block diagram of I/Q receiver. We design an I/Q deserializers that receives serial data from LVDS modules and converts to parallel I/Q samples. Then, deserializer module interface with SRAM memory to store I/Q samples. This is a universal design in our platform which provides I/Q samples to other FPGA blocks such as LoRa demodulator.

% To evaluate \name in receive mode, we program the radio front-end to receive I/Q samples. Then, we program the FPGA to interface with radio front-end using our deserializer FPGA block and converts I/Q serial samples to parallel data. Then we store these samples in FPGA internal memory.


\subsection{Clock Synchronization}

\subsection{Frequency Hopping}























==> eval-2.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Single Tone Transmitter Power Consumption.} We show the total power consumption of \name in single transmitter mode at different output power. Note: this figure will be updated! XXXX}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}

\section{Evaluation}
% In this section, we evaluated our \name platform to show that it is meeting the requirements of an IoT node.
\subsection{LoRa}
% talk about the LoRa modulation to show its complication
% we send and received the signal with the same sensitivity
To show the capability of the sub-GHz radio front-end in \name, we implemented LoRa modulator and demodulator on FPGA on our platform. Here, we explain the block diagram for modulator and demodulator that we implement on FPGA.

\noindent {\bf LoRa Modulator.} Fig.~\ref{fig:lora_tx_block} shows the block diagram of our LoRa modulator. We implement this modulator chain in Verilog HDL programming. Modulator starts with determining LoRa configurations such as $Spreading Factor$ and $Bandwidth$ and symbols values in Packet Generator unit. Then, the Chirp Generator unit uses these information to generate each chirp symbol. It uses a phase accumulator along with two lookup tables for $Sin$ and $Cosin$ functions to generate I/Q samples. We feed I/Q samples to IQ Serializer to generate serial stream information compatible with radio front-end interface. Finally, serial I/Q samples along with TX clock go to two LVDS interface that is connected to radio front-end.

\noindent {\bf LoRa Demodulator.} Fig.~\ref{fig:lora_rx_block} shows the block diagram of our LoRa demodulator. Demodulator interfaces with radio fornt-end through two LVDS connection; one for I/Q serial data and the other for synchronization clock. We implement an IQ Deserializer to convert serial I/Q data to parallel I/Q for further signal processing. Then, we run these data through a low-pass FIR filter. We use a memory in FPGA to buffer raw samples between the front-end and our demodulator. We use the Chirp Generator that we implemen for LoRa modulator to generate a baseline upchirp/downchirp symbol and then we multiply that with the received chirp symbol using Chirp Multiplier unit. Then, we use FFT core implementation provide by Lattice to perform FFT operation on multiplied signal and then detect symbol value and symbol type (upchirp or downchirp) using our Symbol Detector implementation.


\subsection{Zigbee De/Modulator}
\subsection{Power Consumption}
We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 

While Table~\ref{power} shows the power consumption of the receiver, the transmitter power is highly dependent on the output level of the radio and presents a trade-off versus range: high transmit power enables longer range  but requires additional power. To understand this relationship we use an xxx spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and again use an xxx mulitmeter to measure the DC power required. Fig~\ref{fig:bench_tx_power} shows the results. We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the external power amplifier (PA).
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
         \hline
         Mode & Power (mW) \\
         \hline
         LoRa TX & xxx\\ 
         \hline
         LoRa RX & xxx\\
         \hline
         Zigbee TX & xxx\\
         \hline
         Zigbee RX & xxx\\
         \hline
         OTA programming & xxx \\
         \hline
         OTA sleep & xxx \\
         \hline
         All components in sleep mode & xxx \\ 
         \hline
    \end{tabular}
    \caption{\footnotesize{\bf Power consumption of our SDR platform while performing different operations.}}
    \label{tab:power}
\end{table}

\subsection{Duty-cycling}
Considering many IoT nodes often perform short, simple tasks they are typically duty cycled to allow for further power savings. In \name, the microcontroller has the functionality to disable power consuming components such as the radio and FPGA and enter a low power sleep mode. Table~\ref{tab:wakeup} shows both the time required to wake up from sleep mode as well as the average power consumed by the device running at an xx\% duty cycle.
\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|}
         \hline
         Mode & Wake-up time (ms) & Average power (mW) \\
         \hline
         FPGA TX & xxx & xxx\\ 
         \hline
         MCU TX & xxx & xxx\\
         \hline
         Radio TX & xxx & xxx\\ 
         \hline
         \textbf{Total TX} & \textbf{xxx} & \textbf{xxx}\\ 
         \hline
         FPGA RX & xxx & xxx\\ 
         \hline
         MCU RX & xxx & xxx\\
         \hline
         Radio RX & xxx & xxx\\ 
         \hline
         \textbf{Total RX} & \textbf{xxx} & \textbf{xxx}\\ 
         \hline
    \end{tabular}
    \caption{\footnotesize{\bf Wake-up times for each component of our SDR platform.}}
    \label{tab:wakeup}
\end{table}

To further demonstrate the capabilities of \name, we also evaluate it in a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. Fig.~\ref{fig:wakeup_curve} shows the results for this process, and the average power is xx. This means that \name can achieve a battery life of xx using an xx battery.


\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Modulator Evaluation.} We evaluate our LoRa modulator in comparision with Semtech SX1276 LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}

\subsection{Protocols}
To evaluate the use of \name as an IoT endpoint, we implement the LoRa and Zigbee protocols as described in section~\xref{xxx}. Table~\ref{tab:protocol} shows the size for implementing each on the FPGA to show it has sufficient resources to support encoding and decoding packets and leave space for additional custom operations.
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
         \hline
         Protocol & \# of LUT4 & FPGA Utilization\\
         \hline
         Single Tone Modulator  & 58 & 0.24\%\\
         \hline
         LoRa Modulator & 1964  & 8\%\\ 
         \hline
         LoRa Demodulator & xxx  & xxx\\ 
         \hline
         Zigbee Modulator & xxx & xxx\\ 
         \hline
         Zigbee Demodulator & xxx & xxx\\ 
         \hline
    \end{tabular}
    \caption{\footnotesize{\bf FPGA resources required to implement different protocols.}}
    \label{tab:protocols}
\end{table}

Table~\ref{tab:protocols} shows the resources required to implement each protocol, next we evaluate the performance of our implementations. First, we use our LoRa modulator to generate packets with payload size three bytes with an SF of 9 and bandwidth of 500~kHz which we transmit at xx~dBm. We connect the output of \name through a rotary attenuator (xxx) to a Semtech SX1276 LoRa receiver~\cite{sx1257} which we use to measure the packet error rate versus transmitted power and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our implementation to transmissions from an SX1276 LoRa chip and find that we can achieve a comparable sensitivity of -123~dBm which is the LoRa sensitivity with $SF=9$ and $BW=500kHz$. 

Next we evaluate our LoRa demodulator. We connect the output of the Semtech SX1276 LoRa transmitter with an output of -11.5~dBm to \name through a rotary attenuator. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. We use the attenuator to vary the power and plot the results in Fig.~\ref{fig:bench_lora_rx_per}. Our LoRa demodulator can demodulate chirp symbols up to -123~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=250kHz$.

%Todo write up zigbee section
%TODO fig: zigbee per vs rssi tx
%TODO fig: zigbee per vs rssi rx

\subsection{Over-the-air Update}
In order to understand how our SDR system can perform in a real world deployments that may require updating code to run different experiments we evaluate our over the air update system. An effective OTA update system should both minimize use of system resources such as power as well as network downtime. As explained above, the components of our OTA update system consumes a peak power of xx for xx during the update and only xx in sleep mode. By scaling this to once per hour the average power would only be xx, while scaling it to once per day would require as little as xx.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Demodulator Evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different signal powers.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.15in
\end{figure}


We also evaluate the time required for updating a node. Considering the actual time to reprogram the FPGA and microcontroller is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. While compression can reduce the transmission time, it also requires additional time to uncompress the data. To see the impact on a real deployment, we evaluate the total downtime when sending both the raw programming data and the same data compressed using xxx. We set up a LoRa transmitter connected to an xxx antenna transmitting at xxx~dBm and measure the time required to send the programming data at different distances.
%TODO add note about location of experiment e.g. open field etc.

% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\cline{1-3}
\multicolumn{2}{|c|}{Components}       & Price (\$)    \\\hline
\multirow{2}{*}{DSP} & FPGA         & 8.69            \\\cline{2-3}
                     & Oscillator   & 0.9            \\\hline
\multirow{2}{*}{IQ Front-End}       & Radio             & 5.08  \\\cline{2-3}
                                    & Crystal           & 0.53  \\\cline{2-3}
                                    & 2.4~GHz Balun     & 0.36  \\\cline{2-3}
                                    & Sub-GHz Balun     & 0.3   \\\hline
\multirow{2}{*}{Backbone}           & Radio            & 4.5   \\\cline{2-3}
                                    & Crystal           & 0.4    \\\cline{2-3}
                                    & Flash Memory      & 1.6    \\\hline
\multirow{2}{*}{MAC}                & MCU               & 3.89   \\\cline{2-3}
                                    & Crystals          & 0.68    \\\hline
\multirow{2}{*}{RF}                 & Switch            & 3.14    \\\cline{2-3}
                                    & Sub-GHz PA        & 1.54    \\\cline{2-3}
                                    & 2.4~GHz PA        & 1.72    \\\hline
\multirow{1}{*}{Power Management}   & Regulators        & 3.3     \\\hline
\multirow{1}{*}{Supporting Components}      & --        & 4.5     \\\hline
\multirow{2}{*}{Production}         & Fabrication       & 4     \\\cline{2-3}
                                    & Assembly          & 10      \\\hline
\multirow{1}{*}{\bf Total}          & --  & {\bf 55.13}    \\\hline
\end{tabular}
\caption{\footnotesize{\bf Cost breakdown of all the components in \name for 1000 board production.}}
\label{tab:cost}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}




\subsection{Latency}
%TODO
%text only different protocols lora/zigbee numbers


\subsection{Cost}

==> eval-3.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Single Tone Transmitter Power Consumption.} We show the total power consumption of \name in single transmitter mode at different output power. Note: this figure will be updated! XXXX}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}

\section{Evaluation}
% In this section, we evaluated our \name platform to show that it is meeting the requirements of an IoT node.

\subsection{Single-Tone Modulator}
To evaluate \name platform in basic operations at different frequency bands, we implement a single-tone modulator on FPGA. This modulator generates I/Q samples for a continues single-tone transmission and interfaces with LVDS serial interface of I/Q radio front-end. The transmitter power is highly dependent on the output level of the radio and presents a trade-off versus range: high transmit power enables longer range  but requires additional power. To understand this relationship we use an xxx spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and use an xxx mulitmeter to measure the DC power required. Fig~\ref{fig:bench_tx_power} shows the results. We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the external power amplifier (PA).

\subsection{LoRa}
% talk about the LoRa modulation to show its complication
% explain the implementation block diagram at a high-level
% and how are we generating chirp and receiving chirp
% show sensitivity plots, powers and FPGA resource usage 
% we transmit and receive the signal with the same sensitivity as the LoRa chipset

To demonstrate the capability of \name at sub-GHz frequency band, we implemented LoRa modulator and demodulator by putting AT86RF215 in 900~MHz I/Q and programming the FPGA by LoRa baseband. LoRa uses Chirp Spread Scpectrum (CSS) modulation. In CSS, data is modulated using linearly increasing frequency signals or upchirp symbol. Each upchirp symbol has two main features; Spreading Factor (SF) and Bandwidth (BW). Spreading factor determines the length of each upchirp sysmbol and also is equivalent to number of bits that each upchirp symbol reperesents~\cite{netscatter,lorabackscatter}. LoRa uses SF values from 6 to 12. BW determines the total frequency spectrum that each upchirp symbol utilizes. Each upchirp symbol covers the whole BW frequency and the starting point of the symbol in frequency domain determines the symbol value~\cite{lora_basics}. In this section, we first explain our LoRa modulator/demodulator implementation and then we evaluate our implementation.

\noindent {\bf LoRa Modulator.} Fig.~\ref{fig:lora_tx_block} shows the block diagram of our LoRa modulator. We implement this modulator chain in Verilog HDL programming. Modulator starts with determining LoRa configurations such as SF and BW and symbols values in {Packet Generator} module. Then, the {Chirp Generator} module uses these information to generate each chirp symbol. It uses a phase accumulator along with two lookup tables for $Sin$ and $Cosin$ functions to generate I/Q samples. We feed I/Q samples to {I/Q Serializer} to serialize I/Q samples and generate serial information compatible with radio front-end interface. Finally, we feed serial I/Q samples along with TX clock to two LVDS interfaces that are connected to radio front-end.

\noindent {\bf LoRa Demodulator.} Fig.~\ref{fig:lora_rx_block} shows the block diagram of our LoRa demodulator. This demodulator interfaces with radio fornt-end using two LVDS connections; one for I/Q serial data (RXD) and the other for synchronization clock (RXCLK). We implement an {I/Q Deserializer} module to convert serial I/Q data to parallel I/Q for further signal processing. Then, we run these data through a low-pass FIR filter. We use a memory in FPGA to buffer raw samples between the front-end and our demodulator. We use the Chirp Generator that we implemented for LoRa modulator to generate a baseline upchirp/downchirp symbol and then we multiply that with the received chirp symbol using Chirp Multiplier unit. Then, we use FFT core implementation provide by Lattice to perform FFT operation on multiplied signal and then detect symbol value and symbol type (upchirp or downchirp) using our Symbol Detector implementation.

To show the performance of our LoRa implementation, first we evaluate our LoRa modulator. To do this, we use our LoRa modulator to generate packets with three bytes payload with $SF=9$ and $BW=500~kHz$ which we transmit at xx~dBm. We connect the output of \name through a rotary attenuator to a Semtech SX1276 LoRa transceiver~\cite{sx1257} which we use to measure the packet error rate versus transmitted power and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our LoRa modulator implementation to transmissions from an SX1276 LoRa chip and find that we can achieve a comparable sensitivity of -123~dBm which is the LoRa sensitivity with $SF=9$ and $BW=500kHz$ configuration. 

Next we evaluate our LoRa demodulator. We connect the output of the Semtech SX1276 LoRa transmitter with an output of -11.5~dBm to \name through a rotary attenuator. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. We use the attenuator to vary the power and plot the results in Fig.~\ref{fig:bench_lora_rx_per}. Our LoRa demodulator can demodulate chirp symbols up to -123~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=250kHz$.

Next we evaluate the resource utilization of our LoRa implementation on FPGA. Table~\ref{tab:protocol} shows the size for implementing modulator and demodulator on FPGA. This table shows that our FPGA has sufficient resources to support different modules for LoRa protocol while it has sufficient resources for additional custom operations. 


\subsection{Zigbee}

\subsection{Sleep Mode}
Since \name implementation includes multiple components, we define sleep mode operation in terms of the state mode for each component. Therefore, we evaluate power consumption, latency and XXX in following sections based on this definition.

In sleep mode, the MCU controlls every component to reduce the power consumption. For I/Q transceiver we use sleep mode that is defined on the transceiver itself and consumes only 30~nA current. Similarly, we put LoRa radio in sleep mode which consumes 200~nA current. To reduce the static power consumption of the FPGA, we shutdown the FPGA by disabling voltage regulators that provide power to each FPGA IO bank and core voltage. Similarly, we turn off the voltage regulators that provide voltage for sub-GHz PA and 2.4~GHz PA in sleep mode. Finally, we put the MCU in sleep mode XXX and setup timer for wake up to reduce even more power.


% \subsection{Power Consumption}
% \textcolor{red}{Add peak current (to know what kind of batteries you can use etc).}
% We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
         \hline
         Mode & Power (mW) \\
         \hline
         LoRa TX & xxx\\ 
         \hline
         LoRa RX & xxx\\
         \hline
         Zigbee TX & xxx\\
         \hline
         Zigbee RX & xxx\\
         \hline
         OTA programming & xxx \\
         \hline
         OTA sleep & xxx \\
         \hline
         All components in sleep mode & xxx \\ 
         \hline
    \end{tabular}
    \caption{\footnotesize{\bf Power consumption of our SDR platform while performing different operations.}}
    \label{tab:power}
\end{table}

\subsection{Duty-cycling}
Many IoT nodes often perform short, simple tasks they are typically duty cycled to allow for further power savings. In \name, the microcontroller has the functionality to disable power consuming components such as the radio, power amplifiers and FPGA and enter a low power sleep mode. Table~\ref{tab:wakeup} shows both the time required to wake up from sleep mode as well as the average power consumed by each component running at an xx\% duty cycle. At this table shows, FPGA boot up from shutdown state has the dominant time in our platform. The total time for \name to be completely functional in RX/TX modes is XXX which is the sum of wake-up time for FPGA and MCU. This is because we perform I/Q radio setup in parallel to the FPGA boot up.

\begin{table}[H]
    \centering
    \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
    \vskip -0.15 in
    \begin{tabular}{|c|c|c|}
         \hline
         Mode & Wake-up time (ms) & Average power (mW) \\
         \hline
         FPGA & 35 & xxx\\ 
         \hline
         MCU & 0.17 & xxx\\
         \hline
         I/Q Radio & 4.9 & xxx\\ 
         \hline
         {\bf Total} & 35.17 & xxx\\ 
         \hline
    \end{tabular}
    \label{tab:wakeup}
\end{table}

To further demonstrate the capabilities of \name, we also evaluate it in a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. Fig.~\ref{fig:wakeup_curve} shows the results for this process, and the average power is xx. This means that \name can achieve a battery life of xx using an xx battery.


\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Modulator Evaluation.} We evaluate our LoRa modulator in comparision with Semtech SX1276 LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}


\begin{table}[]
    \centering
    \caption{\footnotesize{\bf FPGA resources required to implement different protocols.}}
    \vskip -0.15 in
    \begin{tabular}{|c|c|c|}
         \hline
         Protocol & \# of LUT4 & FPGA Utilization\\
         \hline
         Single Tone Modulator  & 58 & 0.24\%\\
         \hline
         LoRa Modulator & 1964  & 8\%\\ 
         \hline
         LoRa Demodulator & xxx  & xxx\\ 
         \hline
         Zigbee Modulator & xxx & xxx\\ 
         \hline
         Zigbee Demodulator & xxx & xxx\\ 
         \hline
    \end{tabular}
    \label{tab:protocols}
\end{table}


%Todo write up zigbee section
%TODO fig: zigbee per vs rssi tx
%TODO fig: zigbee per vs rssi rx

\subsection{Over-the-air Update}
In order to understand how our SDR system can perform in a real world deployments that may require updating code to run different experiments we evaluate our over the air update system. An effective OTA update system should both minimize use of system resources such as power as well as network downtime. As explained above, the components of our OTA update system consumes a peak power of xx for xx during the update and only xx in sleep mode. By scaling this to once per hour the average power would only be xx, while scaling it to once per day would require as little as xx.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Demodulator Evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different signal powers.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.15in
\end{figure}


We also evaluate the time required for updating a node. Considering the actual time to reprogram the FPGA and microcontroller is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. While compression can reduce the transmission time, it also requires additional time to uncompress the data. To see the impact on a real deployment, we evaluate the total downtime when sending both the raw programming data and the same data compressed using xxx. We set up a LoRa transmitter connected to an xxx antenna transmitting at xxx~dBm and measure the time required to send the programming data at different distances.
%TODO add note about location of experiment e.g. open field etc.

% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\cline{1-3}
\multicolumn{2}{|c|}{Components}       & Price (\$)    \\\hline
\multirow{2}{*}{DSP} & FPGA         & 8.69            \\\cline{2-3}
                     & Oscillator   & 0.9            \\\hline
\multirow{2}{*}{IQ Front-End}       & Radio             & 5.08  \\\cline{2-3}
                                    & Crystal           & 0.53  \\\cline{2-3}
                                    & 2.4~GHz Balun     & 0.36  \\\cline{2-3}
                                    & Sub-GHz Balun     & 0.3   \\\hline
\multirow{2}{*}{Backbone}           & Radio            & 4.5   \\\cline{2-3}
                                    & Crystal           & 0.4    \\\cline{2-3}
                                    & Flash Memory      & 1.6    \\\hline
\multirow{2}{*}{MAC}                & MCU               & 3.89   \\\cline{2-3}
                                    & Crystals          & 0.68    \\\hline
\multirow{2}{*}{RF}                 & Switch            & 3.14    \\\cline{2-3}
                                    & Sub-GHz PA        & 1.54    \\\cline{2-3}
                                    & 2.4~GHz PA        & 1.72    \\\hline
\multirow{1}{*}{Power Management}   & Regulators        & 3.3     \\\hline
\multirow{1}{*}{Supporting Components}      & --        & 4.5     \\\hline
\multirow{2}{*}{Production}         & Fabrication       & 3     \\\cline{2-3}
                                    & Assembly          & 10      \\\hline
\multirow{1}{*}{\bf Total}          & --  & {\bf 54.13}    \\\hline
\end{tabular}
\caption{\footnotesize{\bf Cost breakdown of all the components in \name for 1000 board production.}}
\label{tab:cost}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}







\subsection{Cost}

==> eval-4.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf Single-tone transmitter power consumption.} We show the total power consumption of \name in single transmitter mode at different output power. Note: this figure will be updated! XXXX}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}

\section{Evaluation}
In this section, we evaluate the performance of \name to show how that it meets our design requirements for prototyping IoT nodes. We begin with benchmarks and specs detailing radio performance, power consumption

\subsection{Single-Tone Modulator}
To evaluate \name platform in basic operations at different frequency bands, we implement a single-tone modulator on FPGA. This modulator generates I/Q samples for a continues single-tone transmission and interfaces with LVDS serial interface of I/Q radio front-end. The transmitter power is highly dependent on the output level of the radio and presents a trade-off versus range: high transmit power enables longer range  but requires additional power. To understand this relationship we use an xxx spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and use an xxx mulitmeter to measure the DC power required. Fig~\ref{fig:bench_tx_power} shows the results. We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the external power amplifier (PA).

\subsection{LoRa Evaluation}
To show the performance of our LoRa implementation, first we evaluate our LoRa modulator. To do this, we use our LoRa modulator to generate packets with three bytes payload with $SF=9$ and $BW=500~kHz$ which we transmit at xx~dBm. We connect the output of \name through a rotary attenuator to a Semtech SX1276 LoRa transceiver~\cite{sx1257} which we use to measure the packet error rate versus transmitted power and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our LoRa modulator implementation to transmissions from an SX1276 LoRa chip and find that we can achieve a comparable sensitivity of -123~dBm which is the LoRa sensitivity with $SF=9$ and $BW=500kHz$ configuration. 

Next we evaluate our LoRa demodulator. We connect the output of the Semtech SX1276 LoRa transmitter with an output of -11.5~dBm to \name through a rotary attenuator. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. We use the attenuator to vary the power and plot the results in Fig.~\ref{fig:bench_lora_rx_per}. Our LoRa demodulator can demodulate chirp symbols up to -123~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=250kHz$.

Next we evaluate the resource utilization of our LoRa implementation on FPGA. Table~\ref{tab:protocol} shows the size for implementing modulator and demodulator on FPGA. This table shows that our FPGA has sufficient resources to support different modules for LoRa protocol while it has sufficient resources for additional custom operations. 


\subsection{BLE Evaluation}

\subsection{Sleep Mode}
Since \name implementation includes multiple components, we define sleep mode operation in terms of the state mode for each component. Therefore, we evaluate power consumption, latency and XXX in following sections based on this definition.

In sleep mode, the MCU controls every component to reduce the power consumption. For I/Q transceiver we use sleep mode that is defined on the transceiver itself and consumes only 30~nA current. Similarly, we put LoRa radio in sleep mode which consumes 200~nA current. To reduce the static power consumption of the FPGA, we shutdown the FPGA by disabling voltage regulators that provide power to each FPGA IO bank and core voltage. Similarly, we turn off the voltage regulators that provide voltage for sub-GHz PA and 2.4~GHz PA in sleep mode. Finally, we put the MCU in sleep mode XXX and setup timer for wake up to reduce even more power.


% \subsection{Power Consumption}
% \textcolor{red}{Add peak current (to know what kind of batteries you can use etc).}
% We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|}
         \hline
         Mode & Power (mW) \\
         \hline
         LoRa TX & xxx\\ 
         \hline
         LoRa RX & xxx\\
         \hline
         Zigbee TX & xxx\\
         \hline
         Zigbee RX & xxx\\
         \hline
         OTA programming & xxx \\
         \hline
         OTA sleep & xxx \\
         \hline
         All components in sleep mode & xxx \\ 
         \hline
    \end{tabular}
    \caption{\footnotesize{\bf Power consumption of our SDR platform while performing different operations.}}
    \label{tab:power}
\end{table}

\subsection{Duty-cycling}
Many IoT nodes often perform short, simple tasks they are typically duty cycled to allow for further power savings. In \name, the microcontroller has the functionality to disable power consuming components such as the radio, power amplifiers and FPGA and enter a low power sleep mode. Table~\ref{tab:wakeup} shows both the time required to wake up from sleep mode as well as the average power consumed by each component running at an xx\% duty cycle. At this table shows, FPGA boot up from shutdown state has the dominant time in our platform. The total time for \name to be completely functional in RX/TX modes is XXX which is the sum of wake-up time for FPGA and MCU. This is because we perform I/Q radio setup in parallel to the FPGA boot up.

\begin{table}[H]
    \centering
    \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
    \vskip -0.15 in
    \begin{tabular}{|c|c|c|}
         \hline
         Mode & Wake-up time (ms) & Average power (mW) \\
         \hline
         FPGA & 35 & xxx\\ 
         \hline
         MCU & 0.17 & xxx\\
         \hline
         I/Q Radio & 4.9 & xxx\\ 
         \hline
         {\bf Total} & 35.17 & xxx\\ 
         \hline
    \end{tabular}
    \label{tab:wakeup}
\end{table}

To further demonstrate the capabilities of \name, we also evaluate it in a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. Fig.~\ref{fig:wakeup_curve} shows the results for this process, and the average power is xx. This means that \name can achieve a battery life of xx using an xx battery.


\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Modulator Evaluation.} We evaluate our LoRa modulator in comparison with Semtech LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}


\begin{table}[]
    \centering
    \caption{\footnotesize{{\bf FPGA utilization for LoRa protocol.}}}
    \vskip -0.15 in
    \begin{tabular}{|c|c|c|}
         \hline
         SF & LoRa TX (LUT4) & LoRa RX (LUT4)\\
         \hline
         6 & 976 (4\%) & 2656 (10\%)\\
         \hline
         7 & 976 (4\%) & 2670 (10\%)\\
         \hline
         8 & 976 (4\%) & 2700 (11\%)\\
         \hline
         9 & 976 (4\%) & 2742 (11\%)\\
         \hline
         10 & 976 (4\%) & 2786 (11\%)\\
         \hline
         11 & 976 (4\%) & 2794 (11\%)\\
         \hline
         12 & 976 (4\%) & 2818 (11\%)\\
         \hline
    \end{tabular}
    \label{tab:lora_utilization}
\end{table}

\begin{table}[]
    \centering
    \caption{\footnotesize{{\bf Programming data compression.}}}
    \vskip -0.15 in
    \begin{tabular}{|C{2.6cm}|C{2.2cm}|C{2.2cm}|}
         \hline \rowcolor{lightgray}
         {\bf Protocol Implementation} & {\bf FPGA Compression Ratio} & {\bf MCU Compression Ratio}\\
         \hline
         LoRa RX and TX & XXX\% & XX\%\\ 
         \hline
         BLE Beacon & XXX\% & XX\%\\ 
         \hline
    \end{tabular}
    \label{tab:ota_compression}
\end{table}

% \begin{table}[]
%     \centering
%     \caption{\footnotesize{FPGA resources required to implement different protocols.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          Protocol & \# of LUT4 & FPGA Utilization\\
%          \hline
%          Single Tone Modulator  & 58 & 0.24\%\\
%          \hline
%          LoRa Modulator & 1964  & 8\%\\ 
%          \hline
%          LoRa Demodulator & xxx  & xxx\\ 
%          \hline
%          Zigbee Modulator & xxx & xxx\\ 
%          \hline
%          Zigbee Demodulator & xxx & xxx\\ 
%          \hline
%     \end{tabular}
%     \label{tab:lora_utilization}
% \end{table}


\subsection{Over-the-air Update}
In order to understand how our SDR system can perform in a real world deployments that may require updating code to run different experiments we evaluate our over the air update system. An effective OTA update system should both minimize use of system resources such as power as well as network downtime. As explained above, the components of our OTA update system consumes a peak power of xx for xx during the update and only xx in sleep mode. By scaling this to once per hour the average power would only be xx, while scaling it to once per day would require as little as xx.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa Demodulator Evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different signal received strength.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.15in
\end{figure}


We also evaluate the time required for updating a node. Considering the actual time to reprogram the FPGA and microcontroller is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. While compression can reduce the transmission time, it also requires additional time to uncompress the data. To see the impact on a real deployment, we evaluate the total downtime when sending both the raw programming data and the same data compressed using xxx. We set up a LoRa transmitter connected to an xxx antenna transmitting at xxx~dBm and measure the time required to send the programming data at different distances.
%TODO add note about location of experiment e.g. open field etc.

% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\cline{1-3}
\multicolumn{2}{|c|}{Components}       & Price    \\\hline
\multirow{2}{*}{DSP} & FPGA         & \$8.69            \\\cline{2-3}
                     & Oscillator   & \$0.9            \\\hline
\multirow{2}{*}{IQ Front-End}       & Radio             & \$5.08  \\\cline{2-3}
                                    & Crystal           & \$0.53  \\\cline{2-3}
                                    & 2.4~GHz Balun     & \$0.36  \\\cline{2-3}
                                    & Sub-GHz Balun     & \$0.3   \\\hline
\multirow{2}{*}{Backbone}           & Radio            & \$4.5   \\\cline{2-3}
                                    & Crystal           & \$0.4    \\\cline{2-3}
                                    & Flash Memory      & \$1.6    \\\hline
\multirow{2}{*}{MAC}                & MCU               & \$3.89   \\\cline{2-3}
                                    & Crystals          & \$0.68    \\\hline
\multirow{2}{*}{RF}                 & Switch            & \$3.14    \\\cline{2-3}
                                    & Sub-GHz PA        & \$1.54    \\\cline{2-3}
                                    & 2.4~GHz PA        & \$1.72    \\\hline
\multirow{1}{*}{Power Management}   & Regulators        & \$3.3     \\\hline
\multirow{1}{*}{Supporting Components}      & --        & \$4.5     \\\hline
\multirow{2}{*}{Production}         & Fabrication       & \$3     \\\cline{2-3}
                                    & Assembly          & \$10      \\\hline
\multirow{1}{*}{\bf Total}          & --  & {\bf \$54.13}    \\\hline
\end{tabular}
\caption{\footnotesize{\bf Cost breakdown of all the components in \name for 1000 board production.}}
\label{tab:cost}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}





\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figs/8_lora_orthogonal_rx/lora_multiple.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Orthogonal Demodulator Evaluation.} XXX}}
	\label{fig:lora_multiple_rx}
    \vskip -0.15in
\end{figure}


\subsection{Cost}




==> eval-5.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf Single-tone transmitter power consumption.} We show the total power consumption of \name in single transmitter mode at different output power.}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}

\section{Evaluation}
We evaluate \name's performance  to show that it meets our design requirements for prototyping IoT nodes. We begin with benchmarks and specs detailing radio performance and power consumption followed by cost estimates. We then present the results with our two case studies. Following this, we evaluate the performance of our over the air update system.

\subsection{Benchmarks and Specifications}
{\bf Radio performance.} As a first test of \name's capabilities, we implement a single-tone modulator on the FPGA that generates the appropriate I/Q samples and streams them over LVDS to the radio. We connect the output to an MDO4104b-6~\cite{mdo4104b} spectrum analyzer and observe a single tone, shown in Fig.~\ref{sdds}, with no unexpected harmonics introduced by the modulator and compliant with the specs in the radio datasheet. 

While the receiver's power consumption is  dependent on the specific decoder and protocol being used, the transmitter's power consumption 
is largely dominated by the radio frontend. To evaluate this, we measure the transmitter's DC power consumption which is highly dependent on the RF output power of the radio and presents a trade-off versus range: high RF transmit power enables longer range but requires additional DC power. To understand this relationship we again use the spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and use a Fluke 287 mulitmeter to measure the DC power required. Fig~\ref{fig:bench_tx_power} shows the power conusmption drawn by our SDR platform, for both 900~MHz and 2.4~GHz operation. As expected the power consumption increases with the radio output power. The power consumption at a radio output power of 0 and 12~dBm at 900~MHz was 231 and 275~mW. This is 16 and 15 times better than the USRP E310. Further, in  comparison with  a non-SDR IoT LoRa chipset such as SX1276, we consume only 5 times more power, while providing full SDR capabilities. %On a XXX~V battery, this translates to a battery-life of XXX years for \name\ with a duty-cycle of XXXx which is typical in LoRa networks~\cite{XXX}.

%We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the separate power amplifier (PA) which is otherwise in a low power sleep mode.

% \subsubsection{Sleep Mode}
% Since \name implementation includes multiple components, we define sleep mode operation in terms of the state mode for each component. Therefore, we evaluate power consumption, latency and XXX in following sections based on this definition.

% In sleep mode, the MCU controls every component to reduce the power consumption. For I/Q transceiver we use sleep mode that is defined on the transceiver itself and consumes only 30~nA current. Similarly, we put LoRa radio in sleep mode which consumes 200~nA current. To reduce the static power consumption of the FPGA, we shutdown the FPGA by disabling voltage regulators that provide power to each FPGA IO bank and core voltage. Similarly, we turn off the voltage regulators that provide voltage for sub-GHz PA and 2.4~GHz PA in sleep mode. Finally, we put the MCU in sleep mode XXX and setup timer for wake up to reduce even more power.


% \subsection{Power Consumption}
% \textcolor{red}{Add peak current (to know what kind of batteries you can use etc).}
% We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{\bf Power consumption of different protocols.}}
%     \vskip -0.15in
%     \footnotesize{
%     \begin{tabular}{|c|c|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol} & {\bf Power (mW)}\\
%          \hline
%          LoRa RX & 166\\    %112mW + 30mA*1.8
%          \hline
%          LoRa TX & 210\\    %95mW + 46mA*2.5
%          \hline
%          BLE Beacon & 222.5\\ %95mW + 51mA*2.5
%          \hline
%     \end{tabular}
%     }
%     \label{tab:protocol_pow}
% \end{table}

% \begin{table}[t]
%     \centering
%     \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          {\bf Operation} & {\bf Wake-up time (ms)}\\
%          \hline
%          FPGA & 35\\ 
%          \hline
%          MCU & 0.17\\
%          \hline
%          I/Q Radio & 4.9\\ 
%          \hline
%          {\bf Total} & 35.17\\ 
%          \hline
%     \end{tabular}
%     \label{tab:wakeup}
% \end{table}

\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|c|c|c|}
         \hline \rowcolor{lightgray}
         {\bf Operation} & {\bf Duration (ms)}\\
         \hline
         Sleep to Radio Operation & 21\\ 
         \hline
         Radio Setup & XXX\\ 
         \hline
         TX to RX & 0.045\\     %TX to TRXprep(33us) + TRXprep to RX(200ns) + SPI (10us)
         \hline
         RX to TX & 0.011\\       %RX to TRXprep(200ns) + TRXprep to TX(200ns) + SPI (10us)
         \hline
         Frequency Switch & 0.220\\ %we measured this
         \hline
    \end{tabular}
    }
    \label{tab:wakeup}
\end{table}


{\bf Duty-cycling.} Many IoT and sensor nodes often perform short, simple tasks allowing them to be heavily duty cycled which is the main way they can achieve battery lifetimes of years. We design \name with this critical need in mind such that the microcontroller can toggle on and off power consuming components such as the radio, power amplifiers and FPGA and enter a low power sleep mode.

We do this by first turning off the the I/Q transceiver and LoRa radios by shutting down their voltage regulator. To reduce the static power consumption of the FPGA, we shut it down by disabling the voltage regulators that provide power to each IO bank and core voltage. Similarly, we turn off the voltage regulators that provide power for the PAs. Finally, we put the MCU in sleep mode LPM3 running only a wakeup timer. As shown in Table.~\ref{tab:protocol_pow}, the measured total system sleep power in this mode was around  30~uW.

The low sleep power allows for significant power savings, but also introduces delay in terms of wake time.  Table~\ref{tab:wakeup} shows  the time required to wake up from sleep mode to having an active radio (Tx/Rx). Because we can perform the I/Q radio setup in parallel with booting the FPGA the total wakeup time for RX and TX is 21~ms. The I/Q radio setup takes XXX and so the wakeup time is dominated by the time to boot up the FPGA which itself takes 21~ms. We compare this to a SmartSense Temperature sensor~\cite{smartthings_temp} and find that \name has only a 4x longer wakeup time even though it requires programming unlike commercial products that use a single protocol radio. Additionally many IoT devices operate at low duty cycles waiting in sleep mode for seconds or more making \name's wakeup latency insignificant.
%A wakeup time of 21~ms is however within the expected wakeup times of IoT devices including XXX and XXX~\cite{XXX}. To fully illustrate the wakeup process we demonstrate a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. %Fig.~\ref{fig:wakeup_curve} shows the power consumption versus time and results in an average power of xx for an xx\% duty cycle. This means that \name can achieve a battery life of xx using an xx battery.

{\bf Switching delays.} We also measure the switching delays for different operations on the radio. Specifically, as shown in Table.~\ref{tab:wakeup}, it takes 45~$\mu$s and 11~$\mu$s to switch from TX to RX mode and RX to TX mode respectively. As we see later, this is sufficient to meet the timing requirements of IoT packet acknowledgements and MAC protocols. Further, the delay for switching between different frequencies is only 220~us. To measure these numbers, we switch between 2.426~GHz and 2.480~GHz on the radio. This switching delay is again sufficient to meet the requirements of frequency hopping during Bluetooth advertising.

{\bf Cost.} In addition to the technical specs of \name, we analyze the cost which is an important practical consideration for real world deployment at scale. Table~\ref{tab:cost} shows a detailed breakdown of cost including each component as well as PCB fabrication and assembly, where the overall cost is <\$55. %This would allow for a 1000 node deployment for under \$60k which is not possible with existing platforms.
% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}
\begin{table}[t]
\centering
\caption{\footnotesize{\bf \Name cost breakdown for 1000 board production.}}
\vskip -0.15in
\footnotesize{
    \begin{tabular}{|c|c|C{1.5cm}|}
    \cline{1-3}\rowcolor{lightgray}
    \multicolumn{2}{|c|}{\bf Components}       & {\bf Price}    \\\hline
    \multirow{DSP} & FPGA         & \$8.69            \\\cline{2-3}
                         & Oscillator   & \$0.9            \\\hline
    \multirow{IQ Front-End}       & Radio             & \$5.08  \\\cline{2-3}
                                        & Crystal           & \$0.53  \\\cline{2-3}
                                        & 2.4~GHz Balun     & \$0.36  \\\cline{2-3}
                                        & Sub-GHz Balun     & \$0.3   \\\hline
    \multirow{Backbone}           & Radio            & \$4.5   \\\cline{2-3}
                                        & Crystal           & \$0.4    \\\cline{2-3}
                                        & Flash Memory      & \$1.6    \\\hline
    \multirow{MAC}                & MCU               & \$3.89   \\\cline{2-3}
                                        & Crystals          & \$0.68    \\\hline
    \multirow{RF}                 & Switch            & \$3.14    \\\cline{2-3}
                                        & Sub-GHz PA        & \$1.54    \\\cline{2-3}
                                        & 2.4~GHz PA        & \$1.72    \\\hline
    \multirow{Power Management}   & Regulators        & \$3.7     \\\hline
    \multirow{Supporting Components}      & --        & \$4.5     \\\hline
    \multirow{Production}         & Fabrication       & \$3     \\\cline{2-3}
                                        & Assembly          & \$10      \\\hline
    \multirow{\bf Total}          & --  & {\bf \$54.53}    \\\hline
    \end{tabular}
}
\label{tab:cost}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}


\subsection{Evaluating Protocols}
To better evaluate the performance of \name, we evaluate our two protocol implementations.

{\bf LoRa using \name.} 
We evaluate various different components of \name\ using LoRa as a case study.

{\it LoRa modulator.} 
 To evaluate this, we use our LoRa modulator to generate packets with three byte payloads using a spreading factor of $SF=9$ and bandwidths of 500~kHz and 250~kHz which we transmit at -13~dBm. We receive the output of \name on a  Semtech SX1276 LoRa transceiver~\cite{sx1257} which we use to measure the packet error rate versus received RSSI and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our LoRa modulator implementation to standard transmissions from an SX1276 LoRa transceiver. The plots show that we can achieve a comparable sensitivity of -123~dBm which is the LoRa sensitivity with $SF=9$ and $BW=500kHz$ configuration. This is true for all the three spreading factors, which shows that our low-power SDR can meet the sensitivity requirement of LPWAN IoT protocols.


{\it Lora demodulator.} Next we evaluate our LoRa demodulator on \name. To test this, we use transmissions from a Semtech SX1276 LoRa transmitter with an output of -11.5~dBm. We use the \name\ platform to receive these transmissions. The LoRa transmitter transmits packets with two configureations using a spreading factor of 8 and bandwidths of 250~kHz and 125~kHz. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. We plot the results in Fig.~\ref{fig:bench_lora_rx_per} as a function of the RSSI values for the LoRa transmissions. Our LoRa demodulator can demodulate chirp symbols up to -123~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=250kHz$.


{\it Resource allocation.} Next we evaluate the resource utilization of our LoRa implementation on FPGA. Table.~\ref{tab:lora_utilization} shows the size for implemented modulator and demodulator on FPGA performing using different SFs. Our LoRa modulator supports all LoRa configurations with different SF with no additional cost. However, in LoRa demodulator, we need FFT blocks with different sizes to support different SF configurations. This table shows that our FPGA has sufficient resources to support different modules for LoRa protocol while it has sufficient resources for additional custom operations. 


{\it LoRa MAC.} ??? There should be something to evaluate it? XXXX Delay for ACK? or scheduling? XXXX CDF?


{\it Power consumption.} XXXWhat is the system power consumption of transmitting a Lora packet? What about receiving? XXXX What are the individual power consumption?XXX


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa modulator evaluation.} We evaluate our LoRa modulator in comparison with Semtech LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa demodulator evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different signal received strength.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.15in
\end{figure}

{\bf BLE using \name.} Next, we evaluate \name\ using BLE beacons as a case study. First, we measure the impact of our BLE beacons transmitted from \name\ using the TI CC2650~\cite{cc2650} BLE chip as a receiver. We do this by configuring \name to transmit BLE beacons at a rate of 1 packet per second.  We transmit 100 packets at  and set the CC2650 BLE chip to report bit error rate (BER). Fig~\ref{fig:bench_ble_tx_ber} shows the BER as a function of the received RSSI as reported by the CC2650 BLE chip. The plot shows that we achieve a sensitivity of -94~dBm. This is  within 2~dB of the CC2650 BLE chipset's sensitivity defined by a BER threshold of $10^-3$.

Next we evaluate the latency of our BLE implementation as BLE beacons are typically transmitted in sequence by hopping between three different advertising channels. We measure the minimum time \name takes to switch between these frequencies by connecting its output to a 2.4~GHz envelope detector and using an MDO4104B-6 oscilloscope to measure the time delay between transmissions. Fig.~\ref{fig:ble_timing} plots a sequence of three BLE beacons transmitted on the advertising channels and show our system can transmit packets in 220~us. Fig.~\ref{SDSD} shows a CDF of this timing value for the BLE beacons transmitted by \name\ and the CCS2650 over 130 packets. The plots show that  the variance for \name\ is small and is  comparable to the CC2650's delay between BLE beacons of xxx~us. 

Finally, our implementation of BLE beacons only requires 3\% of our FPGA resources leaving plenty of space for custom processing. 
% VI: removed this number because it looks VERY bad compared to commercial BLE chips that require 5-10~mW
%Further, the total system power consumption of transmitting each BLE beacon is around 259~mW. 
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/11_ble_tx_rssi/ble_tx_ber.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf BLE evaluation.} We evaluate our BLE packet generator at different power levels.}}
	\label{fig:bench_ble_tx_ber}
    \vskip -0.15in
\end{figure}

\begin{table}[h]
    % \centering
    \begin{minipage}[t]{0.45\linewidth}
        \caption{\footnotesize{{\bf FPGA utilization for LoRa protocol.}}}
        \vskip -0.15 in
        \footnotesize{
        \begin{tabular}{|c|C{1.2cm}|C{1.4cm}|}
             \hline \rowcolor{lightgray}
             {\bf SF} & {\bf LoRa TX (LUT)} & {\bf LoRa RX (LUT)}\\
             \hline
             6 & 976 (4\%) & 2656 (10\%)\\
             \hline
             7 & 976 (4\%) & 2670 (10\%)\\
             \hline
             8 & 976 (4\%) & 2700 (11\%)\\
             \hline
             9 & 976 (4\%) & 2742 (11\%)\\
             \hline
             10 & 976 (4\%) & 2786 (11\%)\\
             \hline
             11 & 976 (4\%) & 2794 (11\%)\\
             \hline
             12 & 976 (4\%) & 2818 (11\%)\\
             \hline
        \end{tabular}
        }
        \label{tab:lora_utilization}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}[t]{0.45\linewidth}
        \caption{\footnotesize{\bf Power consumption of different protocols.}}
        \vskip -0.15 in
        \footnotesize{
        \begin{tabular}{|C{1.5cm}|C{1.4cm}|}
             \hline \rowcolor{lightgray}
             {\bf Protocol} & {\bf Power (mW)}\\
             \hline
             LoRa RX & 182\\    %(112mW + 30mA*1.8)*(Reg. Efficiency = 1.1)
             \hline
             LoRa TX & 283\\    %(95mW + 65mA*2.5)*(Reg. Efficiency = 1.1)
             \hline
             BLE Beacon & 259\\ %(101mW + 51mA*2.5)*(Reg. Efficiency = 1.1)
             \hline
        \end{tabular}
        }
        \label{tab:protocol_pow}
    \end{minipage}
\end{table}


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{{\bf Programming data compression.}}}
%     \vskip -0.15 in
%     \begin{tabular}{|C{2.6cm}|C{2.2cm}|C{2.2cm}|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol Implementation} & {\bf FPGA Compression Ratio} & {\bf MCU Compression Ratio}\\
%          \hline
%          LoRa RX and TX & XXX\% & XX\%\\ 
%          \hline
%          BLE Beacon & XXX\% & XX\%\\ 
%          \hline
%     \end{tabular}
%     \label{tab:ota_compression}
% \end{table}

% \begin{table}[]
%     \centering
%     \caption{\footnotesize{FPGA resources required to implement different protocols.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          Protocol & \# of LUT4 & FPGA Utilization\\
%          \hline
%          Single Tone Modulator  & 58 & 0.24\%\\
%          \hline
%          LoRa Modulator & 1964  & 8\%\\ 
%          \hline
%          LoRa Demodulator & xxx  & xxx\\ 
%          \hline
%          Zigbee Modulator & xxx & xxx\\ 
%          \hline
%          Zigbee Demodulator & xxx & xxx\\ 
%          \hline
%     \end{tabular}
%     \label{tab:lora_utilization}
% \end{table}


\subsection{Over-the-Air Programming}
In order to understand how our SDR system can perform in a real world deployments that may require updating code to run different experiments we evaluate our over the air programming system. An effective OTA programming system should both minimize use of system resources such as power as well as network downtime. As explained above, the components of our OTA programming system consumes a peak power of xx for xx during the update and only xx in sleep mode. By scaling this to once per hour the average power would only be xx, while scaling it to once per day would require as little as xx.

We also evaluate the time required for updating a node. Considering the actual time to reprogram the FPGA and microcontroller is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. To see the impact on a real deployment, we evaluate the time required to programm a \tinysdr node at 10 locations around a university campus. We set up a LoRa transmitter connected to an patch antenna transmitting the update data at 14~dBm according to our protocol and measure the time it takes to program a \tinysdr node at each location. Fig.~\ref{fig:ota_exp} plots a CDF of the results, showing updates take an average of xx.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/10_ota_exp/10_ota_time_cdf.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf OTA Programming Time.} We show CDF of OTA programming time for programming LoRa and BLE implementations on \name.}}
	\label{fig:ota_exp}
    \vskip -0.2in
\end{figure}


==> eval-6.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf Single-tone transmitter power consumption.} We show the total power consumption of \name in single transmitter mode at different output power.}}
	\label{fig:bench_tx_power}
    \vskip -0.15in
\end{figure}

\section{Evaluation}
We evaluate \name's performance  to show that it meets our design requirements for prototyping IoT nodes. We begin with benchmarks and specs detailing radio performance and power consumption followed by cost estimates. We then present the results with our two case studies. Following this, we evaluate the performance of our over the air update system.

\subsection{Benchmarks and Specifications}
{\bf Platform transmit performance.} As a first test of \name's capabilities, we implement a single-tone modulator on the FPGA that generates the appropriate I/Q samples and streams them over LVDS to the radio. We connect the output to an MDO4104b-6~\cite{mdo4104b} spectrum analyzer and observe a single tone, shown in Fig.~\ref{sdds}, with no unexpected harmonics introduced by the modulator and compliant with the specs in the radio datasheet. 

While the receiver's power consumption is  dependent on the specific decoder and protocol being used, the transmitter's power consumption 
is largely dominated by the radio frontend. To evaluate this, we measure the transmitter's power consumption which is highly dependent on the RF output power of the radio and presents a trade-off versus range: high RF transmit power enables longer range but requires additional power. To understand this relationship we again use the spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and use a Fluke 287 mulitmeter to measure the required power. Fig~\ref{fig:bench_tx_power} shows the power consumption drawn by our SDR platform, for both 900~MHz and 2.4~GHz operation. As expected the power consumption increases with the radio output power. The total power consumption at a radio output power of 0 and 14~dBm at 900~MHz was 231 and 283~mW. This is 16 and 15 times better than the USRP E310.  Further, in  comparison with a non-SDR IoT LoRa chipset such as SX1276, we consume only 3 times more power, while providing full SDR capabilities. %On a XXX~V battery, this translates to a battery-life of XXX years for \name\ with a duty-cycle of XXXx which is typical in LoRa networks~\cite{XXX}.
%We measure the power of E310 in the lab.

%We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the separate power amplifier (PA) which is otherwise in a low power sleep mode.

% \subsubsection{Sleep Mode}
% Since \name implementation includes multiple components, we define sleep mode operation in terms of the state mode for each component. Therefore, we evaluate power consumption, latency and XXX in following sections based on this definition.

% In sleep mode, the MCU controls every component to reduce the power consumption. For I/Q transceiver we use sleep mode that is defined on the transceiver itself and consumes only 30~nA current. Similarly, we put LoRa radio in sleep mode which consumes 200~nA current. To reduce the static power consumption of the FPGA, we shutdown the FPGA by disabling voltage regulators that provide power to each FPGA IO bank and core voltage. Similarly, we turn off the voltage regulators that provide voltage for sub-GHz PA and 2.4~GHz PA in sleep mode. Finally, we put the MCU in sleep mode XXX and setup timer for wake up to reduce even more power.


% \subsection{Power Consumption}
% \textcolor{red}{Add peak current (to know what kind of batteries you can use etc).}
% We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{\bf Power consumption of different protocols.}}
%     \vskip -0.15in
%     \footnotesize{
%     \begin{tabular}{|c|c|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol} & {\bf Power (mW)}\\
%          \hline
%          LoRa RX & 166\\    %112mW + 30mA*1.8
%          \hline
%          LoRa TX & 210\\    %95mW + 46mA*2.5
%          \hline
%          BLE Beacon & 222.5\\ %95mW + 51mA*2.5
%          \hline
%     \end{tabular}
%     }
%     \label{tab:protocol_pow}
% \end{table}

% \begin{table}[t]
%     \centering
%     \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          {\bf Operation} & {\bf Wake-up time (ms)}\\
%          \hline
%          FPGA & 35\\ 
%          \hline
%          MCU & 0.17\\
%          \hline
%          I/Q Radio & 4.9\\ 
%          \hline
%          {\bf Total} & 35.17\\ 
%          \hline
%     \end{tabular}
%     \label{tab:wakeup}
% \end{table}

\begin{table}[t]
    \centering
    \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|c|c|c|}
         \hline \rowcolor{lightgray}
         {\bf Operation} & {\bf Duration (ms)}\\
         \hline
         Sleep to Radio Operation & 22\\ 
         \hline
         Radio Setup & 1.2\\ %Reg_wakeup(500)+wake_trxoff+traxoff_txprep
         \hline
         TX to RX & 0.045\\     %TX to TRXprep(33us) + TRXprep to RX(200ns) + SPI (10us)
         \hline
         RX to TX & 0.011\\       %RX to TRXprep(200ns) + TRXprep to TX(200ns) + SPI (10us)
         \hline
         Frequency Switch & 0.220\\ %we measured this
         \hline
    \end{tabular}
    }
    \label{tab:wakeup}
\end{table}


{\bf Duty-cycling.} Many IoT and sensor nodes often perform short, simple tasks allowing them to be heavily duty cycled which is the main way they can achieve battery lifetimes of years. We design \name with this critical need in mind such that the microcontroller can toggle on and off power consuming components such as the radio, power amplifiers and FPGA and enter a low power sleep mode.

We do this by first turning off the the I/Q transceiver and LoRa radios by shutting down their voltage regulator. To reduce the static power consumption of the FPGA, we shut it down by disabling the voltage regulators that provide power to each IO bank and core voltage. Similarly, we turn off the voltage regulators that provide power for the PAs. Finally, we put the MCU in sleep mode LPM3 running only a wakeup timer. As shown in Table.~\ref{tab:protocol_pow}, the measured total system sleep power in this mode was 30~uW.

The low sleep power allows for significant power savings, but also introduces delay in terms of wake time.  Table~\ref{tab:wakeup} shows  the time required to wake up from sleep mode to having an active radio (Tx/Rx). Because we can perform the I/Q radio setup in parallel with booting the FPGA the total wakeup time for RX and TX is 22~ms. The I/Q radio setup takes 1.2~ms and so the wakeup time is dominated by the time to boot up the FPGA which itself takes 22~ms. We compare this to a SmartSense Temperature sensor~\cite{smartthings_temp} and find that \name has only a 4x longer wakeup time even though it requires programming unlike commercial products that use a single protocol radio. Additionally many IoT devices operate at low duty cycles waiting in sleep mode for seconds or more making \name's wakeup latency insignificant.
%A wakeup time of 21~ms is however within the expected wakeup times of IoT devices including XXX and XXX~\cite{XXX}. To fully illustrate the wakeup process we demonstrate a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. %Fig.~\ref{fig:wakeup_curve} shows the power consumption versus time and results in an average power of xx for an xx\% duty cycle. This means that \name can achieve a battery life of xx using an xx battery.

{\bf Switching delays.} We also measure the switching delays for different operations on the radio. Specifically, as shown in Table.~\ref{tab:wakeup}, it takes 45~$\mu$s and 11~$\mu$s to switch from TX to RX mode and RX to TX mode respectively. As we see later, this is sufficient to meet the timing requirements of IoT packet acknowledgements and MAC protocols. Further, the delay for switching between different frequencies is only 220~us. To measure these numbers, we switch between 2.426~GHz and 2.480~GHz on the radio. This switching delay is again sufficient to meet the requirements of frequency hopping during Bluetooth advertising.

{\bf Cost.} In addition to the technical specs of \name, we analyze the cost which is an important practical consideration for real world deployment at scale. Table~\ref{tab:cost} shows a detailed breakdown of cost including each component as well as PCB fabrication and assembly, where the overall cost is <\$55. %This would allow for a 1000 node deployment for under \$60k which is not possible with existing platforms.
% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}
\begin{table}[t]
\centering
\caption{\footnotesize{\bf \Name cost breakdown for 1000 board production.}}
\vskip -0.15in
\footnotesize{
    \begin{tabular}{|c|c|C{1.5cm}|}
    \cline{1-3}\rowcolor{lightgray}
    \multicolumn{2}{|c|}{\bf Components}       & {\bf Price}    \\\hline
    \multirow{DSP} & FPGA         & \$8.69            \\\cline{2-3}
                         & Oscillator   & \$0.9            \\\hline
    \multirow{IQ Front-End}       & Radio             & \$5.08  \\\cline{2-3}
                                        & Crystal           & \$0.53  \\\cline{2-3}
                                        & 2.4~GHz Balun     & \$0.36  \\\cline{2-3}
                                        & Sub-GHz Balun     & \$0.3   \\\hline
    \multirow{Backbone}           & Radio            & \$4.5   \\\cline{2-3}
                                        & Crystal           & \$0.4    \\\cline{2-3}
                                        & Flash Memory      & \$1.6    \\\hline
    \multirow{MAC}                & MCU               & \$3.89   \\\cline{2-3}
                                        & Crystals          & \$0.68    \\\hline
    \multirow{RF}                 & Switch            & \$3.14    \\\cline{2-3}
                                        & Sub-GHz PA        & \$1.54    \\\cline{2-3}
                                        & 2.4~GHz PA        & \$1.72    \\\hline
    \multirow{Power Management}   & Regulators        & \$3.7     \\\hline
    \multirow{Supporting Components}      & --        & \$4.5     \\\hline
    \multirow{Production}         & Fabrication       & \$3     \\\cline{2-3}
                                        & Assembly          & \$10      \\\hline
    \multirow{\bf Total}          & --  & {\bf \$54.53}    \\\hline
    \end{tabular}
}
\label{tab:cost}
\end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}


\subsection{Evaluating Protocols}
To better evaluate the performance of \name, we evaluate our two protocol implementations.

{\bf LoRa using \name.} 
We evaluate various different components of \name\ using LoRa as a case study.

{\it LoRa modulator.} 
 To evaluate this, we use our LoRa modulator to generate packets with three byte payloads using a spreading factor of $SF=9$ and bandwidths of 500~kHz and 250~kHz which we transmit at -13~dBm. We receive the output of \name on a  Semtech SX1276 LoRa transceiver~\cite{sx1257} which we use to measure the packet error rate versus received RSSI and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our LoRa modulator implementation to standard transmissions from an SX1276 LoRa transceiver. The plots show that we can achieve a comparable sensitivity of -123~dBm which is the LoRa sensitivity with $SF=9$ and $BW=500kHz$ configuration. This is true for all the three spreading factors, which shows that our low-power SDR can meet the sensitivity requirement of LPWAN IoT protocols.


{\it Lora demodulator.} Next we evaluate our LoRa demodulator on \name. To test this, we use transmissions from a Semtech SX1276 LoRa transmitter with an output of -11.5~dBm. We use the \name\ platform to receive these transmissions. The LoRa transmitter transmits packets with two configureations using a spreading factor of 8 and bandwidths of 250~kHz and 125~kHz. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. We plot the results in Fig.~\ref{fig:bench_lora_rx_per} as a function of the RSSI values for the LoRa transmissions. Our LoRa demodulator can demodulate chirp symbols up to -123~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=250kHz$.


{\it Resource allocation.} Next we evaluate the resource utilization of our LoRa implementation on FPGA. Table.~\ref{tab:lora_utilization} shows the size for implemented modulator and demodulator on FPGA performing using different SFs. Our LoRa modulator supports all LoRa configurations with different SF with no additional cost. However, in LoRa demodulator, we need FFT blocks with different sizes to support different SF configurations. This table shows that our FPGA has sufficient resources to support different modules for LoRa protocol while it has sufficient resources for additional custom operations. 


{\it LoRa MAC.} ??? There should be something to evaluate it? XXXX Delay for ACK? or scheduling? XXXX CDF?


{\it Power consumption.} XXXWhat is the system power consumption of transmitting a Lora packet? What about receiving? XXXX What are the individual power consumption?XXX


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa modulator evaluation.} We evaluate our LoRa modulator in comparison with Semtech LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa demodulator evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different signal received strength.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.15in
\end{figure}

{\bf BLE using \name.} Next, we evaluate \name\ using BLE beacons as a case study. First, we measure the impact of our BLE beacons transmitted from \name\ using the TI CC2650~\cite{cc2650} BLE chip as a receiver. We do this by configuring \name to transmit BLE beacons at a rate of 1 packet per second.  We transmit 100 packets at  and set the CC2650 BLE chip to report bit error rate (BER). Fig~\ref{fig:bench_ble_tx_ber} shows the BER as a function of the received RSSI as reported by the CC2650 BLE chip. The plot shows that we achieve a sensitivity of -94~dBm. This is  within 2~dB of the CC2650 BLE chipset's sensitivity defined by a BER threshold of $10^-3$.

Next we evaluate the latency of our BLE implementation as BLE beacons are typically transmitted in sequence by hopping between three different advertising channels. We measure the minimum time \name takes to switch between these frequencies by connecting its output to a 2.4~GHz envelope detector and using an MDO4104B-6 oscilloscope to measure the time delay between transmissions. Fig.~\ref{fig:ble_timing} plots a sequence of three BLE beacons transmitted on the advertising channels and show our system can transmit packets in 220~us. Fig.~\ref{SDSD} shows a CDF of this timing value for the BLE beacons transmitted by \name\ and an iPhone 6s over 130 packets. The plots show that  the variance for \name\ is small and is less than the iPhone's delay between BLE beacons of 350~us. 

Finally, our implementation of BLE beacons only requires 3\% of our FPGA resources leaving plenty of space for custom processing. 
% VI: removed this number because it looks VERY bad compared to commercial BLE chips that require 5-10~mW
%Further, the total system power consumption of transmitting each BLE beacon is around 259~mW. 
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/11_ble_tx_rssi/ble_tx_ber.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf BLE evaluation.} We evaluate our BLE packet generator at different power levels.}}
	\label{fig:bench_ble_tx_ber}
    \vskip -0.15in
\end{figure}

\begin{table}[h]
    % \centering
    \begin{minipage}[t]{0.45\linewidth}
        \caption{\footnotesize{{\bf FPGA utilization for LoRa protocol.}}}
        \vskip -0.15 in
        \footnotesize{
        \begin{tabular}{|c|C{1.2cm}|C{1.4cm}|}
             \hline \rowcolor{lightgray}
             {\bf SF} & {\bf LoRa TX (LUT)} & {\bf LoRa RX (LUT)}\\
             \hline
             6 & 976 (4\%) & 2656 (10\%)\\
             \hline
             7 & 976 (4\%) & 2670 (10\%)\\
             \hline
             8 & 976 (4\%) & 2700 (11\%)\\
             \hline
             9 & 976 (4\%) & 2742 (11\%)\\
             \hline
             10 & 976 (4\%) & 2786 (11\%)\\
             \hline
             11 & 976 (4\%) & 2794 (11\%)\\
             \hline
             12 & 976 (4\%) & 2818 (11\%)\\
             \hline
        \end{tabular}
        }
        \label{tab:lora_utilization}
    \end{minipage}
    \hspace{0.2in}
    \begin{minipage}[t]{0.45\linewidth}
        \caption{\footnotesize{\bf Power consumption of different protocols.}}
        \vskip -0.15 in
        \footnotesize{
        \begin{tabular}{|C{1.5cm}|C{1.4cm}|}
             \hline \rowcolor{lightgray}
             {\bf Protocol} & {\bf Power (mW)}\\
             \hline
             LoRa RX & 182\\    %(112mW + 30mA*1.8)*(Reg. Efficiency = 1.1)
             \hline
             LoRa TX & 283\\    %(95mW + 65mA*2.5)*(Reg. Efficiency = 1.1)
             \hline
             BLE Beacon & 259\\ %(101mW + 51mA*2.5)*(Reg. Efficiency = 1.1)
             \hline
        \end{tabular}
        }
        \label{tab:protocol_pow}
    \end{minipage}
\end{table}


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{{\bf Programming data compression.}}}
%     \vskip -0.15 in
%     \begin{tabular}{|C{2.6cm}|C{2.2cm}|C{2.2cm}|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol Implementation} & {\bf FPGA Compression Ratio} & {\bf MCU Compression Ratio}\\
%          \hline
%          LoRa RX and TX & XXX\% & XX\%\\ 
%          \hline
%          BLE Beacon & XXX\% & XX\%\\ 
%          \hline
%     \end{tabular}
%     \label{tab:ota_compression}
% \end{table}

% \begin{table}[]
%     \centering
%     \caption{\footnotesize{FPGA resources required to implement different protocols.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          Protocol & \# of LUT4 & FPGA Utilization\\
%          \hline
%          Single Tone Modulator  & 58 & 0.24\%\\
%          \hline
%          LoRa Modulator & 1964  & 8\%\\ 
%          \hline
%          LoRa Demodulator & xxx  & xxx\\ 
%          \hline
%          Zigbee Modulator & xxx & xxx\\ 
%          \hline
%          Zigbee Demodulator & xxx & xxx\\ 
%          \hline
%     \end{tabular}
%     \label{tab:lora_utilization}
% \end{table}


\subsection{Over-the-Air Programming}
In order to understand how our SDR system can perform in a real world deployments that may require updating code to run different experiments we evaluate our over the air programming system. An effective OTA programming system should both minimize use of system resources such as power as well as network downtime. As explained above, the components of our OTA programming system consumes a peak power of xx for xx during the update and only xx in sleep mode. By scaling this to once per hour the average power would only be xx, while scaling it to once per day would require as little as xx.

We also evaluate the time required for updating a node. Considering the time to reprogram the FPGA and microcontroller from flash is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. To see the impact on a real deployment, we evaluate the time required to program a \tinysdr node at 10 locations around a university campus. We set up a LoRa transmitter connected to an patch antenna transmitting the update data at 14~dBm according to our protocol and measure the time it takes to program a \tinysdr node at each location. Fig.~\ref{fig:ota_exp} plots a CDF of the results, showing updates take an average of xx.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/10_ota_exp/10_ota_time_cdf.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf OTA Programming Time.} We show CDF of OTA programming time for programming LoRa and BLE implementations on \name.}}
	\label{fig:ota_exp}
    \vskip -0.2in
\end{figure}


==> eval-7.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/15_spectrum/15_spectrum_plot.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf \Name Single-Tone Frequency Spectrum}}}
	\label{fig:spectrum}
    \vskip -0.11in
\end{figure}

\begin{table}[t!]
    \centering
    \caption{\footnotesize{\bf Different Operation Timing for \Name}}
    \vskip -0.15 in
    \footnotesize{
    \begin{tabular}{|C{4cm}|C{2cm}|}
         \hline \rowcolor{lightgray}
         {\bf Operation} & {\bf Duration (ms)}\\
         \hline
         Sleep to Radio Operation & 22\\ 
         \hline
         Radio Setup & 1.2\\ %Reg_wakeup(500)+wake_trxoff+traxoff_txprep
         \hline
         TX to RX & 0.045\\     %TX to TRXprep(33us) + TRXprep to RX(200ns) + SPI (10us)
         \hline
         RX to TX & 0.011\\       %RX to TRXprep(200ns) + TRXprep to TX(200ns) + SPI (10us)
         \hline
         Frequency Switch & 0.220\\ %we measured this
         \hline
    \end{tabular}
    }
    \vskip -0.2in
    \label{tab:wakeup}
\end{table}

\section{Evaluation}
We deploy a testbed of 20 \name devices across  our institution's campus as shown in Fig.~\ref{fig:ota_map}; we removed the details of the map for anonymity.
To see if \name meets the requirements for IoT endpoint devices, we characterize its power, computational resource usage, delays and cost when operating in different modes and running different protocols. 

%We begin with benchmarks and specs detailing radio performance and power consumption followed by cost estimates. We then present the results with our two case studies. Following this, we evaluate the performance of our over the air update system.

\subsection{Benchmarks and Specifications}
{\bf Sleep mode power.} Many IoT and sensor nodes often perform short, simple tasks allowing them to be heavily duty cycled which is the main way they can achieve battery lifetimes of years. We design \name with this critical need in mind such that the microcontroller can toggle on and off power consuming components such as the radio, power amplifiers and FPGA and enter a low power sleep mode.




We do this by first turning off the the I/Q transceiver and LoRa radios. To reduce the static power consumption of the FPGA, we shut it down by disabling the voltage regulators that provide power to each I/O bank and core voltage. Similarly, we also  turn off the PAs. Finally, we put the MCU in sleep mode LPM3 running only a wakeup timer. The measured total system sleep power in this mode was 30~uW.

The low sleep power allows for significant power savings, but also introduces delay in terms of wake time.  Table~\ref{tab:wakeup} shows  the time required to wake up from sleep mode to having an active radio (Tx/Rx). Because we can perform the I/Q radio setup in parallel with booting the FPGA the total wakeup time for RX and TX is 22~ms. The I/Q radio setup takes 1.2~ms and so the wakeup time is dominated by the time to boot up the FPGA which itself takes 22~ms. We compare this to a SmartSense Temperature sensor~\cite{smartthings_temp} and find that \name has only a 4x longer wakeup time even though it requires programming unlike commercial products that use a single protocol radio. Additionally many IoT devices operate at low duty cycles waiting in sleep mode for seconds or more making \name's wakeup latency insignificant.
%A wakeup time of 21~ms is however within the expected wakeup times of IoT devices including XXX and XXX~\cite{XXX}. To fully illustrate the wakeup process we demonstrate a typical IoT use case. Specifically, we measure the power consumption of our platform as it wakes up from sleep mode, measures a sensor value, and transmits a packet. %Fig.~\ref{fig:wakeup_curve} shows the power consumption versus time and results in an average power of xx for an xx\% duty cycle. This means that \name can achieve a battery life of xx using an xx battery.

{\bf Switching delays.} We also measure the switching delays for different operations on the I/Q radio as is an important parameter for meeting MAC and protocol timing requirements.  Table.~\ref{tab:wakeup} shows that it takes 45~$\mu$s and 11~$\mu$s to switch from TX to RX mode and RX to TX mode respectively. As we see later, this is sufficient to meet the timing requirements of IoT packet ACKs and MAC protocols. Further, the delay for switching between different frequencies is only 220~us. To measure this number, we switch between 2.402~GHz, 2.426~GHz and 2.480~GHz frequencies on the radio. This switching delay is again sufficient to meet the requirements of frequency hopping during Bluetooth advertising.




\begin{table}[t]
\centering
\caption{\footnotesize{\bf \Name Cost Breakdown for 1000 Units}}
\vskip -0.15in
\footnotesize{
    \begin{tabular}{|c|c|C{1.5cm}|}
    \cline{1-3}\rowcolor{lightgray}
    \multicolumn{2}{|c|}{\bf Components}       & {\bf Price}    \\\hline
    \multirow{DSP} & FPGA         & \$8.69            \\\cline{2-3}
                         & Oscillator   & \$0.9            \\\hline
    \multirow{IQ Front-End}       & Radio             & \$5.08  \\\cline{2-3}
                                        & Crystal           & \$0.53  \\\cline{2-3}
                                        & 2.4~GHz Balun     & \$0.36  \\\cline{2-3}
                                        & Sub-GHz Balun     & \$0.3   \\\hline
    \multirow{Backbone}           & Radio            & \$4.5   \\\cline{2-3}
                                        & Crystal           & \$0.4    \\\cline{2-3}
                                        & Flash Memory      & \$1.6    \\\hline
    \multirow{MAC}                & MCU               & \$3.89   \\\cline{2-3}
                                        & Crystals          & \$0.68    \\\hline
    \multirow{RF}                 & Switch            & \$3.14    \\\cline{2-3}
                                        & Sub-GHz PA        & \$1.54    \\\cline{2-3}
                                        & 2.4~GHz PA        & \$1.72    \\\hline
    \multirow{Power Management}   & Regulators        & \$3.7     \\\hline
    \multirow{Supporting Components}      & --        & \$4.5     \\\hline
    \multirow{Production}         & Fabrication~\cite{pcbminions}       & \$3     \\\cline{2-3}
                                        & Assembly~\cite{pcbminions}          & \$10      \\\hline
    \multirow{\bf Total}          & --  & {\bf \$54.53}    \\\hline
    \end{tabular}
}
\vskip -0.2in
\label{tab:cost}
\end{table}




{\bf Transmitter performance.} First,  we implement a single-tone modulator on the FPGA that generates the appropriate I/Q samples and streams them over LVDS to the radio. We connect the output to an MDO4104b-6~\cite{mdo4104b} spectrum analyzer and observe a single tone, shown in Fig.~\ref{fig:spectrum}, with no unexpected harmonics introduced by the modulator.  % and compliant with the specs in the radio datasheet~\cite{at86rf215}.

While the receiver's power consumption is  dependent on the specific decoder and protocol being used, the transmitter's power consumption 
is largely dominated by the radio frontend. To evaluate this, we measure the transmitter's power consumption which is highly dependent on the RF output power of the radio. To understand this relationship we again use the spectrum analyzer to measure the output power of the radio for different gain settings while it is transmitting a single tone signal and use a Fluke 287 multimeter to measure the required power. Fig~\ref{fig:bench_tx_power} shows the power consumption drawn by our SDR platform, for both 900~MHz and 2.4~GHz operation. As expected the power consumption increases with the radio output power. {The total power consumption of \name platform including I/Q radio, FPGA, MCU and regulators at radio output power of 0 and 14~dBm at 900~MHz is 231 and 283~mW. This is 16 and 15 times better than the USRP E310.}  %On a XXX~V battery, this translates to a battery-life of XXX years for \name\ with a duty-cycle of XXXx which is typical in LoRa networks~\cite{XXX}.
%We measure the power of E310 in the lab.

%We note that the sharp increase in power above xx~dBm indicates the maximum output power of the XXX radio front end and transmitting at higher power requires turning on the separate power amplifier (PA) which is otherwise in a low power sleep mode.

% \subsubsection{Sleep Mode}
% Since \name implementation includes multiple components, we define sleep mode operation in terms of the state mode for each component. Therefore, we evaluate power consumption, latency and XXX in following sections based on this definition.

% In sleep mode, the MCU controls every component to reduce the power consumption. For I/Q transceiver we use sleep mode that is defined on the transceiver itself and consumes only 30~nA current. Similarly, we put LoRa radio in sleep mode which consumes 200~nA current. To reduce the static power consumption of the FPGA, we shutdown the FPGA by disabling voltage regulators that provide power to each FPGA IO bank and core voltage. Similarly, we turn off the voltage regulators that provide voltage for sub-GHz PA and 2.4~GHz PA in sleep mode. Finally, we put the MCU in sleep mode XXX and setup timer for wake up to reduce even more power.


% \subsection{Power Consumption}
% \textcolor{red}{Add peak current (to know what kind of batteries you can use etc).}
% We begin by evaluating the power consumption of \name to demonstrate it is both lower power than any SDR platform on the market and more importantly that its power requirements are within an acceptable range for use as an IoT endpoint. We measure the power consumption for different functions such as running a transmitter or receiver for various protocols by running each function xx times and measuring the required current and voltage using an xxx digital multimeter. We show the results in Table~\ref{tab:power}. To give some comparison, the XXX LoRa radio consumes XX~mW in receive mode making \name only xxx more power expensive than these custom solutions. 


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{\bf Power consumption of different protocols.}}
%     \vskip -0.15in
%     \footnotesize{
%     \begin{tabular}{|c|c|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol} & {\bf Power (mW)}\\
%          \hline
%          LoRa RX & 166\\    %112mW + 30mA*1.8
%          \hline
%          LoRa TX & 210\\    %95mW + 46mA*2.5
%          \hline
%          BLE Beacon & 222.5\\ %95mW + 51mA*2.5
%          \hline
%     \end{tabular}
%     }
%     \label{tab:protocol_pow}
% \end{table}

% \begin{table}[t]
%     \centering
%     \caption{\footnotesize{\bf Wake-up times for each component of \name.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          {\bf Operation} & {\bf Wake-up time (ms)}\\
%          \hline
%          FPGA & 35\\ 
%          \hline
%          MCU & 0.17\\
%          \hline
%          I/Q Radio & 4.9\\ 
%          \hline
%          {\bf Total} & 35.17\\ 
%          \hline
%     \end{tabular}
%     \label{tab:wakeup}
% \end{table}



\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/5_bench_power/bench_tx_pow.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf Single-Tone Transmitter Power Consumption.} We show the total power consumption of \name including I/Q radio, FPGA,  MCU  and regulators at different transmitter output power. This is 15-16 times lower power consumption than the USRP E310 embedded SDR.}}
	\label{fig:bench_tx_power}
    \vskip -0.2in
\end{figure}


{\bf Cost.} We also analyze the cost which is an important practical consideration for real world deployment at scale. Table~\ref{tab:cost} shows a detailed breakdown of cost including each component as well as PCB fabrication and assembly based on quotes for 1000 units~\cite{XXX}, where the overall cost is  around  \$55. %This would allow for a 1000 node deployment for under \$60k which is not possible with existing platforms.
% \usepackage{array}
% \usepackage{multirow,longtable,array}
% \renewcommand{\arraystretch}{1}


% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%          \hline
%          Component & Cost \\
%          \hline
%          FPGA  & 8.69\\ 
%          \hline 
%          Microcontroller  & 3.89\\ 
%          \hline
%          I/Q Front-End  & 5.08\\ 
%          \hline
%          OTA Components & xxx\\ 
%          \hline
%          LoRa Radio & xxx\\ 
%          \hline
%          PCB cost & xxx\\ 
%          \hline
%          Assembly cost & xxx\\ 
%          \hline
%          \textbf{Total} & \textbf{xxx}\\ 
%          \hline
%     \end{tabular}
%     \caption{\footnotesize{\bf Cost breakdown of all the components in \name.}}
%     \label{tab:cost}
% \end{table}


\subsection{Evaluating the Case Studies}
%To better evaluate the performance of \name, we evaluate our two protocols: LoRa and BLE beacons.

{\bf LoRa using \name.} 
We evaluate various different components of \name\ using LoRa as a case study.

{\it LoRa modulator.} 
 To evaluate this, we use our LoRa modulator to generate packets with three byte payloads using a spreading factor of $SF=8$ and bandwidths of 250~kHz and 125~kHz which we transmit at -13~dBm. We receive the output of \name on a  Semtech SX1276 LoRa transceiver~\cite{sx1257} which we use to measure the packet error rate versus RSSI and plot the results in Fig.~\ref{fig:bench_lora_tx_per}. We compare our LoRa modulator to transmissions from an SX1276 LoRa transceiver. The plots show that we can achieve a comparable sensitivity of -126~dBm which is the LoRa sensitivity for $SF=8$ and $BW=125kHz$ configuration. This is true for both configurations, which shows that our low-power SDR can meet the sensitivity requirement of LPWAN IoT protocols.


{\it Lora demodulator.} Next we evaluate our LoRa demodulator on \name. To test this, we use transmissions from a Semtech SX1276 LoRa transceiver and use the \name\ platform to receive these transmissions. The LoRa transceiver transmits packets with two configurations using a spreading factor of 8 and bandwidths of 250~kHz and 125~kHz. We record the received RF signal in the FPGA memory and run it through our demodulator to compute a chirp symbol error rate. \textcolor{red}{Note that the Semtech LoRa transceiver does not give access to symbol error rate but  since  we have  access to I/Q samples, we can  compute it on our platform.} We plot the results in Fig.~\ref{fig:bench_lora_rx_per} as a function of the LoRa RSSI values. Our LoRa demodulator can demodulate chirp symbols up to -126~dBm which is LoRa protocol sensitivity at $SF=8$ and $BW=125kHz$. Both the LoRa modulator  and demodulator run in real-time. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_lora_tx_rssi/lora_tx_per.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf LoRa Modulator Evaluation.} We evaluate our LoRa modulator in comparison with Semtech LoRa chip.}}
	\label{fig:bench_lora_tx_per}
    \vskip -0.15in
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/2_lora_rx_rssi/lora_rx_chirp.eps}
    \vskip -0.15in
    \caption{\footnotesize{{\bf LoRa Demodulator Evaluation.} We evaluate our LoRa demodulator by demodulating chirp symbols at different RSSI.}}
	\label{fig:bench_lora_rx_per}
    \vskip -0.2in
\end{figure}

\begin{table}[t]
    \centering
    % \begin{minipage}[t]{\linewidth}
        \caption{\footnotesize{{\bf FPGA Utilization for LoRa Protocol}}}
        \vskip -0.15 in
        \footnotesize{
        \begin{tabular}{|C{1cm}|C{2.5cm}|C{2.5cm}|}
             \hline \rowcolor{lightgray}
             {\bf SF} & {\bf LoRa TX (LUT)} & {\bf LoRa RX (LUT)}\\
             \hline
             6 & 976 (4\%) & 2656 (10\%)\\
             \hline
             7 & 976 (4\%) & 2670 (10\%)\\
             \hline
             8 & 976 (4\%) & 2700 (11\%)\\
             \hline
             9 & 976 (4\%) & 2742 (11\%)\\
             \hline
             10 & 976 (4\%) & 2786 (11\%)\\
             \hline
             11 & 976 (4\%) & 2794 (11\%)\\
             \hline
             12 & 976 (4\%) & 2818 (11\%)\\
             \hline
        \end{tabular}
        }
        \label{tab:lora_utilization}
        \vskip -0.2in
    % \end{minipage}
    % \hspace{0.2in}
    % \begin{minipage}[t]{0.45\linewidth}
    %     \caption{\footnotesize{\bf Power consumption of different protocols.}}
    %     \vskip -0.15 in
    %     \footnotesize{
    %     \begin{tabular}{|C{1.5cm}|C{1.4cm}|}
    %          \hline \rowcolor{lightgray}
    %          {\bf Protocol} & {\bf Power (mW)}\\
    %          \hline
    %          LoRa RX & 186\\    %(112mW + 30mA*1.8+4mW MCU)*(Reg. Efficiency = 1.1)
    %          \hline
    %          LoRa TX & 287\\    %(95mW + 65mA*2.5+4mW MCU)*(Reg. Efficiency = 1.1)
    %          \hline
    %          BLE Beacon & 263\\ %(101mW + 51mA*2.5+4mW MCU)*(Reg. Efficiency = 1.1)
    %          \hline
    %     \end{tabular}
    %     }
    %     \vskip -0.2in
    %     \label{tab:protocol_pow}
    % \end{minipage}
\end{table}

{\it Resource allocation.} Next, we evaluate the resource utilization of our LoRa PHY implementation on FPGA. Table.~\ref{tab:lora_utilization} shows the size for implemented modulator and demodulator on FPGA performing using different SFs. Our LoRa modulator supports all LoRa configurations with different SF with no additional cost. However, in LoRa demodulator, we need FFT blocks with different sizes to support different SF configurations. This table shows that our FPGA has sufficient resources to support different modules for LoRa protocol while it has sufficient resources for additional custom operations. 

% ??? There should be something to evaluate it? XXXX Delay for ACK? or scheduling? XXXX CDF?
%(32+15)/256=18%
%5/65
{\it LoRa MAC.} We implement the LoRa MAC based on TTN's Arduino libraries~\cite{ttnarduino}. TTN protocol together with control for I/Q radio, backbone radio, FPGA and PMU and decompression algorithm for OTA take 18\% of MCU resources. Also, as shown in Table~\ref{tab:wakeup}, our timings are well within the requirements for LoRaWAN specifications~\cite{loraalliance} by LoRa Alliance. 

% XXXWhat is the system power consumption of transmitting a Lora packet? What about receiving? XXXX What are the individual power consumption?XXX
 We also measure the power consumption of our platform for LoRa packet transmission and reception. LoRa packet transmission with $SF=9$ and $BW=500~kHz$ and radio output power of 14~dBm consumes a total power of 287~mW from which 179~mW is for the radio and the rest is for the FPGA and MCU. LoRa packet reception consumes 186~mW with radio taking 59~mW.
% In comparison with a non-SDR IoT LoRa chipset such as SX1276, we consume only 3 times more power, while providing full SDR capabilities. SX1276 packet reception takes around 20~mW.



{\bf BLE using \name.} Next, we evaluate \name\ using BLE beacons as a case study. First, we measure the impact of our BLE beacons transmitted from \name\ using the TI CC2650~\cite{cc2650} BLE chip as a receiver. We do this by configuring \name to transmit BLE beacons at a rate of 1 packet per second.  We transmit 100 packets   and set the CC2650 BLE chip to report bit error rate (BER). Fig~\ref{fig:bench_ble_tx_ber} shows the BER as a function of the received RSSI as reported by the CC2650 BLE chip. The plot shows that we achieve a sensitivity of -94~dBm. This is  within 2~dB of the CC2650 BLE chipset's sensitivity, defined by a BER threshold of $10^{-3}$.

Next we evaluate the latency of our BLE implementation as BLE beacons are typically transmitted in sequence by hopping between three different advertising channels. We measure the minimum time \name takes to switch between these frequencies by connecting its output to a 2.4~GHz envelope detector and using an MDO4104B-6 oscilloscope to measure the time delay between transmissions. Fig.~\ref{fig:ble_timing} plots a sequence of three BLE beacons in time-domain transmitted on the advertising channels and shows that our system can transmit packets with 220~us delay between advertising beacons. The corresponding result when a iPhone 8 transmits beacons is 350~us. Finally, our implementation of BLE beacons only requires 3\% of the FPGA resources on the platform \textcolor{red}{ and can run for over 2 years on a 1000~mAh battery when transmitting once per second} 

% Fig.~\ref{SDSD} shows a CDF of this timing value for the BLE beacons transmitted by \name\ and an iPhone 6s over 130 packets. The plots show that  the variance for \name\ is small and is less than the iPhone's delay between BLE beacons of 350~us. 

% VI: removed this number because it looks VERY bad compared to commercial BLE chips that require 5-10~mW
%Further, the total system power consumption of transmitting each BLE beacon is around 259~mW. 



% \begin{table}[h]
%     % \centering
%     \begin{minipage}[t]{0.45\linewidth}
%         \caption{\footnotesize{{\bf FPGA utilization for LoRa protocol.}}}
%         \vskip -0.15 in
%         \footnotesize{
%         \begin{tabular}{|c|C{1.2cm}|C{1.4cm}|}
%              \hline \rowcolor{lightgray}
%              {\bf SF} & {\bf LoRa TX (LUT)} & {\bf LoRa RX (LUT)}\\
%              \hline
%              6 & 976 (4\%) & 2656 (10\%)\\
%              \hline
%              7 & 976 (4\%) & 2670 (10\%)\\
%              \hline
%              8 & 976 (4\%) & 2700 (11\%)\\
%              \hline
%              9 & 976 (4\%) & 2742 (11\%)\\
%              \hline
%              10 & 976 (4\%) & 2786 (11\%)\\
%              \hline
%              11 & 976 (4\%) & 2794 (11\%)\\
%              \hline
%              12 & 976 (4\%) & 2818 (11\%)\\
%              \hline
%         \end{tabular}
%         }
%         \label{tab:lora_utilization}
%     \end{minipage}
%     \hspace{0.2in}
%     \begin{minipage}[t]{0.45\linewidth}
%         \caption{\footnotesize{\bf Power consumption of different protocols.}}
%         \vskip -0.15 in
%         \footnotesize{
%         \begin{tabular}{|C{1.5cm}|C{1.4cm}|}
%              \hline \rowcolor{lightgray}
%              {\bf Protocol} & {\bf Power (mW)}\\
%              \hline
%              LoRa RX & 182\\    %(112mW + 30mA*1.8)*(Reg. Efficiency = 1.1)
%              \hline
%              LoRa TX & 283\\    %(95mW + 65mA*2.5)*(Reg. Efficiency = 1.1)
%              \hline
%              BLE Beacon & 259\\ %(101mW + 51mA*2.5)*(Reg. Efficiency = 1.1)
%              \hline
%         \end{tabular}
%         }
%         \label{tab:protocol_pow}
%     \end{minipage}
% \end{table}


% \begin{table}[]
%     \centering
%     \caption{\footnotesize{{\bf Programming data compression.}}}
%     \vskip -0.15 in
%     \begin{tabular}{|C{2.6cm}|C{2.2cm}|C{2.2cm}|}
%          \hline \rowcolor{lightgray}
%          {\bf Protocol Implementation} & {\bf FPGA Compression Ratio} & {\bf MCU Compression Ratio}\\
%          \hline
%          LoRa RX and TX & XXX\% & XX\%\\ 
%          \hline
%          BLE Beacon & XXX\% & XX\%\\ 
%          \hline
%     \end{tabular}
%     \label{tab:ota_compression}
% \end{table}

% \begin{table}[]
%     \centering
%     \caption{\footnotesize{FPGA resources required to implement different protocols.}}
%     \vskip -0.15 in
%     \begin{tabular}{|c|c|c|}
%          \hline
%          Protocol & \# of LUT4 & FPGA Utilization\\
%          \hline
%          Single Tone Modulator  & 58 & 0.24\%\\
%          \hline
%          LoRa Modulator & 1964  & 8\%\\ 
%          \hline
%          LoRa Demodulator & xxx  & xxx\\ 
%          \hline
%          Zigbee Modulator & xxx & xxx\\ 
%          \hline
%          Zigbee Demodulator & xxx & xxx\\ 
%          \hline
%     \end{tabular}
%     \label{tab:lora_utilization}
% \end{table}

\subsection{Over-the-Air Programming}
In order to understand how our SDR system can perform in a real world deployments that may require updating firmware to run different experiments we evaluate our over the air programming system. An effective OTA programming system should both minimize use of system resources such as power as well as network downtime. Considering the time to reprogram the FPGA and microcontroller from flash is fixed, the downtime for programming a node depends only on the throughput which varies with SNR. To see the impact on a real deployment, we evaluate the time required to program a \tinysdr node at 20 locations around a university campus. We set up LoRa transceiver with $SF=8$, $BW=500~kHz$ and $CodingRate=6$ configuration connected to an patch antenna transmitting at 14~dBm as an AP and measure the time it takes to program a \tinysdr node at each location according to our protocol. We send FPGA compressed programming bitstream for LoRa (BLE) with 95~kB (37~kB) programming data size. Fig.~\ref{fig:ota_exp} plots a CDF of the results, showing OTA programming of the FPGA with LoRa (BLE) bitstream takes an average of 150s (59s). Our OTA programming system components, backbone radio and MCU, consumes an average energy of 6144~mJ (2342~mJ) with 14~dBm output power for \name backbone radio for LoRa (BLE). Having a 1000~mAh LiPo battery, we can OTA program \name 2100 (5600) times for similar FPGA compressed bitstream file sizes. Assuming OTA programming of once per day, the average power consumption would be 71~uW and 27~uW respectively.




% \begin{figure}[t]
%     \begin{subfigure}{0.49\linewidth}
%     \centering
%         \includegraphics[width=1\linewidth]{figs/10_ota_exp/10_ota_time_cdf.eps}
%         \vskip -0.1in
%         \caption{\footnotesize{{\bf Programming Time}}}
%         \label{fig:ota_exp}
%     \end{subfigure}
% 	\begin{subfigure}{0.48\linewidth}
% 	    \centering
%         \includegraphics[width=0.59\linewidth]{figs/10_ota_exp/map.eps}
%         \vskip -0.1in
%         \caption{\footnotesize{{\bf Evaluation Map}}}
%         \label{fig:ota_map}
%     \end{subfigure}
%     \vskip -0.1in
%     \caption{\footnotesize{{\bf OTA Programming Evaluation.} We show CDF of OTA programming time for programming LoRa and BLE implementations.}}
%     \label{fig:ota_eval}
% \end{figure}



==> hardware-0.tex <==
\section{Hardware Implementations}
Next we describe the implementation details of our hardware prototypes such as the PCB design and clocking. We build two prototypes: \name V1, in which we implement the core software radio components and \name V2 in which we design the final cost and form factor optimized version including the OTA update system. We explain the details of each below.

\subsection{\name V1}
Before designing the full system we begin by prototyping the core SDR modules including the FPGA, radio, MCU, and SD card to validate our key performance specs such as sensitivity and ability to process samples in real time. \name V1 is shown in Fig.~\ref{fig:tinysdrv1}. The design consists of a four layer FR-4 PCB and uses the M2GL010-FGG484~\cite{igloo2} IGLOO2 FPGA from Microsemi. The IGLOO FPGA has a large internal SRAM memory which allows for easy debugging by simply recording I/Q samples in memory which can be saved to a computer using a JTAG debugger. We verify the performance of our LVDS interface and I/Q radio as well as as the ability to write data to the SD card. Additionally this platform allows us to test the interface between the radio and MSP430FR5969~\cite{msp430} and evaluate the characteristics of the radio output signal. While the IGLOO2 allows for easy prototyping, its high price ($\approx \$40$), limited number of logic units, and large form factor make it impractical for a final design. 


\subsection{\name V2}
After verifying the core components on \name V1, we developed \name V2 which fully optimizes the size, power and form factor to achieve our original design specs. We implement \name V2 on a 6 layer FR-4 PCB with dimension of $3cm\times 5cm$ as shown in Fig.~\ref{fig:sdr_hardware}. In this version, we implement the power management system described above with multiple controllable voltage domains. We use MSP432P401R~\cite{msp432P401R} microcontroller which is in the same family as the MCU described above but provides more FLASH and SRAM memory necessary for data compression in our OTA system. In addition, it support multiple SPI interfaces which we use to interface with FPGA, I/Q radio and backbone radio.

In this design we also exchange the large, expensive IGLOO2 for the smaller form factor LFE5U-25F-BG256~\cite{latticeLFE5U} FPGA from Lattice Semiconductor and has almost 2x more logic units. We connect the FPGA with I/Q radio using LVDS, and these connections require careful design. Each differential signal has two trace lines on PCB which must be the same length to have similar timing characteristics. We use tools in design software to implement differential lines with same length. In addition, LVDS requires 100~$\ohm$ differential impedance between two lines. To do this, we simulate differential impedance between LVDS lines based on material properties, differential line width and separation and PCB layers and use the results to set the appropriate dimensions.

In addition to the PCB design considerations we also have to coordinate the various clocks and timing on each device. Both of the radios require crystals which they use as a reference for their onboard PLLs which synthesize the high frequency RF signals. While the FPGA has a dedicated 32~MHz reference oscillator and onboard PLL it uses for generating the 64~MHz clock when transmitting samples over LVDS, and it maintains synchronization when reading by instead using a clock reference output by the radio. The MCU also has both a high frequency mode which can run up to 48~MHz to perform computation intensive tasks like compression and an ultra-low power watchdog timer when in sleep mode.

In addition, we add SX1276 radio for backbone support along with the supporting hardware as well as the various voltage regulators discussed previously to minimize power. \name V2 also exposes a number of external interfaces to the MCU such as SPI, I2C and ADC pins which can be used to connect a variety of analog or digital sensors to create a complete IoT sensor node.

%The sleep process which is controlled by the MCU is the following, it sets the timer, puts all the regulators to shut-down mode and then it goes to low power mode consuming only 550~nA.


==> hardware-1.tex <==
%\section{Hardware Implementations}


%{\bf \name v1.} Before designing the full system we begin by prototyping the core SDR modules including the FPGA, radio, MCU, and SD card to validate our key performance specs such as sensitivity and ability to process samples in real time. \name V1 is shown in Fig.~\ref{fig:tinysdrv1}. The design consists of a four layer FR-4 PCB and uses the M2GL010-FGG484~\cite{igloo2} IGLOO2 FPGA from Microsemi. The IGLOO FPGA has a large internal SRAM memory which allows for easy debugging by simply recording I/Q samples in memory which can be saved to a computer using a JTAG debugger. We verify the performance of our LVDS interface and I/Q radio as well as as the ability to write data to the SD card. Additionally this platform allows us to test the interface between the radio and MSP430FR5969~\cite{msp430} and evaluate the characteristics of the radio output signal. While the IGLOO2 allows for easy prototyping, its high price ($\approx \$40$), limited number of logic units, and large form factor make it impractical for a final design. 


%{\bf \name V2.} After verifying the core components on \name V1, we developed \name V2 which fully optimizes the size, power and form factor to achieve our original design specs. We implement \name V2 on a 6 layer FR-4 PCB with dimension of $3cm\times 5cm$ as shown in Fig.~\ref{fig:sdr_hardware}. In this version, we implement the power management system described above with multiple controllable voltage domains. We use MSP432P401R~\cite{msp432P401R} microcontroller which is in the same family as the MCU described above but provides more FLASH and SRAM memory necessary for data compression in our OTA system. In addition, it support multiple SPI interfaces which we use to interface with FPGA, I/Q radio and backbone radio.

%In this design we also exchange the large, expensive IGLOO2 for the smaller form factor LFE5U-25F-BG256~\cite{latticeLFE5U} FPGA from Lattice Semiconductor and has almost 2x more logic units. We connect the FPGA with I/Q radio using LVDS, and these connections require careful design. Each differential signal has two trace lines on PCB which must be the same length to have similar timing characteristics. We use tools in design software to implement differential lines with same length. In addition, LVDS requires 100~$\ohm$ differential impedance between two lines. To do this, we simulate differential impedance between LVDS lines based on material properties, differential line width and separation and PCB layers and use the results to set the appropriate dimensions.

%In addition to the PCB design considerations we also have to coordinate the various clocks and timing on each device. Both of the radios require crystals which they use as a reference for their onboard PLLs which synthesize the high frequency RF signals. While the FPGA has a dedicated 32~MHz reference oscillator and onboard PLL it uses for generating the 64~MHz clock when transmitting samples over LVDS, and it maintains synchronization when reading by instead using a clock reference output by the radio. The MCU also has both a high frequency mode which can run up to 48~MHz to perform computation intensive tasks like compression and an ultra-low power watchdog timer when in sleep mode.

%%In addition, we add SX1276 radio for backbone support along with the supporting hardware as well as the various voltage regulators discussed previously to minimize power. \name V2 also exposes a number of external interfaces to the MCU such as SPI, I2C and ADC pins which can be used to connect a variety of analog or digital sensors to create a complete IoT sensor node.

==> impl-1.tex <==
%explain that we built the first version to show the proof of concept, evaluate radio and MAC capabilities. Then we design second version with new requirements such as larger FPGA, power managemnet, MCU that can handle multiple radios and etc.

\section{Hardware Implementation}
In this section we go over the implementation of \name hardware and present design choices. 
Fig.~\ref{fig:blcok} shows the block diagram of \name system. We choose various components of our implementation based on this block diagram to fulfill our goals for \name that mentioned in XXX.

We use a low-power low-cost RF front-end, AT86RF215~\cite{ref:AT86RF215} from Microchip as the I/Q transceiver for our design. This radio can operate in 400~MHz, 900~MHz and 2.4~GHz frequency bands which satisfy our goal of supporting different ISM bands. It provides all the necessary blocks of the transceiver chain from the antenna to the digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, synthesizer and voltage-controlled oscillator. To exchange digitized I/Q baseband data between radio and baseband processing unit, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. This chip is capable of 13~bits ADC/DAC which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP~\cite{xxxx}. To receive I/Q samples from this radio, we need to interface with an FPGA with LVDS capability.

We use LFE5U-25F~\cite{} FPGA from Lattice Semiconductor for baseband processing. This FPGA has 24k logic units, it supports multiple I/O voltages for different interfaces and also it has LVDS capability. We use a small form-factor of this FPGA on our design. Hoever, the logic unit size is more than most of the existing SDR platforms including XXX, XXX and XXX. We use an external FLASH memory with XX~Mb size which can store multiple boots of this FPGA at the same time. We connect FPGA to flash with a Quad SPI interface to enable dynamic programmable capability for the FPGA.

To enable over-the-air updates, we use a Semtech SX1276~\cite{sx1276} LoRa radio as the backbone radio. SX1276 can operate at different LoRa configurations, it provides long-range coverage and it is power efficient. This chip supports frequency range of 137~MHz to 1020~MHz with bitrate range of 0.018~kbps to 37.5~kbps.


In \name platform, we control every components with a low-power microcontroller. We use MSP432P401R~\cite{} 32-Bit Cortex M4F microcontroller to controll two radios, communicate with baseband processor and power management. This microcontroller has 64~kB RAM along with 256~kB FLASH memory for programming. This microcontroller provides huge flexibility for performing compression algorithms, complex MAC layer implementation IoT protocols and sensor reading applications.

Finally, to implement the RF section we use two RF paths, one for sub-GHz frequency bands and the other for 2.4~GHz frequency band. We use 2.4~GHz power amplifier ,SE2431L~\cite{}, and 900~MHz band power amplifier, SE2435L~\cite{}, to increase the maximum output power of our radios. Since both I/Q radio and backbone radio share the sub-GHz RF path, we use an ADG904~\cite{} RF switch to select between I/Q radio, RX and TX mode of LoRa radio.

We integrate all components on a 6-layers FR-4 PCB with the dimension of $30mm\times50mm$ as shown in Fig.~\ref{fig:board}. Our board provides different sensor interfaces including SPI and I2C as external GPIOs for sensor reading applications.


\begin{figure}[t]
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_tx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{XXX}}
        \label{fig:lora_tx_block}
    \end{subfigure}
% 	\begin{subfigure}{\linewidth}
% 	    \centering
%         \includegraphics[width=1\linewidth]{figs/block_diagram/tx_block.eps}
%         \caption{\footnotesize{{\bf Single Tone Transmitter.}}}
%         \label{fig:tx_block}
%     \end{subfigure}
    \vskip -0.15in
    \caption{\footnotesize{LoRa FPGA Block Diagrams. XXX}}
    \label{fig:lora_blocks}
\end{figure}



==> impl-2.tex <==
%explain that we built the first version to show the proof of concept, evaluate radio and MAC capabilities. Then we design second version with new requirements such as larger FPGA, power managemnet, MCU that can handle multiple radios and etc.

\section{Hardware Implementation}
In this section we go over the implementation of \name hardware and present design choices. The hardware is implemented based on the system design presented in \xref{sec:system} in fig.~\ref{fig:system} and components are chosen to meet our goal of designing a system that is suitable for IoT testbed implementation.

\subsection{MAC Layer}
We use MSP432P401R~\cite{} a 32-Bit Cortex M4F MCU with floating point unit to control two I/Q and backbone transceiver, communicate with baseband processor and managing power on the platform. This MCU has 64~kB RAM along with 256~kB FLASH memory for programming and provides huge flexibility for performing compression algorithms, complex MAC layer implementation of IoT protocols and sensor reading applications. It supports up to eight SPI, four UART and four I2C interfaces. It can operate at low frequencies, such as 128~kHz, as well as high frequencies up to 48~MHz. It has two 32-bits timers and more importantly it supports different low-power modes. As an example, it supports LPM4.5 mode which only consumes 25~nA current. These features make this MCU a suitable choice for \name to operate at low-power and also perfomr accurate duty-cycling.

\subsection{PHY Layer}
We use a low-power low-cost RF front-end, AT86RF215~\cite{ref:AT86RF215} from Microchip. We choose this chip as it is a highly integrated solution designed for operation in all of our target ISM bands (400~MHz, 900~MHz and 2.4~GHz ISM) and most importantly is one of the few commercial chips that also provides an I/Q output to allow for custom protocols and modulation. It provides all the blocks of the transceiver chain required between the antenna and digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, frequency synthesizer and voltage-controlled oscillator. This chip provides two RF ports for sub-Ghz and 2.4~GHz frequencies. Each RF port is access with balanced differential signal pairs. We use 0896BM15E0025E~\cite{} balun for sub-GHz RF port and 2450FB15A050E~\cite{} balun for 2.4~GHz RF port. The receiver chain passes signal through an LNA and then downconverts the signal using a mixer that is controlled by frequency synthesizer (PLL). This chip utilizes two PLLs for sub-GHz and 2.4~GHz transceivers. Both PLLs use a 26~MHz crystal as reference and they can synthesize any frequencies with the step of around 198~Hz. Then signal goes through an analog bandpass filter and then sampled by a 13-bits Sigma-Delta analog to digital convertor (ADC). On the transmitter side, the digital controller feeds I/Q samples to digital front-end. Then, the signal is sampled by a 13-bits digital to analog converter (DAC). This signal goes to a analog lowpass filter and upcoverts by the mixer which uses the same PLL. Finally, signal is amplified with internal power amplifier of this chip. Each RF port has one internal power amplifier (PA) that can output signal up to 14~dBm. This optimal power, however, is achieved when the RF port is matched to 50~$\ohm$ differential.


\textcolor{red}{Add noise figure, mention it provides two RF outputs (separate paths for sub GHz and 2.4 GHz, add specs for each internal block like LNA noise, PA efficiency, xx order filter, frequency synthesizer specs/step sizes. Mention what kind of architecture it is (e.g. superheterodyne, direct conversion etc.)What kind of clock input does it require?}

To exchange digitized I/Q baseband data between radio and baseband processing unit, it uses 64~MHz double data-rate low voltage differential signaling (LVDS).

\textcolor{red}{What is LVDS? Knowing nothing about the protocol I'm assuming it's low power and differential to reject common mode but how does it work? Add 1-2 sentences about it, if there's anything special you have to do for people who haven't heard of it.}

The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. This chip is capable of 13~bits ADC/DAC which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP~\cite{xxxx}. The current consumption of this chip is several tens of milli-ampere which is around an order of magnitude\textcolor{red}{lower than} the AD93XX series used in common SDR platfroms like USRP. Note that AD93XX series have higher sampling rate and frequency spectrum coverage which are not required considering our target application of IoT node implementation. Moreover, AD93XX series' price is at least 100\$ or even several hundreds of dollar depending on the version compared to our I/Q transceiver which is about 5\$. In conclusion, AT86RF215 has unique properties which are suitable for IoT node implementation.
% To receive I/Q samples from this radio, we need to interface with an FPGA with LVDS capability.
\textcolor{red}{Expand this: Additionally the rf front end chip can be set to implement different basic modulations (FSK OFDM etc). This allows us to bypass the FPGA entirely and enable greater power savings when implementing standard modulations while developing a MAC protocol.}

We use LFE5U-25F~\cite{} FPGA from Lattice Semiconductor for baseband processing which talks to the I/Q transceiver using LVDS interface. This FPGA has 24k logic units which is comparable to other common SDR platforms including XXX, XXX and XXX. We use a small form-factor of this FPGA on our design to decrease the platform physical size. Compared to FPGAs used in other existing platform this FPGA provides higher number of LUTs for the same cost. Since this is an SRAM-based FPGA, our design requires an external FLASH memory with XX~Mb size capable of storing multiple boots of this FPGA is included in the design. The FPGA talks to the flash with Quad SPI interface. 
\textcolor{red}{What happens when this goes into sleep mode and wakes up? Explain details of reprogramming (e.g. on wake up it reads from xxx memory address in flash for bitstream). How big is the bitstream to program the whole thing? Does this vary by design? You mention you can have multiple boots in this flash, can you use the MCU to select which one to load. One reason I can think of is mabye you want to do an experiment comparing two protocols one after another? Mention if this FPGA has IP cores for encryption algorithms or machine learning as well, just to add other features. Also what is the cost of the flash, does flash + fpga make the chip more expensive than others? For clocking does it have a PLL, does it get a reference from an external clock/crystal?}

Finally, to implement the RF section we use two RF paths, one for sub-GHz frequency bands and the other for 2.4~GHz frequency band. We use 2.4~GHz power amplifier ,SE2431L~\cite{}, and 900~MHz band power amplifier, SE2435L~\cite{}, to increase the maximum output power of our radios. Since both I/Q radio and backbone radio share the sub-GHz RF path, we use an ADG904~\cite{} RF switch to select between I/Q radio, RX and TX mode of LoRa radio.\textcolor{red}{Talk about bypass option, explain the switch network, how this handles all TX/RX switching.}

\subsection{Over-the-Air Update}
We employed LoRa protocol at 900~MHz for backbone communication. LoRa is a propriety protocol by Semtech which uses Chirp Spread Spectrum to increase the sensitivity and achieve long-ranges. In \name, we used SX1276 from Semtech that is designed for sub-GHz. Depending on the range, the update rate can be higher than xxx~kbps which is enough considering the compressed programming data of FPGA and MCU. For example with 30~dBm output power, $SF = xxx$, $BW = xxx$ and a 2~dBi antenna, we can achieve xxx~kbps at xxxx~km.

Over-the-air updates is enabled using 

Semtech SX1276~\cite{sx1276} as backbone radio talking to the access point by LoRa protocol\textcolor{red}{Why this particular Semtech chip? Explain for people who don't know LoRa is proprietary so it has to be Semtech, but also within their line of chips why this one? What kind of range can you get for different rates/SF with the PA (and mention that this would be when transmitting at xx power with a 2 dBi antenna)? Put some numbers}. Depending on the range, the update rate can be between 0.018~kbps to 37.5~kbps which is enough considering the compressed programming data of FPGA and MCU. In section~\xref{}, these rates and also compressed programming data volume is evaluated for different cases to measure the update duration.

\subsection{Power Management Unit}
\textcolor{red}{Add a paragraph about power, what voltages regulators etc. Can you use this to power an external sensor? What voltages do you have? What components can you turn off, what is always on?}

We integrate all components on a 6-layers FR-4 PCB with the dimension of $30mm\times50mm$ as shown in Fig.~\ref{fig:board}. Our board provides different sensor interfaces including SPI and I2C as external GPIOs for sensor reading applications.


\begin{figure}[t]
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_tx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{LoRa Modulator}}
        \label{fig:lora_tx_block}
    \end{subfigure}
	\begin{subfigure}{\linewidth}
	    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_rx_block.eps}
        \caption{\footnotesize{LoRa Demodulator}}
        \label{fig:lora_rx_block}
    \end{subfigure}
    \vskip -0.15in
    \caption{\footnotesize{LoRa implementation FPGA block diagrams.}}
    \label{fig:lora_blocks}
\end{figure}



==> impl-3.tex <==
%explain that we built the first version to show the proof of concept, evaluate radio and MAC capabilities. Then we design second version with new requirements such as larger FPGA, power managemnet, MCU that can handle multiple radios and etc.

\section{Hardware Implementation}
In this section we go over the implementation of \name hardware and present design choices. The hardware is implemented based on the system design presented in \xref{sec:system} in Fig.~\ref{fig:system} and components are chosen to meet our goal of designing a system that is suitable for IoT testbed implementation.

\subsection{MAC Layer}
We use MSP432P401R~\cite{} a 32-Bit Cortex M4F MCU with floating point unit to control two I/Q and backbone transceiver, communicate with baseband processor and managing power on the platform. This MCU has 64~kB RAM along with 256~kB FLASH memory for programming and provides huge flexibility for performing compression algorithms, complex MAC layer implementation of IoT protocols and sensor reading applications. It supports up to eight SPI, four UART and four I2C interfaces. It can operate at low frequencies, such as 128~kHz, as well as high frequencies up to 48~MHz. It has two 32-bits timers and more importantly it supports different low-power modes. As an example, it supports LPM4.5 mode which only consumes 25~nA current. These features make this MCU a suitable choice for \name to operate at low-power and also perfomr accurate duty-cycling.

\subsection{PHY Layer}
We use a low-power low-cost RF front-end, AT86RF215~\cite{ref:AT86RF215} from Microchip. We choose this chip as it is a highly integrated solution designed for operation in all of our target ISM bands (400~MHz, 900~MHz and 2.4~GHz ISM) and most importantly is one of the few commercial chips that also provides an I/Q output to allow for custom protocols and modulation. It provides all the blocks of the transceiver chain required between the antenna and digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, frequency synthesizer and voltage-controlled oscillator. This chip provides two RF ports for sub-Ghz and 2.4~GHz frequencies. Each RF port is access with balanced differential signal pairs. We use 0896BM15E0025E~\cite{} balun for sub-GHz RF port and 2450FB15A050E~\cite{} balun for 2.4~GHz RF port. The receiver chain passes signal through an LNA with noise figure of 4.5 and then downconverts the signal using a mixer that is controlled by frequency synthesizer (PLL). This chip utilizes two PLLs for sub-GHz and 2.4~GHz transceivers. Both PLLs use a shared 26~MHz crystal as reference and they can synthesize any frequencies with 198~Hz step size. Then signal goes through an analog bandpass filter and then sampled by a 13-bits Sigma-Delta analog to digital converter (ADC). On the transmitter side, the digital controller feeds I/Q samples to digital front-end. Then, the signal is sampled by a 13-bits digital to analog converter (DAC). This signal goes to a analog lowpass filter and upconverts by the mixer which uses the same PLL. Finally, signal is amplified with internal power amplifier. Each RF port has one internal power amplifier (PA) that can output signal up to 14~dBm. This optimal power, however, is achieved when the RF port is matched to 50~$\ohm$ differential.


\textcolor{red}{Add noise figure, mention it provides two RF outputs (separate paths for sub GHz and 2.4 GHz, add specs for each internal block like LNA noise, PA efficiency, xx order filter, frequency synthesizer specs/step sizes. Mention what kind of architecture it is (e.g. superheterodyne, direct conversion etc.)What kind of clock input does it require?}

To exchange digitized I/Q baseband data between radio and baseband processing unit, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). LVDS is a differential serial communication protocol which operates at low power and can run at very high speeds. This protocol transmits information as the difference between the voltages on a pair of wires. The two wire voltages are compared at the receiver. To achieve the best connection between two components with LVDS interface, the differential impedance between each pair should be 100~$\ohm$ which we consider when we design \name PCB.
% \textcolor{red}{What is LVDS? Knowing nothing about the protocol I'm assuming it's low power and differential to reject common mode but how does it work? Add 1-2 sentences about it, if there's anything special you have to do for people who haven't heard of it.}
The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. This chip is capable of 13~bits ADC/DAC which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP~\cite{xxxx}. \textcolor{red}{The current consumption of this chip is several tens of milli-ampere which is around an order of magnitude lower than the AD93XX series used in common SDR platfroms like USRP}. Note that AD93XX series have higher sampling rate and frequency spectrum coverage which are not required considering our target application of IoT node implementation. Moreover, AD93XX series' price is at least 100\$ or even several hundreds of dollar depending on the version compared to our I/Q transceiver which is about 5\$. In addition, our I/Q transceiver support various modulations such as MR-FSK, MR-OFDM, MR-O-QPSK and O-QPSK. This allows us to bypass the FPGA entirely and enable greater power savings when we use standard modulations supported by our transceiver. In conclusion, AT86RF215 has unique properties which are suitable for IoT node implementation.
% To receive I/Q samples from this radio, we need to interface with an FPGA with LVDS capability.
% \textcolor{red}{Expand this: Additionally the rf front end chip can be set to implement different basic modulations (FSK OFDM etc). This allows us to bypass the FPGA entirely and enable greater power savings when implementing standard modulations while developing a MAC protocol.}

We use LFE5U-25F~\cite{} FPGA from Lattice Semiconductor for baseband processing which talks to the I/Q transceiver using LVDS interface. This FPGA has 24k logic units which is comparable to other common SDR platforms including XXX, XXX and XXX. We use a small form-factor of this FPGA on our design to decrease the platform physical size. Compared to FPGAs used in other existing platform this FPGA provides higher number of LUTs for the same cost. Since this is an SRAM-based FPGA, our design requires an external FLASH memory with XX~Mb size capable of storing multiple boots of this FPGA which is included in the design. However, the price of the FLASH memory is not significant compare to the total price of the platform based on Table~\ref{tab:cost}. We use a 32~MHz clock oscillator as the reference clock for the FPGA. When I/Q radio operates in transmit mode, we use this clock reference to generate a 64~MHz clock reference for I/Q serial interface. However, when the I/Q operates in receive mode, we turn off this clock oscillator since the I/Q interface provides an clock reference and we use this reference for DSP operations in FPGA. 

Note: Explain the programming chain in detail.
\textcolor{red}{What happens when this goes into sleep mode and wakes up? Explain details of reprogramming (e.g. on wake up it reads from xxx memory address in flash for bitstream). How big is the bitstream to program the whole thing? Does this vary by design? You mention you can have multiple boots in this flash, can you use the MCU to select which one to load. One reason I can think of is mabye you want to do an experiment comparing two protocols one after another? Mention if this FPGA has IP cores for encryption algorithms or machine learning as well, just to add other features. Also what is the cost of the flash, does flash + fpga make the chip more expensive than others? For clocking does it have a PLL, does it get a reference from an external clock/crystal?}

Finally, to implement the RF section we use two RF paths, one for sub-GHz port and the other for 2.4~GHz port. Since the I/Q transceiver can only go up to 14~dBm output power~\cite{}, we use a power amplifier for each port. Since both I/Q radio and backbone radio share the sub-GHz RF port, we use an ADG904~\cite{} RF switch to select between different modes. There are three 900~MHz RF paths that share sub-GHz RF port including I/Q Transceiver RX/TX, backbone radio RX and backbone radio TX. We connect all these three paths to the RF switch and the output of the switch goes to sub-GHz PA. We use SE2435L~\cite{} PA for sub-GHz RF port. This PA has bypass capabilities, LNA and power amplifier. This means gives us flexibility in different operations. For example, in receive mode we can either pass the incoming signal through the LNA and then connect it to the transceiver of completely bypass the LNA and connect the signal directly. Similarly, in transmit operation we can pass the signal through the PA and amplify the signal or turn off the PA and just pass the signal directly to the antenna. We use similar PA, SE2431L~\cite{}, for 2.4~GHz RF port with identical capabilities. Since the 2.4~GHz RF port is only used by I/Q transceiver, it does not require an RF switch and we connect the PA directly to the I/Q transceiver. Using PA with bypass and sleep mode options gives us great capability to reduce power consumption in the case of lower power transmissions.

% \textcolor{red}{Talk about bypass option, explain the switch network, how this handles all TX/RX switching.}

\subsection{Over-the-Air Update}
We employed LoRa protocol at 900~MHz for backbone communication. LoRa is a propriety protocol by Semtech which uses Chirp Spread Spectrum (CSS) to increase the sensitivity and achieve long-ranges. In \name, we used SX1276 from Semtech that is designed for sub-GHz. Depending on the range, the update rate can be higher than xxx~kbps which is enough considering the compressed programming data of FPGA and MCU. For example with 30~dBm output power, $SF = xxx$, $BW = xxx$ and a 2~dBi antenna, we can achieve xxx~kbps at xxxx~km. In section~\xref{}, these rates and also compressed programming data volume is evaluated for different cases to measure the update duration.

\noindent{\bf Compression.} We compress the over-the-air updates before transmitting them to our testbed nodes. We use miniLZO compression algorithm presented in~\cite{compressionWebsite}. miniLZO is a very lightweight subset of the Lempel–Ziv–Oberhumer (LZO) compression algorithm. Current implementation of miniLZO requires memory allocation with the size of the uncompressed file. Since we have limited SRAM memory available on the MCU, we first divide the original FPGA programming file into smaller block size. Then we perform compression algorithm on each block separately and then we transmit these files to the \name end-node. On the \name platform, we use the same algorithm on MCU to decompresss each file and write it to the flash memory.

\subsection{Power Management Unit}
% \textcolor{red}{Add a paragraph about power, what voltages regulators etc. Can you use this to power an external sensor? What voltages do you have? What components can you turn off, what is always on?}
We implement power management unit with the purpose of having maximum control over all components' power supplies. Table~\ref{tab:voltages} shows various voltage requirements for each component in \name. To power the FPGA, we use three switching regulators to provide 1.1V, 1.8V and 2.5V. We use switching regulators since they have better efficiency and XXX compare to XXX. MCU requires 1.8V power supply which is in common with FPGA. Since we want to completely power of the FPGA, we cannot share V2 voltage domain with MCU. We use an XXX LDO to provide V4 voltage domain for MCU. The reason is XXX. We use a shared voltage domain for I/Q transceiver and backbone radio which we provide the power with a programmable switch regulator, Semtech SC195ULTRT~\cite{}. Using this voltage regulator, we are able to adjust the radio voltage based on the radio mode and maximum power output. Therefore, we can optimize power consumption of the radio in different modes. We power the sub-GHz PA with another switching regulator that provides V6 voltage domain. Similarly, we use a separate voltage regulator for analog voltage power supply of the 2.4~GHz PA and we share its digital power supply with V2 voltage domain. Finally, we share power supplies for FLASH memory and Micro SD memory with other power domain since their functionalities has overlap with other components and they are not power hungry components.



We integrate all components on a 6-layers FR-4 PCB with the dimension of $30mm\times50mm$ as shown in Fig.~\ref{fig:board}. Our board provides different sensor interfaces including SPI and I2C as external GPIOs for sensor reading applications.


\begin{table}[H]
    \centering
    \caption{\footnotesize{\bf Voltage domains in \name.}}
    \vskip -0.15 in
    \begin{tabular}{|c|c|c|}
         \hline
         Component & Voltage & Voltage Domain\\
         \hline
         FPGA & 1.1V, 1.8V, 2.5V & V1, V2, V3\\
         \hline
         MCU & 1.8V & V4\\
         \hline
         I/Q Transceiver & 1.8V< V5 <3.6V & V5\\
         \hline
         Backbone Radio & 1.8V< V5 <3.6V & V5\\
         \hline
         sub-GHz PA & 4.0V & V6\\
         \hline
         2.4~GHz PA & 1.8V, 3.0V & V2, V7\\
         \hline
         FLASH Memory & 1.8V & V2\\
         \hline
         Micro SD Memory& 3.0V & V7\\
         \hline
    \end{tabular}
    \label{tab:voltages}
\end{table}

% \begin{figure}[t]
%     \begin{subfigure}{\linewidth}
%     \centering
%         \includegraphics[width=1\linewidth]{figs/block_diagram/lora_tx_block.eps}
%         \vskip -0.1in
%         \caption{\footnotesize{LoRa Modulator}}
%         \label{fig:lora_tx_block}
%     \end{subfigure}
% 	\begin{subfigure}{\linewidth}
% 	    \centering
%         \includegraphics[width=1\linewidth]{figs/block_diagram/lora_rx_block.eps}
%         \caption{\footnotesize{LoRa Demodulator}}
%         \label{fig:lora_rx_block}
%     \end{subfigure}
%     \vskip -0.15in
%     \caption{\footnotesize{LoRa implementation FPGA block diagrams.}}
%     \label{fig:lora_blocks}
% \end{figure}



==> impl-5.tex <==
\vspace{-0.05 in}
\section{System Implementation}
In this section, we explain the operation of each of the above blocks in detail. To do this we walk through the technical challenges of reading the digitized signal into the FPGA at the full sampling rate of the radio output and into internal memory followed by saving them to an SD card. Next we give an end to end description of our over-the-air update system including the access point communication protocol, compression and reprogramming sequence.

%In order to receive samples he interfaces between each of the components described above as well as their internal software blocks. We 

%We first explain our I/Q interface with I/Q radio. Then we explain our memory interface and finally we show steps of our over-the-air system to update each \name node in the network.

\subsection{Reading and Writing I/Q Samples}
The AT86RF215 radio chipset samples baseband signals at a rate of 4~MHz with a 13~bit resolution for both I and Q. Operating at the full rate therefore requires an interface which can support a throughput of over 100~Mbps without consuming a large amount of power to meet our design objectives. To do this we use a standard called low-voltage differential signaling (LVDS)~\cite{XXX} which is provided by AT86RF215. LVDS is a high-speed digital interface that reduces power by using lower voltage signals but maintains good SNR by sending data over two differential lines to reduce common mode noise. 


\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/iq_structure.eps}
	\vskip -0.15 in
	\caption{\footnotesize{I/Q word structure used in I/Q interface.}}
	\label{fig:iq_structure}
	\vskip -0.2 in
\end{figure}

\noindent{\bf Receiving serial I/Q data.}
Our system communicates by LVDS to the FPGA in synchronous serial mode to transfer I/Q data with a physical interface consisting of 2 pairs of differential I/O lines, one pair for data and one for clock. The radio outputs 32-bit serial data words at 4~Mwords/s using the format in Fig.~\ref{fig:iq_structure}. Each data word starts with the $I\_{SYNC}$ pattern which indicates the start of the $I$ sample which we use for synchronization. Next, it has 13 bits $I\_{Data}$ followed by a control bit. The same format follows for $Q$, beginning with a synchronization pattern $Q\_{SYNC}$ and then 13 bits for $Q\_{Data}$ and the final control bit. The required 128~Mbps data rate is achieved using a 64~MHz double data rate clock provided by the radio, meaning that the data should be sampled at both the rising and falling edges of the clock signal. We implement an I/Q deserializer on the FPGA module to read the data. The deserializer samples the data signal at both the rising and falling edges of the clock, uses the $I\_{SYNC}$ and $Q\_{SYNC}$ to detect the beginning of the data fields and loads the $I$ and $Q$ values into 13~b registers to allow for parallel processing.
 
\noindent{\bf Transmitting I/Q samples.} In TX mode we need to do the opposite of the above sequence to convert from the parallel representation on the FPGA to a serialized LVDS stream. To do this, we use the FPGA's onboard PLL to generate the 64~MHz clock signal. Next to create our double data rate output signal that varies on both positive and negative edges of this clock signal, we use a dual-edge D flip-flop design~\cite{hildebrandt2011pseudo} resulting in the desired 128~Mbps data rate. We use this to generate the same I/Q word structure described above.

\subsection{RF Interfaces} 
Our goal in designing \name is supporting 900~MHz and 2.4~GHz ISM bands. AT86RF215 provides differential RF signal for both 900~MHz and 2.4~GHz and has integrated TX/RX switch for both paths. On the 2.4~GHz side, the differential signal is transformed to single-ended using 2450FB15A050E~\cite{24balun} balun and then fed to SKY66112~\cite{SKY66112} front-end which has LNA and PA. The LNA and PA of SKY66112 can be bypassed if needed. Finally, after passing through matching network, the 2.4~GHz signal is connected to SMA. On the 900~MHz side, the differential signal of the AT86RF215 is connected to 0896BM15E0025E~\cite{900balun} to get single-ended signal. 
There are three signal lines that need to share the 900~MHz path to the antenna. Backbone radio's two separate RF paths for transmit and receive and AT86RF215's 900~MHz single-ended signal. We choose between these three using ADG904~\cite{adg904} SP4T RF switch. The single port side of the switch is connected to the SE2435L~\cite{SE2435L} 900~MHz front-end which similar to the 2.4~GHz front-end has PA and LNA that can be bypassed.

\subsection{Control and Sensor Interfaces} 
As mentioned previously, MCU is the central controller and controls all the components of the system. It talks to I/Q radio, backbone radio, FPGA and Flash memory through SPI. Moreover, it has control signals for FPGA programming, 900~MHz and 2.4~GHz front-end modules, RF switch and voltage regulators. To enable testing of different application scenarios, \name is utilized with common sensor interfaces like ADC, I2C and SPI. These interfaces are handled by the MCU.

\subsection{Memory Interfaces}
After reading the raw data from the LVDS lines using the I/Q deserializer described above, the next step is to store the samples into a FIFO buffer implemented using the FPGA's embedded SRAM to prepare them for processing by FPGA. We implement a simple memory controller to write data to the FIFO as shown in Fig.~\ref{fig:memory_block} which generates the memory control signals and writes a full data word on each cycle. The embedded memory can run at rates significantly greater than 4~MHz meaning it is not a limiting factor for real time processing. The SRAM alone can buffer up to 126 kB, and additional embedded memory options such as DRAM could allow for larger buffer sizes as well.

The data stored in the FIFO can then be sent to signal processing blocks to implement filters, cryptographic functions, etc. or to non-volatile flash memory. For flash we use microSD cards which support two modes: native SD mode and standard SPI mode. In native SD mode, we can use up to 4 bit parallel data lines to read/write data to/from the microSD card. This mode supports a higher data rate compare to the SPI mode which only supports 1 bit serial interface. However, we implement SPI mode since it supports the data rate of XX~Mbps which our system requires to write data in real time and has a simpler implementation. This allows us to re-use the same, simpler SPI block for multiple functions and save resources on the FPGA.


\subsection{Over-the-Air Update}
In this section, we explain the operation of \name's over-the-air system. This system requires addressing multiple challenges including a protocol for interacting with the centralized access point to ensure each node receives the full bit stream, as well as minimizing transmission length to reduce network downtime. First, we explain how we prepare updates on the access point and handle transmissions to each node. Then, we explain the details of storing the update data and reprogramming the system.

\noindent{\bf OTA AP and MAC Protocol.} To control a network of multiple \name devices in a testbed, we use a single centralized access point with a LoRa radio to communicate with each node. In order to propagate updates throughout a testbed network or to specific \name nodes, we design a MAC layer system over the LoRa physical layer protocol. In order to avoid the chance of corrupted firmware due to packet loss during the update, and considering each update takes only XXX~s as shown in Fig.~\ref{xxx}, our access point updates each \name node individually.

First, the AP sends an update request as a LoRa packet with a specific device ID indicating the node to be updated in the payload. Upon processing this packet and detecting its ID, the \name node switches into update mode and sends a ready message to the access point. Then, the AP transmits the firmware update as a series of LoRa packets with sequence numbers. Upon receiving each packet, the \name node checks the sequence number and CRC. For a correct packet it writes the data to its flash memory and transmits an ACK to indicate correct reception. In the case of failure, the AP retransmits the corrupted packet. After the AP has sent all the firmware data, it sends a final packet indicating the end of firmware update, and the \name node switch its state to normal operation upon receiving this.


\noindent{\bf Compressing and decompressing the bitstream.} Our system uses compression to minimize the amount of data sent in each update, however this compression must be compatible with the resources available on \name. We choose the miniLZO compression algorithm~\cite{miniLZO}, which is a lightweight subset of Lempel–Ziv–Oberhumer (LZO) compression algorithm. Our current implementation of miniLZO decompression algorithm only requires a memory allocation equal to the size of the uncompressed data. We perform compression on the AP. The compression ratio of bitstream file varies based on the content of the bitstream. In worst case scenario, the compressed file has exactly the same size of the original file which is the lowest compression ratio. In this case, we need memory allocation on the MCU on \name with the size of original bitstream file. This is around XXX~kB SRAM memory which we cannot afford on a low-cost MCU. To address this, we first divide the original update file into blocks of 20~kB that will fit in the MCU memory. Then we compress each block separately and transmit them to the \name node one by one. Considering the LoRa radio takes more power than the MCU, we immediately write the data to our dedicated programming flash memory using an SPI interface.

After receiving all the data we turn off the LoRa radio and decompress the data. First, we allocate memory on SRAM on the MCU equal to the block size and load a block of data from flash. Next, we perform decompression and write the data in the allocated SRAM memory. Finally, we write the decompressed data back to the flash beginning at the corresponding address of the programming boot file. We repeat these steps until we decompress the full firmware update.


\noindent{\bf Programming.} After storing uncompressed programming data in flash memory, we perform FPGA programming. We use the MCU to set the FPGA into programming mode. When FPGA switches to programming mode, it automatically reads programming data directly from the flash memory using a quad SPI interface and programs itself. Reading from flash using quad SPI, which can run up to 62~Mbps, achieves programming times of xx~ms which is similar to FPGAs with embedded flash memory and results in minimal system down time. After programming is complete, it resumes operation and begins running the new firmware.

%Master quad SPI can achieve up to 62~Mbps data rate. Using quad SPI for programming is more necessary when FPGA wakes up from sleep mode. Since our FPGA is SRAM-based and does not include internal flash memory for programming, it requires external flash memory. When FPGA wakes up from sleep mode, it automatically program itself by reading programming file from external flash memory. In this case, using quad SPI reduces the programming time and it becomes similar to Flash-based FPGAs programming time.

==> intro-0.tex <==
Software defined radios (SDR) has been an essential part of research community and industry marketfor the past years. In 2011, Ettus Research released USRP N200 which was one the most advancedSDR design by the time.  Since early releases of SDR platform, most companies have focusedon building SDR platform which runs at high sampling rates, support large bandwidths at hugefrequency spectrum [?,?]. Recent SDR platforms such as bladeRF 2.0 micro uses expensive radiofrequency (RF) front-end which is optimized in noise figure for a large bandwidth. Conventionalgoals of SDR platform led to power-hungry SDR designs that is bulky and expensive. Today, theadvent of Internet of Things (IoT) and usage of various IoT protocols across the world has led tonew research problems: multi-technology SDR platform that can support various IoT protocols atlow cost. A naiveXX design for such system is to build gateways that includes radios for differentprotocols. Since IoT technologies are growing fast, this approach is not sustainable for researchcommunity. In addition, research projects in IoT domain need to perform network evaluation atlarge-scale with wide-area deployment. Therefore, we are looking for creating an SDR platformwhich is can be battery-powered, supports multiple IoT protocols at the same time and benefits frommultiple frequency bands including 900 MHz and 2.4 GHz ISM bands.

\section{Introduction}

%%para 1
% history of SDR

%%para 2
%%issues with previous platforms

%%%para 3
% motivation

%para 4
% more details of our motivation

%para 5
% challenges

%para 6
% solutions

%para 7
% Demonstrated Applications


%par 8
% Contribution

==> intro-1.tex <==
\section{Introduction}
Recent years have seen significant work on wireless communication protocols for IoT endpoint devices. There is currently no de-facto communication standard for these devices as protocols such as LoRa, Sigfox and NB-IoT have only been introduced in the past few years; this has led to a number of works in this space such as xxx, xxx, xxx, xxx.   

Despite the interest in developing solutions for IoT endpoints, the research community is limited by the lack of tools to develop and evaluate these protocols. While commercial chipsets implement a single IoT protocol, they aim to provide a turnkey solution for products and offer little to no flexibility for modifying or improving any layer of the network stack and eliminate any possibility of clean slate designs. Moreover, some implementations such as LoRa are proprietary and even details of the standard are not publicly available. Considering the rapid growth of IoT technologies, using one or a combination of inflexible, single protocol chipsets to develop dedicated hardware for individual projects is not sustainable for research community.

In contrast software defined radios (SDRs) solve this problem by offering access to the raw radio signals. SDR platforms such as the USRP have become an essential tool in the wireless research community enabling diverse works ranging from WiFi and LTE access points to backscatter and localization techniques; however we observe that a focus on achieving high bandwidth and wide spectrum coverage leads SDR platforms to be bulky, expensive, and power hungry. While these high performance specs are ideal for development of access points, existing SDR platforms do not meet the following three constraints unique to \textit{IoT endpoints}:

\squishlist
    \item {\bf Computation.}
    An IoT endpoint should be standalone and include onboard computation to run its basic functions such as periodically waking up from sleep mode to sample a sensor and process data, transmit a message, and go to back to sleep mode. The need for many SDR platforms to be tethered via USB or Ethernet to a laptop is acceptable for use as a gateway or access point but makes them infeasible for use as IoT nodes.
    \item {\bf Power consumption.}
    IoT endpoints are often deployed in locations without dedicated power infrastructure and must be battery powered. Unlike plugged in access points, low power consumption is a paramount concern and existing SDR platforms often consume xx~W.
    \item {\bf Cost and scalability.}
    Many real world IoT deployments require a large number of nodes, and studying the complex networking challenges requires a scalable testbed. This adds the additional constraint of requiring individual nodes to be low cost.
\squishend

In this work we present \name: an SDR platform specifically tailored to the needs of IoT endpoint research. We exploit recent trends that have produced small, low power radios, microcontrollers, and FPGAs to develop our SDR platform. Specifically \name has the following capabilities:

\squishlist
    \item {\it Raw samples.} Our platform outputs raw I/Q samples which enable phase based applications like localization and can be processed in real time or stored to an onboard SD card for offline processing.
    \item {\it Low power.} The whole platform consumes xx~mW in transmit mode and only xx~mW in receive mode.
    \item {\it Small form factor.} The total size of our platform is xx $\times$ xx cm.
    \item {\it Frequency bands.} Our platform covers both the 900~MHz and 2.4~GHz ISM bands allowing for use with a variety of IoT protocols.
    \item {\it Transmit/Receive capability.} Despite the small size and low power, it can transmit up to xx~dBm and has a receiver noise figure of only xx~dB.
    \item {\it Sensitivity.} This platform can achieve the sensitivity of commercial LoRa chipsets allowing for long range operation.
    \item {\it Bandwidth.} The xx~MHz bandwidth is sufficient for a variety of IoT protocols.
    \item {\it Computation/programmability.} An included FPGA and microcontroller allow for standalone operation and flexibility to implement custom algorithms onboard.
    \item {\it Sensor inputs} The microntroller allows for analog and digital sensor inputs, enabling a complete plug and play IoT sensor node solution.
\squishend

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/3_platform_power/platform_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Radio Power Consumption.} We show radio power consumption for each platform. We normalized TX power consumption for output equals to 14~dBm.\newline
    **RTL-SDR does not support transmitter mode.}}
	\label{fig:platform_power}
    \vskip -0.15in
\end{figure}

To demonstrate the functionality of our platform we further present an application scenario: distributed localization and mapping of sensor nodes. In We use our platform to propose the first solution that allows a network of IoT nodes to \textit{localize each other} without the need for a central gateway or access point. 
[TODO insert description of algorithm]

We summarize our contributions below:
\begin{itemize}
    \item We develop the first SDR platform tailored to the needs of IoT endpoints. Our platform is capable of implementing numerous IoT protocols, gives access to raw samples, and achieves low power cost and size needed for large scale deployments.
    \item We extensively characterize and evaluate our platform to show its capabilities including implementations of LoRa and XX as well as sensitivity and synchronization experiments.
    \item We present a novel distributed localization system capable of localizing IoT nodes without the need for a centralized access point.
\end{itemize}

==> intro-2.tex <==
\section{Introduction}
The grand vision for Internet of Things (IoT) technologies is to extend internet connectivity to everyday physical objects across homes, vehicles, hospitals, farms, factories and more. The diversity of needs in each of these different sectors has led to significant work on wireless communication protocols for IoT endpoint devices in recent years; however there is currently no de-facto communication standard as protocols like LoRa, Sigfox, NB-IoT and others compete for market share.

%%%problems
This leads to a host of problems for researchers, consumers, and chipset manufacturers alike. On the one hand, chipset manufacturers are incentivized to produce proprietary protocols for a specific industry offering little to no flexibility for modifying or improving \textcolor{red}{any layer of the network stack -> LoRa MAC can be changed} or interacting with other technologies; however customers must then bet on the long term success of a particular IoT technology, or attempt to interconnect them. \textcolor{red}{ Similarly, while this presents an opportunity for researchers to develop novel solutions the lack of flexibility stifles innovation.} Additionally, while recent works in the networking community have sought to solve problems in the IoT space~\cite{xxx,xxx,xxx}, their scope and potential for commercial adoption is limited by the lack of a large scale testbed for real-world deployments.

%%iot lab
Similar to how PlanetLab~\cite{planetlab} presented a novel tool for developing disruptive technologies for the Internet, a large scale flexible testbed of IoT nodes would open the door for researchers to address the \textcolor{red}{ outstanding challenges} outlined above. In this paper we take the first step towards building such a testbed by developing \name, a platform for prototyping IoT endpoint nodes.

In order to allow for flexibility, \name uses a software defined radio (SDR) which offers access to the raw radio signals. Existing SDR platforms such as the USRP have become an essential tool in the wireless research community enabling diverse works ranging from WiFi and LTE access points to backscatter and localization techniques; however we observe that a focus on achieving high bandwidth and wide spectrum coverage leads existing SDR platforms to be bulky, expensive, and power hungry. While these high performance specs are ideal for development of access points, existing SDR platforms do not meet the following three constraints unique to \textit{IoT endpoints}:

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/3_platform_power/platform_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{Radio power consumption for each platform. We normalized TX power consumption for output power of 14~dBm.\newline
    **GalioT does not support transmitter mode.}}
	\label{fig:platform_power}
    \vskip -0.2in
\end{figure}

\squishlist
    \item {\bf Computation.}
    An IoT endpoint should be standalone and include onboard computation to run its basic functions such as periodically waking up from sleep mode to sample a sensor and process data, transmit a message, and go to back to sleep mode. The need for many SDR platforms to be tethered via USB or Ethernet to a laptop is acceptable for use as a gateway or access point but makes them infeasible for use as IoT nodes.
    \item {\bf Power consumption.}
    IoT endpoints are often deployed in locations without dedicated power infrastructure and must be battery powered. Unlike plugged in access points, low power consumption is a paramount concern and existing SDR platforms often consume xx~W.
    \item {\bf Cost and scalability.}
    Solving real world problems for IoT deployments requires a large number of nodes, and studying the complex networking challenges requires a scalable testbed. This adds the additional constraint of requiring individual nodes to be low cost.
\squishend

In contrast \name is an SDR platform specifically tailored to the needs of IoT endpoint research. We exploit recent trends that have produced small, low power radios, microcontrollers, and FPGAs to develop our SDR platform. Specifically \name has the following capabilities:

\squishlist
    \item {\it Raw samples.} Our platform outputs raw I/Q samples which enable phase based applications like localization and can be processed in real time or stored to an onboard SD card for offline processing.
    \item {\it Low power.} The whole platform consumes xx~mW in transmit mode and only xx~mW in receive mode.
    \item {\it Small form factor.} The total size of our platform is xx $\times$ xx cm.
    \item {\it Frequency bands.} Our platform covers both the 900~MHz and 2.4~GHz ISM bands allowing for use with a variety of IoT protocols.
    \item {\it Transmit/Receive capability.} Despite the small size and low power, it can transmit up to xx~dBm and has a receiver noise figure of only xx~dB.
    \item {\it Sensitivity.} This platform can achieve the sensitivity of commercial LoRa chipsets allowing for long range operation.
    \item {\it Bandwidth.} The xx~MHz bandwidth is sufficient for a variety of IoT protocols.
    \item {\it Computation/programmability.} An included FPGA and microcontroller allow for standalone operation and flexibility to implement custom algorithms onboard.
    \item {\it Sensor inputs} The microntroller allows for analog and digital sensor inputs, enabling a complete plug and play IoT sensor node solution.
\squishend





We summarize our contributions below:
\begin{itemize}
    \item We develop the first SDR platform tailored to the needs of IoT endpoints. Our platform is capable of implementing numerous IoT protocols, gives access to raw samples, and achieves low power cost and size needed for large scale deployments.
    \item We extensively characterize and evaluate our platform to show it is capable of implementing existing protocols such as LoRa and XX to as a starting point for researchers to develop custom solutions.
\end{itemize}

==> intro-3.tex <==
\section{Introduction}
%some background on IoT space
The grand vision for Internet of Things (IoT) technologies is to extend internet connectivity to everyday physical objects across homes, vehicles, hospitals, farms, factories and more. The diversity of needs in each of these different sectors has led to significant work on wireless communication protocols for IoT endpoint devices in recent years; however there is currently no de-facto communication standard as protocols like LoRa, Sigfox, NB-IoT and others compete for market share.

%%%problems: -ASICs are not flexible -There is no IoT testbed available 
This leads to a host of problems for researchers, consumers, and chipset manufacturers alike. On the one hand, chipset manufacturers are incentivized to produce proprietary protocols for a specific industry offering little to no flexibility for modifying or improving PHY or MAC layer or interacting with other technologies; however customers must then bet on the long term success of a particular IoT technology, or attempt to interconnect them. \textcolor{red}{ Similarly, while this presents an opportunity for researchers to develop novel solutions the lack of flexibility stifles innovation.} Additionally, while recent works in the networking community have sought to solve problems in the IoT space~\cite{xxx,xxx,xxx}, their scope and potential for commercial adoption is limited by the lack of a large scale testbed for real-world deployments.

%%iot lab
%We need something like PlanetLab, called IoTLab, to be used as a testbed.=> we need something flexible like SDR
%it should end with the need for software defined radio
Similar to how PlanetLab~\cite{planetlab} presented a novel tool for developing disruptive technologies for the Internet, a large scale flexible testbed of IoT nodes would open the door for researchers to address the outstanding challenges outlined above. As shown in fig.~\ref{fig:vision}, our vision is to build a testbed to enable large-scale innovation in IoT domain. This testbed would have hundreds and thousands IoT endpoints distributed around a large area talking to each other or an access point. These endpoints should be flexible to be able to be programmed with different PHY and MAC layer codes so that users can test their customized protocols. In this paper we take the first step towards building such a testbed by developing \name, a platform for prototyping IoT nodes. 

%%what are the requirements of the SDR used in this testbed based on the requirements of the testbed and what is the issue with the current available setup

In order to allow for flexibility, \name uses a software defined radio (SDR) architecture which offers access to the raw radio signals. Existing SDR platforms such as the USRP have become an essential tool in the wireless research community enabling diverse works ranging from WiFi and LTE access points to backscatter and localization techniques; however we observe that a focus on achieving high bandwidth and wide spectrum coverage leads these platforms to be bulky, expensive, and power hungry. While these high performance specs are suitable for development of access points, existing SDR platforms do not meet the following constraints unique to IoT node development platform:

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/map.eps}
    \vskip -0.1in
    \caption{\footnotesize{Our vision is to build an IoT testbed including hundreds of IoT endpoints spanning across a large area.}}
	\label{fig:vision}
    \vskip -0.2in
\end{figure}

%Explain what are the requirements of the SDR to be used in an IoT testbed
\squishlist
    \item {\bf Cost and scalability.}
    Solving real world problems for IoT deployments requires a large number of nodes, and studying the complex networking challenges requires a scalable testbed. This imposes the constraint of requiring individual nodes to be low cost.
    
    \item {\bf Standalone operation.}
    An IoT endpoint should be standalone and include onboard computation to run its basic functions such as periodically waking up from sleep mode to sample a sensor and process data, transmit a message, and go back to sleep mode. Although, existing SDR platform's FPGA are capable of reprogramming, it is not practical and efficient to develop such functions on them and in most cases they are tethered via USB or Ethernet to a laptop which is acceptable for use as a gateway or access point but makes them infeasible for use as IoT nodes.
    
    \item {\bf Over-the-air (OTA) update.}
    In the described testbed, there are hundreds and thousands of flexible IoT nodes which are deployed across a large area. Existing SDR platforms are lack of wireless backbone support to update PHY and MAC layer implementations on the IoT endpoint.

    \item {\bf Power consumption.}
    IoT endpoints are often deployed in locations without dedicated power infrastructure and must be battery powered. Unlike plugged in access points, low power consumption is a paramount concern and existing SDR platforms often consume several watts of power. Moreover, they are not capable of being duty-cycled which results in significantly short battery life times.
    
    \item {\bf \textcolor{red}{Duty-cycling.}}

\squishend


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/3_platform_power/platform_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{Radio power consumption for each platform. We normalized TX power consumption for output power of 14~dBm.\newline
    **GalioT does not support transmitter mode.}}
	\label{fig:platform_power}
    \vskip -0.2in
\end{figure}

In contrast \name is an SDR platform specifically tailored to the needs of IoT endpoint research. We exploit recent trends that have produced small, low power radios, microcontrollers, and FPGAs to develop our SDR platform. Specifically \name has the following capabilities and characteristics:
\squishlist
    \item {\it Over-the-air update.} We enable over-the-air update functionality on \name by using an extra backbone radio with LoRa protocol.
    \item {\it Granular power management.} We design power distribution in \name to have full control over all power sources and optimize power consumption in each operation mode.
    \item {\it Raw samples.} Our platform outputs raw I/Q samples which enable phase based applications like localization and can be processed in real time or stored to an onboard mico SD card for offline processing.
    \item {\it Low power.} The whole platform consumes xx~mW in transmit mode and only xx~mW in receive mode.
    % \name can operate for more than a year with 0.1\% duty-cycling on 1000mAh 3V battery. XXXX
    \item {\it Small form factor.} The total size of our platform is $3\times5~cm$.
    \item {\it Frequency bands.} Our platform covers both the 900~MHz and 2.4~GHz ISM bands allowing for use with a variety of IoT protocols.
    \item {\it Transmit/Receive capability.} Despite the small size and low power, it can transmit up to xx~dBm and has a receiver noise figure of only 5~dB.
    \item {\it Sensitivity.} This platform can achieve the sensitivity of commercial LoRa chipsets allowing for long range operation.
    \item {\it Bandwidth.} The 4~MHz bandwidth is sufficient for a variety of IoT protocols.
    \item {\it Computation/programmability.} An included FPGA and microcontroller allow for standalone operation and flexibility to implement custom algorithms onboard.
    \item {\it Sensor inputs.} The microntroller allows for analog and digital sensor inputs, enabling a complete plug and play IoT sensor node solution.
\squishend




We summarize our contributions below:
\begin{itemize}
    \item We develop the first SDR platform tailored to implement the IoT testbed. Our platform is low cost, capable of implementing numerous IoT protocols both in 900~MHz and 2.4~GHz ISM bands, have large computation resources to do various on-board processing, modular power management and can be duty-cycled and more importantly its codes can be updated through a remote access point.
    \item We extensively characterize and evaluate our platform. To show the flexibility of \name, two IoT protocols in two frequency bands of 900~MHz and 2.4~GHz is implemented. The power consumption is measured in multiple implementation scenarios. Over-the-air update is characterized for multiple different programming data and different ranges of an access point and platform and update times are measured. Moreover, we show cost breakdown for building 1000 \name.
\end{itemize}




==> intro-4.tex <==
\section{Introduction}
Recent years have seen development on wireless protocols for Internet of Things (IoT) devices. In addition to longtime standards such as Bluetooth and Zigbee, a number of other protocols such as LoRa, Sigfox, NB-IoT, LTE-M, and 802.11h have been developed and due to the lack of a de-facto standard this space remains an active area of development for both industry and academia. The rapid advances in this space however presents practical challenge for researchers: each of these protocols requires a dedicated radio chipset to evaluate, and these proprietary solutions often leave little room for protocol modification. The academic community is therefore severely handicapped by the lack of a \textit{flexible} platform as even a complex multi-radio prototype cannot adapt to evaluate new protocols or even customize existing solutions. The current ecosystem therefore discourages researchers from investigating the important questions that arise when scaling up IoT networks, and more importantly taking a systematic approach to develop new protocols from the ground up.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/map.eps}
%     \vskip -0.1in
%     \caption{\footnotesize{Our vision is to build an IoT testbed including hundreds of IoT endpoints spanning across a large area.}}
% 	\label{fig:vision}
%     \vskip -0.2in
% \end{figure}

%protocols for IoT remain an
%researchers are handicapped
%many protocols and active development
%recent interest
%new protocol every year
%802.11ah sigfox, nbiot lte-m, lora, ble zigbee
%each protocol is proprietary
%need a new testbed for each protocol
%more imprortantly  taking more systematic approach
%academic community is handicapped and can't develop own protocols

Ideally, we would like a large scale network testbed with the flexibility to run \textit{any} IoT protocol and push changes using simple over-the-air software updates. Fig~\ref{fig:vision} illustrates this vision of a large area network testbed with hundreds of endpoints across a city. This would allow for side-by-side performance comparisons to investigate the trade offs of existing standards and showcase the advantages of an entirely new custom solution. Moreover, to make such a system representative of real-world deployments, we would like for the individual network nodes to model the constraints of IoT endpoints. Specifically, these devices should be able to run on a battery, have appropriate power controls and options to duty cycle transmissions, and interfaces to connect sensors like real IoT nodes. The ability to run these endpoints on batteries would also allow for flexibility of deployment in spaces without dedicated power access, or even on mobile devices.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{figs/map.eps}
%     \vskip -0.1in
%     \caption{\footnotesize{Our vision is to build an IoT testbed including hundreds of IoT endpoints spanning across a large area.}}
% 	\label{fig:vision}
%     \vskip -0.2in
% \end{figure}

Realizing this vision however is limited by the hardware platforms that exist today for prototyping IoT systems. Specifically, such a system requires a software defined radio (SDR) to maximize flexibility for implementing different IoT protocols, but there is currently no SDR platform that meets all of our requirements. If we look at commercially available SDR systems, we notice that they are expensive, consume large amounts of power, require wired infrastructure and often a dedicated computer, and a wired backbone for updates. Said differently, devices on the market focus on achieving high performance in terms of bandwidth, etc. because they are tailored to the needs of gateway style devices and there is currently no SDR platform that serves the unique needs of IoT endpoints.

%ideally large network testbed
%wirelessly update, small modifications
%test performance, etc
%custom protocols
%within constraints of endpoint

%need development platform
%while there has been work on access points SDRs/gateways, there is no sdr for Iot endpoints
%everything that exists is high power, most require wired infrastructure
%need wired backbone to update
%cost


\begin{figure}[t]
    \centering
	\includegraphics[width=0.7\linewidth]{./figs/foo.eps}
	\vskip -0.2 in
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
	\vskip -0.2 in
\end{figure}


Driven by a need for such a platform in our own research, we build \name.
\name is the first SDR platform specifically tailored to the needs of IoT endpoint research. Our SDR platform provides an entirely standalone solution that incorporates a radio front end, FPGA and microcontroller for custom processing, wireless update capabilities, a microSD card interface for storage, and a highly granular power managment options to enable battery powered operation. It is capable of transmitting and receiving in both the 900~MHz and 2.4~GHz ISM bands, supports 4~MHz of bandwidth, and can achieve the sensitivity of commercial solutions such as LoRa chipsets. Additionally it includes a variety of analog and digital I/O options for connecting sensors and measures only $3\times5~cm$.



We exploit recent trends that have produced small, low power radios, microcontrollers, and FPGAs to develop our SDR platform, however building this platform required a number of careful design decisions and multiple engineering challenges:
\squishlist
    \item {\bf Hardware architecture.} Achieving a small form-factor, low power design requires a minimalist design approach to identify only the key system requirements. We analyze the priorities for IoT endpoints and then design and build a complete system to meet these needs.
    \item {\bf OTA update system.} Enabling a truly scalable system requires a wireless updates, however also introduces the challenges of how to communicate these robustly to each device in the network while minimizing downtime. We address this by using a dedicated LoRa backbone subsystem complete with a MAC protocol and compression.
    \item {\bf Power management.} Fully optimizing power consumption requires shutting down parts of the system when not in use. This presents a design trade off however between the complexity of being able to toggle each power source on and off and the cost of additional circuitry to do so. We address this challenge by grouping components into a small number of controllable power domains.
\squishend


Our final prototype of \name measures $3\times5~cm$, and costs \$xx to produce at volumes of xxx or more, and we perform detailed measurements of power consumption showing it consumes only XX~uW in its lowest power sleep mode. Additionally, we measure the performance of our over-the-air update system for and show it requires only xx~ms of network downtime at ranges as far as xx~m.

We further evaluate the performance of our \name by presenting case studies of two common protocols: LoRa and Bluetooth. We show that we can implement a LoRa modulator and demodulator using only xx\% of the FPGA resources and can achieve a sensitvity of -xxx~dBm which is the same as the SXxx LoRa chipset. We then evaluate the power consumption of generating LoRa transmissions versus output power and show it is as low as xxx for 14~dBm output. Additionally we demonstrate a MAC protocol on our MCU which is compatible with the existing Things Network and show \name can meet the timing requirements of xxx.

Similarly, we demonstrate 2.4 GHz transmissions by generating BLE advertisement packets. We implement the full baseband packet generation on the FPGA using only xx\% of its resources with a power consumption of xx~mW when transmitting at 0~dBm. We demonstrate a delay between sending packets on different channels of only xx and show our implementation achieves a sensitivity of xx which is comparable to the commercial BLE chips.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/3_platform_power/platform_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{Radio power consumption for each platform. We normalized TX power consumption for output power of 14~dBm.\newline
    **GalioT does not support transmitter mode.}}
	\label{fig:platform_power}
    \vskip -0.2in
\end{figure}

We summarize our contributions below:
\begin{itemize}
    \item We develop the first SDR platform tailored for the needs of an IoT testbed. Our platform is low cost, capable of implementing numerous IoT protocols both in 900~MHz and 2.4~GHz ISM bands, has an computation resources to do on-board processing, and highly granular power management for duty-cycled operation.
    \item We develop a complete over the air update system  its codes can be updated through a remote access point.
    \item We extensively characterize and evaluate our platform. To show the flexibility of \name, including case studies of two IoT protocols at 900~MHz and 2.4~GHz. We provide detailed measurements of the required FPGA resources and power needed for each. We also characterize our over-the-air update system for different programming data and measure ranges of an access point and platform and update times are measured.
\end{itemize}

%results
%- two boards
%fpga size, etc
%implemented LoRa and BLE sensitivity
%updates
%meet timing requirement



%show two case studies

==> platform-1.tex <==
{\footnotesize{
\centering
\vskip 0.2in
\begin{tabular}{|C{1.1cm}|C{0.6cm}|C{0.65cm}|C{1.4cm}|C{0.6cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
	\hline \rowcolor{black}
	\centering
	{\bf\color{white}Platform}
	& {\bf\color{white}Max BW}
	& {\bf\color{white}ADC}
	& {\bf\color{white}Frequency Spectrum}
% 	& {\bf\color{white}Size (inches)}
	& {\bf\color{white}Cost}
	& {\bf\color{white}Battery XXX}
	& {\bf\color{white}Scalibility}
	\\
	
    \hline \rowcolor{lightgray}
	{USRP E310\cite{usrpe310, ad9361digikey}} & 30.72 & 12 & 70$\sim$6000 & \$3k & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 30.72 & 12 & 70$\sim$6000 & \$733 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{bladeRF 2.0\cite{bladerf2, ad9361digikey}} & 30.72 & 12 & 47$\sim$6000 & \$720 & \xmark & \xmark\\

	\hline \rowcolor{lightgray}
	{LimeSDR Mini\cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 12 & 10$\sim$3500 & \$159 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{PlutoSDR\cite{XXX, XXX}} & 20 & 12 & 325$\sim$3800 & \$149 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{$\mu$SDR\cite{XXX, XXX}} & 40 & 8 & 2400$\sim$2500 & \$150 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{GalioT\cite{galiot, rtl2832}} & 14.4 & 8 & 0.5$\sim$1766 & \$60 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{\bf{\name}} & 4 & 13 & 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 & \$60 & \cmark & \cmark\\
	\hline
\end{tabular}
% \vskip -0.1in
\captionof{table}{\footnotesize{\bf SDR Platforms.}}
\label{tab:platforms}
}}

\section{Platform}
To motivate the need for an SDR platform tailored to prototyping IoT endpoints, we begin by outlining the unique challenges such as the power, size, and cost requirements of these devices as well as what capabilities this platform needs in terms of computation, frequency and bandwidth. Next, we present a detailed analysis of the capabilities of existing SDR platforms and show that there is currently no solution to support the growing research interests in this area. We will then outline the capabilities of our device.

%TODO: battery-powered definition
\subsection{Requirements for IoT endpoints}
We outline the unique needs of IoT endpoints to understand what a useful prototyping platform requires.

\squishlist
    \item {\bf Flexibility.} Unlike technologies such as Wi-Fi, there is no de-facto communication standard for IoT; in contrast, IoT protocols themselves are in active development which requires a platform that is flexible enough to implement, modify, and improve them. A common SDR platform that gives access to the raw signals allows for physical layer work on the protocols. Additionally, an SDR implementation of proprietary protocols such as LoRa would allow researchers to modify and improve the standard as well as enable higher layer work such as experimenting with MAC protocols. 
    
    \item{\bf Frequency and Bandwidth}
    A radio for IoT must operate at least at both 900~MHz and 2.4~GHz as IoT devices typically operate in these ISM bands. A single SDR platform that can operate at both frequencies would allow for side-by-side comparison of different protocols with a common radio front-end. Additionally, IoT sensor nodes produce relatively small amounts of data. Therefore unlike Wi-Fi which requires 20~MHz of bandwidth, IoT protocols such as LoRa and Sigfox are designed to use less than 500~kHz bandwidth and require lower sampling rates of maximum 1~MHz. 
     
    \item {\bf Scalibility.} 
    IoT nodes are often designed for large scale deployments on farms, in warehouses, across cities, and in many other environments without reliable power infrastructure. Therefore the ability to operate the platform on a battery is imperative and adds the additional constraint of low power consumption. A useful research platform should be able to operate for more than a year on a single charge when it is operating at 0.1 percent duty cycle with a 1000~mAh Lithium-Ion battery. Moreover, large batteries are expensive which raises the additional constraint of cost; an SDR platform should minimize cost with a target price of approximately \$xx per node in order to make larger scale deployments viable. Considering IoT nodes are operated as standalone devices, an SDR platform must also include all of the necessary computation and memory within this low power, low cost package. In addition, an IoT endpoint suitable for an IoT testbed requires wireless backbone support so it can perform PHY and MAC layer update remotely.
\squishend
    

\subsection{Existing SDR Platforms}
In order to understand why existing SDR platforms do not meet the above requirements we analyze their capabilities.
\vskip 0.05in\noindent{\bf Commercial SDR platforms.} Ettus Research (National Instruments) is one of the world's leaders in SDR platform technologies. They provide a variety of platforms such as USRP N210~\cite{}, Embedded USRP~\cite{} and USRP networked series~\cite{}. Many USRP models use peripheral buses such as USB or Ethernet to connect to a computer for controlling its function and recording data. The Embedded USRP series integrates a Dual Core ARM A9 processor and runs embedded Linux to allow for standalone applications but is priced at \$3000 per unit. Lime microsystems provides SDR platforms such as LimeSDR~\cite{} and LimeSDR Mini~\cite{}, which have open source design and use their custom transceiver IC. Nuand is another commercial SDR provider which recently released the bladeRF 2.0 micro SDR platform to provide a lower cost alternative to USRPs. More recently, Analog Devices has released their education focused PlutoSDR~\cite{} platform which uses AD9363~\cite{} radio front-end.
    
\vskip 0.05in\noindent{\bf Research SDR platforms.}
Over the past decade there has been multiple works on designing SDR platforms.  Tick~\cite{} achieves good programmability, high throughput and low latency by software-hardware co-design solutions. However, it uses a high power radio on the order of several watts~\cite{AD9371} and the whole design costs more than \$3000. SORA~\cite{sora} is a research platform that uses PCI-Express bus to provide sub 1~$\mu$s latency. However, it requires host PC for backbone processing and hence it ends up with a large form-factor. $\mu$SDR solves the latency challenge by using an advanced microcontroller bus architecture (AMBA) along with a Cortex-M3 ARM processor~\cite{musdr} and flash-based FPGA to process data. However, it is power-hungry for an IoT network deployment and relatively expensive. SODA~\cite{} proposed a fully programmable SDR architecture IC simulation which meets the requirements of high-end wireless protocols and consist of four SIMD cores. However, it has a slightly customized VLIW+SIMD ISA which needs users to hand-tune their program. KUAR~\cite{} is a research SDR platform that has a large form-factor design and requires PCI-Express connection to a host an embedded PC-like environment to operate. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio~\cite{rtl2832} connected to a Raspberry pi computer. This platform can only receive signal and the receiver RF front-end is power-hungry as shown in Fig.~\ref{fig:platform_power}.

%Adding the over the air support!
\vskip 0.05in\noindent{\bf Scalibility comparison.}
These commercial SDR platforms are designed to operate over frequencies up to 6~GHz and support bandwidths of 60~MHz, which requires high sampling rate ADCs and DACs and more importantly high digital baseband throughput to the processing unit and a computationally extensive processing unit. Moreover, the radio front-ends must also maintain good performance over this large frequency spectrum and bandwidth. Achieving good wide-band performance makes the fundamental trade-off of burning more power, making these platforms consume a few watts. Fig.~\ref{fig:platform_power} shows the power consumption of only the radio module in existing SDR platforms. Additionally, Table~\ref{tab:platforms} shows a comparison of other factors affecting deployment including XXX, XXX, and cost. This table shows that no existing solution meets all of the deployability concerns of IoT endpoints. 

\subsection{Our Capabilites}
Our platform achieves the requirements of IoT endpoints by providing all of the capabilities shown in Table~\ref{xxx}. Additionally it consumes only xx~mW of power.
We achieve this low power consumption using the following key insight: IoT protocols only require a few MHz of bandwidth and do not require microsecond latency therefore leaving an over-designed gap between the current SDR designs and what is required for IoT communication. By designing specifically for IoT solutions \name achieves low-power and last XXX years using only a XXX battery.



==> platform-2.tex <==
{\footnotesize{
\centering
\captionof{table}{\footnotesize{\bf SDR Platforms.}}
\vskip -0.15 in
\begin{tabular}{|C{1.1cm}|C{0.6cm}|C{0.65cm}|C{1.4cm}|C{0.6cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
	\hline \rowcolor{black}
	\centering
	{\bf\color{white}Platform}
	& {\bf\color{white}Max BW}
	& {\bf\color{white}ADC}
	& {\bf\color{white}Frequency Spectrum}
% 	& {\bf\color{white}Size (inches)}
	& {\bf\color{white}Cost}
	& {\bf\color{white}Battery XXX}
	& {\bf\color{white}Scalibility}
	\\
	
    \hline \rowcolor{lightgray}
	{USRP E310\cite{usrpe310, ad9361digikey}} & 30.72 & 12 & 70$\sim$6000 & \$3k & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 30.72 & 12 & 70$\sim$6000 & \$733 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{bladeRF 2.0\cite{bladerf2, ad9361digikey}} & 30.72 & 12 & 47$\sim$6000 & \$720 & \xmark & \xmark\\

	\hline \rowcolor{lightgray}
	{LimeSDR Mini\cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 12 & 10$\sim$3500 & \$159 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{PlutoSDR\cite{XXX, XXX}} & 20 & 12 & 325$\sim$3800 & \$149 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{$\mu$SDR\cite{XXX, XXX}} & 40 & 8 & 2400$\sim$2500 & \$150 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{GalioT\cite{galiot, rtl2832}} & 14.4 & 8 & 0.5$\sim$1766 & \$60 & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{\bf{\name}} & 4 & 13 & 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 & \$60 & \cmark & \cmark\\
	\hline
\end{tabular}
% \vskip -0.1in
\label{tab:platforms}
}}

\section{SDR Requirements for IoT devices} 
To motivate the need for XXXX XXXX XXXXXXXX XXXXX XXXXX XXXXX XXXXxx xx   We outline the unique needs of IoT endpoints to understand what a useful prototyping platform requires.

\squishlist
    \item {\bf Flexibility.} Unlike technologies such as Wi-Fi, there is no de-facto communication standard for IoT; in contrast, IoT protocols themselves are in active development which requires a platform that is flexible enough to implement, modify, and improve them. A common SDR platform that gives access to the raw signals allows for physical layer work on the protocols. Additionally, an SDR implementation of proprietary protocols such as LoRa would allow researchers to modify and improve the standard as well as enable higher layer work such as experimenting with MAC protocols. 
    
    \item{\bf Frequency and Bandwidth}
    A radio for IoT must operate at least at both 900~MHz and 2.4~GHz as IoT devices typically operate in these ISM bands. A single SDR platform that can operate at both frequencies would allow for side-by-side comparison of different protocols with a common radio front-end. Additionally, IoT sensor nodes produce relatively small amounts of data. Therefore unlike Wi-Fi which requires 20~MHz of bandwidth, IoT protocols such as LoRa and Sigfox are designed to use less than 500~kHz bandwidth and require lower sampling rates of maximum 1~MHz. 
     
    \item {\bf Scalibility.} 
    IoT nodes are often designed for large scale deployments on farms, in warehouses, across cities, and in many other environments without reliable power infrastructure. Therefore the ability to operate the platform on a battery is imperative and adds the additional constraint of low power consumption. A useful research platform should be able to operate for more than a year on a single charge when it is operating at 0.1 percent duty cycle with a 1000~mAh Lithium-Ion battery. Moreover, large batteries are expensive which raises the additional constraint of cost; an SDR platform should minimize cost with a target price of approximately \$xx per node in order to make larger scale deployments viable. Considering IoT nodes are operated as standalone devices, an SDR platform must also include all of the necessary computation and memory within this low power, low cost package. In addition, an IoT endpoint suitable for an IoT testbed requires wireless backbone support so it can perform PHY and MAC layer update remotely.
\squishend
    

\subsection{Existing SDR Platforms}
In order to understand why existing SDR platforms do not meet the above requirements we analyze their capabilities.
\vskip 0.05in\noindent{\bf Commercial SDR platforms.} Ettus Research (National Instruments) is one of the world's leaders in SDR platform technologies. They provide a variety of platforms such as USRP N210~\cite{}, Embedded USRP~\cite{} and USRP networked series~\cite{}. Many USRP models use peripheral buses such as USB or Ethernet to connect to a computer for controlling its function and recording data. The Embedded USRP series integrates a Dual Core ARM A9 processor and runs embedded Linux to allow for standalone applications but is priced at \$3000 per unit. Lime microsystems provides SDR platforms such as LimeSDR~\cite{} and LimeSDR Mini~\cite{}, which have open source design and use their custom transceiver IC. Nuand is another commercial SDR provider which recently released the bladeRF 2.0 micro SDR platform to provide a lower cost alternative to USRPs. More recently, Analog Devices has released their education focused PlutoSDR~\cite{} platform which uses AD9363~\cite{} radio front-end.
    
\vskip 0.05in\noindent{\bf Research SDR platforms.}
Over the past decade there has been multiple works on designing SDR platforms.  Tick~\cite{} achieves good programmability, high throughput and low latency by software-hardware co-design solutions. However, it uses a high power radio on the order of several watts~\cite{AD9371} and the whole design costs more than \$3000. SORA~\cite{sora} is a research platform that uses PCI-Express bus to provide sub 1~$\mu$s latency. However, it requires host PC for backbone processing and hence it ends up with a large form-factor. $\mu$SDR solves the latency challenge by using an advanced microcontroller bus architecture (AMBA) along with a Cortex-M3 ARM processor~\cite{musdr} and flash-based FPGA to process data. However, it is power-hungry for an IoT network deployment and relatively expensive. SODA~\cite{} proposed a fully programmable SDR architecture IC simulation which meets the requirements of high-end wireless protocols and consist of four SIMD cores. However, it has a slightly customized VLIW+SIMD ISA which needs users to hand-tune their program. KUAR~\cite{} is a research SDR platform that has a large form-factor design and requires PCI-Express connection to a host an embedded PC-like environment to operate. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio~\cite{rtl2832} connected to a Raspberry pi computer. This platform can only receive signal and the receiver RF front-end is power-hungry as shown in Fig.~\ref{fig:platform_power}.

%Adding the over the air support!
\vskip 0.05in\noindent{\bf Scalibility comparison.}
These commercial SDR platforms are designed to operate over frequencies up to 6~GHz and support bandwidths of 60~MHz, which requires high sampling rate ADCs and DACs and more importantly high digital baseband throughput to the processing unit and a computationally extensive processing unit. Moreover, the radio front-ends must also maintain good performance over this large frequency spectrum and bandwidth. Achieving good wide-band performance makes the fundamental trade-off of burning more power, making these platforms consume a few watts. Fig.~\ref{fig:platform_power} shows the power consumption of only the radio module in existing SDR platforms. Additionally, Table~\ref{tab:platforms} shows a comparison of other factors affecting deployment including XXX, XXX, and cost. This table shows that no existing solution meets all of the deployability concerns of IoT endpoints. 


==> platform-3.tex <==
\begin{table*}[t]
    \centering
    \caption{\footnotesize{SDR Platforms.}}
    \vskip -0.15 in
    \footnotesize{
\begin{tabular}{|c|C{1.2cm}|C{1.4cm}|c|c|C{1.7cm}|c|c|c|c|}
	\hline 
	\rowcolor{lightgray}
	{Platform} & {\bf Sleep Current (uA)} & {Standalone} & {\bf OTA} & {\bf Cost} & {\bf Max BW (MHz)} & {\bf ADC Resolution} & {\bf Frequency Spectrum (MHz)}& {\bf Size}\\
	{USRP E310 \cite{usrpe310, ad9361}} & XXX & XXX & XXX & \$3000 & 30.72 & 12 & 70$\sim$6000 & XXX\\
	\hline
% 	{USRP B200mini \cite{usrpb200mini, ad9364}} & 30.72 & 12 & 70$\sim$6000 & \$733 & XXX & \xmark\\
% 	\hline
% 	{bladeRF 2.0 \cite{bladerf2, ad9361}} & 30.72 & 12 & 47$\sim$6000 & \$720 & XXX & \cmark\\
% 	\hline
% 	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 12 & 10$\sim$3500 & \$159 & XXX  & \xmark\\
% 	\hline
% 	{PlutoSDR \cite{ad9363}} & 20 & 12 & 325$\sim$3800 & \$149 & XXX & \xmark\\
%     \hline
% 	{$\mu$SDR \cite{max2831, ad9228, max5189}} & 40 & 8 & 2400$\sim$2500 & \$150 & XXX & \xmark\\
% 	\hline
% 	{GalioT \cite{galiot, rtl2832}} & 14.4 & 8 & 0.5$\sim$1766 & \$60 & XXX & \cmark\\
% 	\hline
% 	{\bf{\name}} & 4 & 13 & 389.5$\sim$510, 779$\sim$1020, 2400$\sim$2483 & \$60 & XXX &\cmark\\
% 	\hline
\end{tabular}
}
\label{tab:platforms}
\end{table*}

% {\footnotesize{
% \centering
% \captionof{table}{\footnotesize{SDR Platforms.}}
% \vskip -0.15 in
% \begin{tabular}{|C{1.1cm}|C{0.6cm}|C{0.65cm}|C{1.4cm}|C{0.6cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
% 	\hline \rowcolor{black}
% 	\centering
% 	{\bf\color{white}Platform}
% 	& {\bf\color{white}Max BW}
% 	& {\bf\color{white}ADC}
% 	& {\bf\color{white}Frequency Spectrum}
% % 	& {\bf\color{white}Size (inches)}
% 	& {\bf\color{white}Cost}
% 	& {\bf\color{white}Battery XXX}
% 	& {\bf\color{white}Standalone}
% 	\\
	
%     \hline \rowcolor{lightgray}
% 	{USRP E310 \cite{usrpe310, ad9361}} & 30.72 & 12 & 70$\sim$6000 & \$3k & \xmark & \cmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{USRP B200mini \cite{usrpb200mini, ad9364}} & 30.72 & 12 & 70$\sim$6000 & \$733 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{bladeRF 2.0 \cite{bladerf2, ad9361}} & 30.72 & 12 & 47$\sim$6000 & \$720 & \xmark & \cmark\\

% 	\hline \rowcolor{lightgray}
% 	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 12 & 10$\sim$3500 & \$159 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{PlutoSDR \cite{ad9363}} & 20 & 12 & 325$\sim$3800 & \$149 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{$\mu$SDR \cite{max2831, ad9228, max5189} & 40 & 8 & 2400$\sim$2500 & \$150 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{GalioT \cite{galiot, rtl2832}} & 14.4 & 8 & 0.5$\sim$1766 & \$60 & \xmark & \cmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{\bf{\name}} & 4 & 13 & 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 & \$60 & \cmark & \cmark\\
% 	\hline
% \end{tabular}
% % \vskip -0.1in
% \label{tab:platforms}
% }}

\section{SDR Requirements for IoT Nodes} 
To motivate the need for \name and inform our design decisions we begin by identifying the key requirements for an IoT endpoint platform that can be used to build the testbed vision described above. These include operation in the 900 MHz and 2.4~GHz bands, low power operation which requires the ability to transition to an ultra-low power sleep mode, standalone operation which requires an onboard control unit to duty cycle the radio, an OTA programming interface to manage large scale deployments, and low cost per node. While there are a number of commercially available SDRs~\cite{usrp} on the market and numerous SDR research prototypes~\cite{dinesh,sora,swarun,warp}, all of them have been designed to implement gateway devices. We analyze the shortcomings of each of these platforms in the context of IoT endpoint requirements below and show that \name is the only one that can meet these needs.

\subsection{Low power operation and sleep mode}
How do SDR platforms compare in terms of power? Fig.~\ref{fig:platform_power} compares the power consumption of the radio module alone in existing SDR platforms considering each one has different peripherals. Interestingly we find that most SDR platforms consume 200-300~mW in receive mode, but almost 10x when transmitting. While this may be acceptable for a gateway typical IoT endpoints do the opposite and are required to transmit data like sensor information. Moreover, real IoT nodes spend a very short time transmit before quickly transitioning to ultra-low power sleep modes. Although IoT radios often consume milliwatts of power, and the key to achieving long battery lifetimes is exploiting the microwatt power sleep modes. Table~\ref{tab:platforms} shows that none of the other platforms can benefit from duty cycling as they consume more power in sleep mode than \name does when transmitting. In contrast \name's microwatt power consumption in sleep mode enables the benefits of duty cycling and allows for dramatic power savings.

\subsection{Standalone operation and cost}
We first observe that half of these platforms do not allow for standalone operation, meaning they cannot be used in a testbed deployment without an external computer. Among the ones that do,  Embedded USRP and bladeRF cost \$700 or more per unit making large scale deployments exorbitantly expensive. GalioI~\cite{galiot} presents an SDR platform using the low cost RTL2832U radio~\cite{rtl2832} connected to a Raspberry Pi computer which allows for standalone operation, however it does not support the 2.4~GHz band. Moreover, this platform is \textit{receiver only} and cannot be used to prototype a typical IoT node that transmits data. This leaves \name as the only low cost platform that can transmit and receive in both ISM bands without being tethered to an external computer.

\subsection{OTA programming}
As shown in Table~\ref{tab:platforms}, all of the existing SDR platforms rely on wired interfaces for programming. This means that even if one of these systems were connected to a battery, running an experiment would require either tethering each one to a wired network or individually programming each one. An OTA programming system is crucial to realizing the goal of a large scale wide area testbed as it leaves researchers to decide between limiting themselves to deployment scenarios with wired infrastructure which are not representative of most real IoT use cases or traveling over \textit{kilometer} distances to update individual nodes for \textit{each} experiment or minor modification to a protocol which is unmanageable.

% \squishlist
%     \item{\bf Frequency and Bandwidth}
%      IoT endpoints typically operate in the 900~MHz or 2.4~GHz ISM bands. A platform to develop and evaluate these protocols should therefore be able to operate in both bands. In terms of bandwidth, IoT sensor nodes typically produce small amounts of data and seek to share the crowded ISM band between many nodes. An IoT platform therefore only requires a few megahertz of bandwidth to support common protocols such as BLE, LoRa and Sigfox.
    
%     \item {\bf Raw I/Q processing.} In order to support any protocol as well as the development of new ones a flexible endpoint must give access to raw I/Q complex samples and include onboard computation. This enables full access to the physical layer for experimenting with different modulation techniques, as well as the ability to process signals with filters, encryption, compression or machine learning algorithms.
    
%     \item {\bf Low power operation.} In addition to providing the SDR flexibility described above, a useful IoT endpoint platform should be able to run off of a battery just like real IoT devices in large scale deployments and include flexible options for power management.
%     sleep current 
     
%     \item {\bf Standalone operation.} While battery operation untethers nodes from a power source, true standalone operation that would enable a an IoT testbed must also include an onboard control unit to run functions like a MAC protocol and toggling power modes as well as a means of wirelessly updating the firmware to actually run different tests on the network. 
    
%     \item {\bf Low cost and small form factor.} The requirements above describe the technical needs of an IoT endpoint, but from a practical perspective an IoT prototyping platform should also minimize size and cost, targeting a price of \$xx or less to make large scale deployments feasible.
% \squishend
    
% \subsection{Existing SDR Platforms}
% Now that we have identified the needs of an SDR platform for IoT, we analyze the many existing SDR platforms in this context to determine whether they meet these requirements. Table ~\ref{tab:platforms} breaks down the specs of each of these SDRs. 

% iot requires xxx
% while there has been prior work xxx xxx
% all have been designed for gateways
% usrp dinesh sora swarun warp

==> protocol-0.tex <==
\begin{figure}[t]
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_tx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{LoRa Modulator}}
        \label{fig:lora_tx_block}
    \end{subfigure}
	\begin{subfigure}{\linewidth}
	    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_rx_block.eps}
        \caption{\footnotesize{LoRa Demodulator}}
        \label{fig:lora_rx_block}
    \end{subfigure}
    \vskip -0.15in
    \caption{\footnotesize{LoRa implementation FPGA block diagrams.}}
    \label{fig:lora_blocks}
\end{figure}

\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/lora_packet.eps}
	\vskip -0.15 in
	\caption{\footnotesize{LoRa packet structure.}}
	\label{fig:lora_packet}
	\vskip -0.2 in
\end{figure}

\section{Implementing Protocols}
\subsection{LoRa}
To demonstrate the capability of \name at sub-GHz frequencies, we implement a LoRa modulator and demodulator. We choose LoRa as it is gaining popularity for IoT solutions due to its long range capabilities described above. Considering LoRa is a proprietary standard, we begin by describing the basics of its modulation and packet structure followed by the implementation details of our modulator and demodulator.

\subsubsection{LoRa Protocol Primer}
\vskip -0.1 in
LoRa achieves long ranges by using Chirp Spread Scpectrum (CSS) modulation. In CSS, data is modulated using linearly increasing frequency signals or upchirp symbol. Each upchirp symbol has two main features; Spreading Factor (SF) and Bandwidth (BW). Spreading factor determines determines the number of bits that each upchirp symbol represents~\cite{netscatter,lorabackscatter} and $\frac{1}{BW}$ shows the length of each upchirp symbol in time. The SF and BW settings therefore allows users to trade data rate for range. LoRa uses SF values from 6 to 12. The BW determines the total frequency spectrum that each upchirp symbol utilizes which results in a data rate of $\frac{2^{SF}}{BW}\times CR$. The final CR term represents any coding of the data in the payload itself. Each upchirp symbol covers the whole BW frequency. The starting point of the symbol in frequency domain which is the cyclic shift of the upchirp symbol determines the chirp symbol value~\cite{lora_basics}.

Fig.~\ref{fig:lora_packet} shows the LoRa packet structure which begins with a preamble which consists of 10 zero symbols (upchirps with zero cyclic-shift). This is followed by the Sync field with two upchirp data symbols that can indicate information about the network or configuration. Next, a sequence of 2.25 downchirp symbols (chirp symbol with linearly decreasing frequency) indicate the beginning of the payload. The payload then consists of a sequence of upchirp symbols which encode a header, payload and CRC.

\subsubsection{LoRa modulator}
\vskip -0.1 in
Fig.~\ref{fig:lora_tx_block} shows the block diagram of our LoRa modulator. Because CSS is not a pre-programmed modulation option on the AT86RF215, we use our FPGA to implement a LoRa modulator in Verilog and stream data to the radio in I/Q mode. The modulator begins with the {Packet Generator} module reading the data symbols to be sent either from FPGA memory for transmitting fixed packets or from the MCU, as well as LoRa configuration parameters such as SF, and BW. This module then determines all of the necessary parameters for generating a chirp such as its length, chirp slope, and step resolution of the linear frequency sweep. Next, the {Packet Generator} sends these parameters along with the symbol values to the {Chirp Generator} module, which generates the complex values for each chirp symbol in the packet. This block uses a phase accumulator along with two lookup tables for $Sin$ and $Cosin$ functions to generate I/Q samples for a linear chirp as demonstrated in~\cite{lorabackscatter}. We then feed the complex samples into {I/Q Serializer} explained above to stream them over the LVDS interface to the I/Q radio.

\subsubsection{LoRa demodulator}
Fig.~\ref{fig:lora_rx_block} shows the block diagram of our LoRa demodulator. This demodulator begins by reading data from the I/Q radio into the {I/Q Deserializer} module on the FPGA which converts the serial I/Q stream to parallel I/Q for further signal processing. Next, we run these data through an XXX tap XXX low-pass FIR filter to xxxxxx. We store the filtered samples in a buffer implemented using the FPGAs onboard memory. To decode the data, we use the {Chirp Generator} mpodule from the {LoRa modulator} described above to generate a baseline upchirp/downchirp symbol, and then we multiply that with the received chirp symbol using our {Chirp Multiplier} unit which gives the coding gain of CSS. The output of the multiplication then goes to an XXX-point FFT block implemented using a standard IP core from Lattice. Finally the {Symbol Detector} scans the output of the FFT for peaks and records the frequency of the peak to determine the symbol value. To detect chirp type (upchirp/downchirp), we multiply each chirp symbol with both upchirp and downchirp and then compare the amplitude of their FFT peak. The higher peak in FFT result shows higher correlation which we use to detect the chirp type.

\subsubsection{LoRa MAC Layer}
To demonstrate that our LoRa implementation can be used in a real network, we need a MAC protocol to manage transmissions between devices in addition to the physical layer described above. We show that \name is compatible with the existing LoRa based {The Things Network} (TTN)~\cite{thingsnetwork} by implementing its MAC protocol. We adopt the design from TTN's open source Arduino libraries~\cite{ttnarduino} and implement it on \name's MCU. TTN uses two methods for device association; Over-the-air activation (OTAA) and activation by personalization (ABP). OTAA is a secure way to connect with TTN in which nodes perform a join-procedure with the network. During this process a dynamic device address is assigned to the node and security keys are negotiated. ABP allows for a simplified approach in which the device address as well as the security keys are hard coded on the device allowing it to skip the join procedure. Our implementation supports both OTAA and ABP methods.

\subsection{Bluetooth Low Energy}
In addition to the sub-GHz radio our AT86RF215 includes a 2.4~GHz radio as well. To demonstrate \name's 2.4~GHz capabilities we implement Bluetooth beacons which are commonly used for IoT devices. We begin with a brief primer on the BLE physical layer followed by details about our implementation.


\subsubsection{BLE Advertising Primer}
\vskip -0.1 in
Bluetooth Low Energy includes a variety of different modes and packet types, we specifically implement non-connectable BLE advertisements (ADV\_NON\_CONN\_IND) which are broadcast packets used for beacons. These packets allow a low power device to simply boardcast its data to any listening receiver within range without the power overhead of exchanging packets needed to negotiate a connection. These packets themselves have a bit rate of 1~Mbps in Bluetooth 4.0 or up to 2~Mbps in Bluetooth 5.0 and are generated using GFSK with a modulation index of 0.45-0.55. The GFSK modulation is simply binary frequency shift keying (BFSK) with the addition of a Gaussian filter to the square wave pulses to be transmitted which reduces the spectral width. While BLE divides the 2.4~GHz band into a total of 40 channels each spaced 2~MHz apart, only 3 of these throughout the band are set aside for advertisements. A typical BLE advertisement is transmitted on each of the three advertising channels one after another to mitigate the chance of collisions as this protocol trades off a more sophisticated MAC protocol for power savings.

\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/ble_tx_block.eps}
	\vskip -0.15 in
	\caption{BLE implementation on FPGA.}
	\label{fig:ble_tx_block}
\end{figure}

\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/ble_packet.eps}
	\vskip -0.15 in
	\caption{\footnotesize{BLE packet structure.}}
	\label{fig:ble_packet}
	\vskip -0.2 in
\end{figure}

\subsubsection{Generating a BLE packet}
The first step to transmitting a BLE advertisement is to generate the bitstream for a valid BLE packet. The structure of an advertising packet is shown in Fig.~\ref{fig:ble_packet}. Advertisements range from 6-37 octets, beginning with a fixed preamble of 0xAA followed by the access address field which is also set to a fixed sequence 0x8E89BED6 which indicates to a receiver the packet is a non-connectable advertisement. These fields are followed by the packet data unit (PDU) which begins with a 2 byte length field indicating the size of the PDU followed by the data segment which includes an advertisement address which can indicate specific device or device type followed by the packet data such as a 128 bit UUID. In addition to this packet structure, BLE requires a 3 byte CRC as well as whitening of the PDU to create a valid packet which we explain below.


\noindent {\bf CRC Generation.} The Bluetooth CRC is a 3 byte sequence generated using the 24-bit linear feedback shift register (LFSR) with the polynomial $x^{24} + x^{10} + x^{9} + x^{6} + x^{4} + x^{3} + x + 1$. The LFSR is set to a starting state of 0x555555 and each byte of the PDU beginning with the length field is input to the LFSR LSB first. The final state of the LFSR after all of the data bits pass through then becomes the CRC. We implement this in xxx on the xxx.

\noindent {\bf Data Whitening.} Data whitening is performed to eliminate long strings of zeros or ones within a packet. This is also done using a 7-bit LFSR with polynomial $x^7 + x^4 + 1$. The LFSR is initialized with the lower 7 bits of the channel number the packet will be transmitted on, and each byte is input LSB first. We implement this in xxx on the xxx.

\noindent {\bf Transmitting a packet.} Now that we have the bitstream, we need to generate the I/Q samples to stream to the radio. To do this we begin by taking the bitstream and upsampling it to XX~MHz to generate a square wave corresponding to the segments of high and low frequencies for BLE's FSK modulation. Before actually modulating the data however, we first smooth the waveform using a Gaussian filter which eliminates the sharp transitions between bits and suppresses unwanted sidelobes. Finally, to generate the BLE waveform we use a modified version of our phase accumulator block described above that creates frequency modulated signals for LoRa. This block us the integrates the frequency to get the phase which we feed to a sine and cosine function to get the I and Q signals. These samples are then sent to the I/Q serializer and streamed to the radio.


==> protocol-1.tex <==
\begin{figure}[t]
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_tx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{{\bf LoRa Modulator}}}
        \label{fig:lora_tx_block}
    \end{subfigure}
	\begin{subfigure}{\linewidth}
	    \centering
        \includegraphics[width=1\linewidth]{figs/block_diagram/lora_rx_block.eps}
        \vskip -0.1in
        \caption{\footnotesize{{\bf LoRa Demodulator}}}
        \label{fig:lora_rx_block}
    \end{subfigure}
    \vskip -0.1in
    \caption{\footnotesize{{\bf LoRa implementation block diagrams.}}}
    \label{fig:lora_blocks}
\end{figure}

\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/lora_packet.eps}
	\vskip -0.15 in
	\caption{\footnotesize{{\bf LoRa packet structure.}}}
	\label{fig:lora_packet}
	\vskip -0.2 in
\end{figure}

\section{Protocol Case Studies}
To demonstrate the use of \name at 900~MHz and 2.4~GHz, we explore two case studies: LoRa and Bluetooth beacons.
\subsection{LoRa Protocol with \name}
 We choose LoRa as it is gaining popularity for IoT solutions due to its long range capabilities. Since LoRa is a proprietary standard, we begin by describing the basics of its modulation and packet structure followed by the implementation details of our modulator, demodulator and MAC protocol.

{\bf LoRa Protocol Primer.} 
LoRa achieves long ranges by using Chirp Spread Scpectrum (CSS) modulation. In CSS, data is modulated using linearly increasing frequency signals or upchirp symbol. Each upchirp symbol has two main features; Spreading Factor (SF) and Bandwidth (BW). SF determines the number of bits of each upchirp symbol~\cite{lorasigcomm17,netscatter,lorabackscatter} and BW is the difference between upper and lower frequency of the chirp which together with SF determines the length of each upchirp symbol. The SF and BW settings trade data rate for range. Data is modulated by $2^{SF}$ cyclic-shifts of an upchirp symbol. The starting point of the symbol in frequency domain which is the cyclic shift of the upchirp symbol determines the chirp symbol value~\cite{lora_basics}. LoRa uses SF values from 6 to 12 and BW values from 7.8125~KHz to 500~KHz which achieves PHY-layer rate of $\frac{BW}{2^{SF}}\times SF$. 

Fig.~\ref{fig:lora_packet} shows the LoRa packet structure which begins with a preamble with 10 zero symbols (upchirps with zero cyclic-shift). This is followed by the Sync field with two upchirp  symbols that indicate information about the network or configuration. Next, a sequence of 2.25 downchirp symbols (chirp symbol with linearly decreasing frequency) indicate the beginning of the payload. The payload then consists of a sequence of upchirp symbols which encode a header, payload and CRC.

{\bf LoRa Modulator.} 
Fig.~\ref{fig:lora_tx_block} shows the block diagram of our LoRa modulator. Because CSS is not a pre-programmed modulation option on the AT86RF215, we use our FPGA to implement a LoRa modulator in Verilog and stream data to the radio in I/Q mode. The modulator begins with the {\it Packet Generator} module reading the data symbols to be sent either from FPGA memory for transmitting fixed packets or from the MCU, as well as LoRa configuration parameters such as SF, coding and BW. This module then determines all of the necessary parameters for generating a chirp such as its length, chirp slope, and step resolution of the linear frequency sweep. Next, the {\it Packet Generator} sends these parameters along with the symbol values to the {\it Chirp Generator} module, which generates the complex values for each chirp symbol in the packet. This block uses a phase accumulator along with two lookup tables for $Sin$ and $Cosin$ function to generate I/Q samples for a linear chirp similar to~\cite{lorabackscatter}. We then feed the complex samples into {I/Q Serializer}  to stream them over the LVDS interface to the I/Q radio.

{\bf LoRa Demodulator. }
Fig.~\ref{fig:lora_rx_block} shows the block diagram of our LoRa demodulator. It begins by reading data from the I/Q radio into the {\it I/Q Deserializer} module on the FPGA which converts the serial I/Q stream to parallel I/Q for further signal processing. Next, we run these data through a 14 tap FIR low-pass filter to suppress high frequency noise and interference. We store the filtered samples in a buffer implemented using the FPGA memory blocks. To decode the data, we use the {\it Chirp Generator} module from the {\it LoRa Modulator} described above to generate a baseline upchirp/downchirp symbol, and then we multiply that with the received chirp symbol using our {\it Chirp Multiplier} unit which gives the coding gain of CSS. The output of the multiplication then goes to an FFT block implemented using a standard IP core from Lattice. Finally the {\it Symbol Detector} scans the output of the FFT for peaks and records the frequency of the peak to determine the symbol value. To detect chirp type (upchirp/downchirp), we multiply each chirp symbol with both upchirp and downchirp and then compare the amplitude of their FFT peak. The higher peak in FFT result shows higher correlation which we use to detect the chirp type.

{\bf LoRa MAC Layer.} 
To demonstrate that LoRa implementation on \name is compatible with existing LoRa networks such as {The Things Network} (TTN)~\cite{thingsnetwork}, we adopt LoRa MAC design from TTN's Arduino libraries~\cite{ttnarduino} and implement it on \name's MCU. TTN uses two methods for device association; Over-the-air activation (OTAA) and activation by personalization (ABP). {In OTAA, each node performs a join-procedure with the network, during which a dynamic device address is assigned with the device. However, in ABP we can hard-code the device address in the device which makes it simpler since the node skips the join procedure. Our implementation supports both OTAA and ABP methods.}

\subsection{BLE Beacons with \name}
To demonstrate \name's 2.4~GHz capabilities we implement Bluetooth beacons which are commonly used for IoT devices. 


{\bf BLE Beacon Primer.} 
BLE includes a variety of different modes and packet types, we specifically implement non-connectable BLE advertisements (ADV\_NON\_CONN\_IND) which are broadcast packets used for beacons. These packets allow a low power device to broadcast its data to any listening receiver within range without the power overhead of exchanging packets needed to negotiate a connection. These packets themselves have a bit rate of 1~Mbps in Bluetooth 4.0 or up to 2~Mbps in Bluetooth 5.0 and are generated using GFSK with a modulation index of 0.45-0.55. The GFSK modulation is simply binary frequency shift keying (BFSK) with the addition of a Gaussian filter to the square wave pulses to be transmitted which reduces the spectral width. 
\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/ble_tx_block.eps}
	\vskip -0.15 in
	\caption{\footnotesize{{\bf BLE implementation block diagram.}}}
	\label{fig:ble_tx_block}
\end{figure}

\begin{figure}[t]
    \centering
	\includegraphics[width=\linewidth]{./figs/block_diagram/ble_packet.eps}
	\vskip -0.15 in
	\caption{\footnotesize{{\bf BLE packet structure.}}}
	\label{fig:ble_packet}
	\vskip -0.2 in
\end{figure}

{\bf Generating a BLE Packet.} 
 The structure of an BLE beacon is shown in Fig.~\ref{fig:ble_packet}. Advertisements range from 6-37 octets, beginning with a fixed preamble of 0xAA followed by the access address field which is also set to a fixed sequence 0x8E89BED6 which indicates to a receiver the packet is a non-connectable advertisement. These fields are followed by the packet data unit (PDU) which begins with a 2 byte length field indicating the size of the PDU followed by the data segment which includes an advertisement address which can indicate specific device or device type followed by the packet data such as a 128 bit UUID. In addition to this packet structure, BLE requires a 3 byte CRC as well as whitening of the PDU to create a valid packet.


 {\bf CRC Generation.} The Bluetooth CRC is a 3 byte sequence generated using the 24-bit linear feedback shift register (LFSR) with the polynomial $x^{24} + x^{10} + x^{9} + x^{6} + x^{4} + x^{3} + x + 1$. The LFSR is set to a starting state of 0x555555 and each byte of the PDU beginning with the length field is input to the LFSR LSB first. The final state of the LFSR after all of the data bits pass through then becomes the CRC. We implement this block in Verilog on the FPGA.

 {\bf Data Whitening.} Data whitening is performed to eliminate long strings of zeros or ones within a packet. This is also done using a 7-bit LFSR with polynomial $x^7 + x^4 + 1$. The LFSR is initialized with the lower 7 bits of the channel number the packet will be transmitted on, and each byte is input LSB first. We implement this block in Verilog on the FPGA.

{\bf Transmitting a packet.} From this bitstream, we need to generate the I/Q samples to feed to the I/Q radio. As shown in Fig.~\ref{fig:ble_tx_block}, first, we filter the generated bitstream by a  Gaussian filter. This gives us the frequency which we then integrate it to get the phase. We feed the phase to sine and cosine function to get I and Q samples, which are passed to I/Q serializer to send them to I/Q radio through LVDS interface.

{\bf MAC protocol.}  While BLE divides the 2.4~GHz band into a total of 40 channels each spaced 2~MHz apart, a typical BLE beacon is transmitted on each of the three advertising channels in a sequential order separated by a few hundred microseconds, without carrier sense. This sequence of three beacons are re-transmitted every advertising interval which is a minimum of 20~ms~\cite{ble_spec}.


% \subsection{Orthogonal LoRa Demodulation}
% In this section, we demonstrate that we can demodulate multiple orthogonal chirp symbols on \name. 

% \subsubsection{LoRa orthogonal transmissions.}
% LoRa protocol supports orthogonal transmissions~\cite{lora_basics} which can occupy the same frequency channel and does not interference with each other. LoRa uses orthogonal transmissions to increase network capacity. For a chirp with spreading factor of $SF$ and bandwith of $BW$, we define chirp slope as the bandwidth occupation of the chirp over time and it is qual to $\frac{BW^{2}}{2^{SF}}$~\cite{netscatter}. Two chirp symbols are orthogonal when they have different chirp slope. Semtech chipset such as SX1308~\cite{sx1308} provides programmable parallel demodulation for different LoRa configurations. Here, we show that we can also demodulate different multiple LoRa transmissions at the same time using \name.

% \subsubsection{Orthogonal demodulation}
% We target to demodulate two upchirp symbols which has two configurations; $SF1, BW1$ and $SF2, BW2$. First, we generate two downchirp symbols with the same configurations. We perform correlation on each separately by multiplying each upchirp symbol to the corresponding downchirp symbol. After correlation, we use FFT operation to detect the maximum peak power of each upchirp symbol. We perform all operations on two parallel pip-lines to demodulate two upchirp symbols concurrently. 

==> related-1.tex <==
\section{The Case for \name and Related Work}
To demonstrate that \name is the best platform for network research community to deploy  large-scale IoT networks, we first compare it with existing SDR platforms in terms of XXX, XXX and XXX. We then discuss prior work on SDR platforms and compare \name with existing solutions.



\squishlist
    \item {\bf Power consumption.} Conventional SDR platforms are designed to operate at high frequency bandwidth which result in using high sampling rate ADCs and DACs. Existing platforms such as Embedded USRP E310~\cite{XXX}, bladeRF~\cite{XXX} and LimeSDR~\cite{XXX} operate up to 60~MHz bandwidth ans support wide-band frequency spectrum. Therefore, they require to use radios with high sampling rate front-end and also optimize radio noise figure over large frequency spectrum. In contrast, IoT protocols such as LoRa, Sigfox use less than 500~kHz bandwidth and operate at low sampling rate. Fig.~\ref{fig:platform_power} shows the power consumption of radio module in conventional SDR platforms. This plot shows that existing SDR platforms use power-hungry RF front-ends which consumes in the order of few watts of power in transmit mode and few hundred milliwatts of power in receive mode. High power consuming radios are not suitable for a battery-powered SDR platform which is the our target for large-scale research deployments. This requirements lead us to redesigning existing SDR solutions and optimizing them for IoT protocols. We design \name that can operate at low-power and last XXX years using only a XXX battery.
    
    % \item {\bf Bandwidth.} Conventional SDR platform are designed to support huge sampling rate and bandwidth. These platforms support wide-band frequency spectrum and more than 20~MHz bandwidth to support different 802.11 standards. In contrast, IoT protocols such as LoRa, Sigfox and etc. use less than 500~kHz bandwidth and operate at low sampling rate. This requirements lead us to redesigning existing SDR solutions and optimizing them for IoT protocols. We design \name platform based on requirements of existing IoT protocols.    
    
    \item {\bf Latency.} Existing conventional SDR platforms focused on providing a low-latency design. SORA~\cite{sora} uses PCI-Express bus to provide sub 1~$mu$s latency. USRP uses peripheral buses such as USB or Ethernet to connect to a computer with operating system for its controlling signal. Embedded USRP E310 benefits from a Dual Core ARM A9 processor for processing high data-rate information. $\mu$SDR solves the latency challenge by using an advanced microcontroller bus architecture (AMBA) along with a Cortex-M3 ARM processor. These efforts for designing low-latency platform is only because of the need for processing high rate information and supporting delay-bounded protocols such as Wi-Fi~\cite{}. However, IoT protocols have higher flexibility in design. For example, LoRa MAC protocols requires to support receive windows for downlink message in XXX and XXX seconds after uplink message~\cite{}. This requirement, however, is achievable with low-computation processing units which result in much simpler design compare to conventional platforms.
    
    \item {\bf Deployability.} Recent work in IoT networks~\cite{choir, netscatter} are required to deploy at large-scale to show the feasibility of new inventions in IoT network domain. However, building large-scale IoT networks with existing SDR platforms is very expensive since they are bulky in design, hardware is expensive in nature and most importantly they require power and communication backbone infrastructure. With the advent of new IoT protocols~\cite{}, the demand for a universal inexpensive platform with processing capabilities for IoT protocols increases. Table~\ref{tab:platforms} shows existing platforms and compares them in terms of size, cost and power requirement. We define large-scale deployability of a platform in terms of form-factor size, cost and infrastructure requirements. We design a cheap battery-powered SDR platform which does not require any infrastructure to operate and is optimized for IoT network research.
\squishend

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/1_platform_power/platform_pow.eps}
    \vskip -0.1in
    \caption{\footnotesize{{\bf Radio Power Consumption.} We show radio power consumption for each platform. We normalized TX power consumption for output equals to 14~dBm.\newline
    **RTL-SDR does not support transmitter mode.}}
	\label{fig:platform_power}
    \vskip -0.15in
\end{figure}

In summary, \name provides the smallest SDR solution which enables large-scale deployments for network research community at very low cost. XXX

Related work in SDR platform domain falls into two categories which we explain here.
\squishlist
    \item{\bf Commercial SDR platforms.} Ettus research is one of the world's leaders in SDR platform technologies. They provide a variety of platforms such as USRP N210~\cite{}, Embedded USRP~\cite{} and USRP networked series~\cite{}. Lime microsystem provides SDR platforms such as LimeSDR~\cite{} and LimeSDR Mini~\cite{}. Nuand is another commercial SDR provider which recently realsead bladeRF 2.0 micro SDR platform. More recently, Analog Devices has released PlutoSDR~\cite{} platform which uses AD9363~\cite{} radio front-end. Commercial SDR platforms are designed to support large spectrum frequency and provide flexibility for different applications. However, they are bulky in design, expensive and power-hungry in nature. Here, we target to build a platform for IoT network research community which provides flexibility in design while can it can be battery-powered.
    
    \item{\bf Research SDR platforms.} Over the past decade there has been multiple work on designing SDR platforms. SODA~\cite{} proposed a fully programmable SDR architecture IC simulation which meets the requirements of high-end wireless protocols and consist of four SIMD cores. KUAR~\cite{} and SORA~\cite{} are research SDR platforms that have large form-factor design and required PCI-Express connection to a host PC to operate. $\mu$SDR designed an integrated SDR that uses flash-based FPGA and AMR Cortex-M3 to process data. However, this design is power-hungry for an IoT network deployment and relatively expensive. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio~\cite{rtl2832} connected to a Raspberry pi computer. This platform can only receive signal and the receiver RF front-end is power-hungry as shown in Fig.~\ref{fig:platform_power}. XXXX
\squishend



% Conventional SDR platforms follow similar trends in design such as providing large bandwidth, supporting huge frequency bands and optimizing RF front-end noise figure for all supported frequency bands. To achieve these requirements, conventional SDR platforms use expensive RF front-end with high sampling rate and optimized noise figure for all frequency bands. For instance, LimeSDR-USB~\cite{limesdrusb} uses LMS7002M~\cite{lms7002m} RF front-end which operates at 61.44~MHz sampling rate and generates 12 bits I and Q data. Running radio front-end at high sampling rate generates high data rate of more than 1.4~GHz which requires a high sampling-rate digital design for digital signal processing. In addition, optimizing noise figure to support large bandwidth over a wide frequency spectrum significantly increases the power consumption of the RF front-end. As a result, both analog front-end and digital design for conventional SDR platforms are power-hungry. In contrast, IoT protocols such as LoRa, SigFox and NB-IoT require less than 500~kHz bandwidth. Therefore, conventional SDR platforms are over designed for implementing IoT protocols and significantly less power efficient. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio dongle~\cite{rtl2832} connected to a Raspberry pi computer. However, this platform can only receive signal and the receiver RF front-end is relatively power-hungry for a battery-free scenario.

% \noindent\name provide an SDR platform that satisfies requirements for IoT protocols. \name first version design can operate up to 2~MHz bandwidth, runs at 4~MHz sampling rate and provide 13 bits I/Q samples. Using low sampling rate with additional ADC resolution provides a low-power SDR platform which also has better sensitivity compare to existing SDR platforms. \name first design uses low-power RF front-end transceiver AT86RF215~\cite{at86rf215} from Atmel which supports three frequency bands including 900~MHz and 2.4~GHz ISM bands, consumes only 28~mA in receive mode and 40$\sim$62~mA in transmit mode. This chip cost only \$5~\cite{at86rf215digikey} while conventional SDR platforms use AD9361~\cite{ad9361digikey}, AD9364~\cite{ad9364digikey} or LMS7002M~\cite{lms7002m} RF front-ends which cost few hundred dollars.





{\footnotesize{
\centering
\vskip 0.2in
\begin{tabular}{|C{1.4cm}|C{0.8cm}|C{0.8cm}|C{1cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
	\hline \rowcolor{black}
	\centering
	{\bf\color{white}Platform}
	& {\bf\color{white}Size (inches)}
	& {\bf\color{white}Cost}+
	& {\bf\color{white}Standalone}
	& {\bf\color{white}Battery-Powered}
	& {\bf\color{white}Deployability}
	\\
	
    \hline \rowcolor{lightgray}
	{USRP E310\cite{usrpe310, ad9361digikey}} & 5.23 $\times$ 2.68 & \$3057 & \cmark & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 3.26 $\times$ 2.0 & \$733 & \cmark & \xmark& \xmark\\
	
	\hline \rowcolor{lightgray}
	{bladeRF 2.0\cite{bladerf2, ad9361digikey}} & 5.0 $\times$ 2.5 & \$720 & \cmark & \xmark& \xmark\\

	\hline \rowcolor{lightgray}
	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 3.9 $\times$ 2.36 & \$159 & \cmark & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{PlutoSDR\cite{XXX, XXX}} & XXX $\times$ XXX & \$149 & \cmark & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{$\mu$SDR\cite{XXX, XXX}} & XXX $\times$ XXX & \$150 & \cmark & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{GalioT\cite{galiot, rtl2832}} & 2.75 $\times$ 1.0 & \$60 & \cmark & \xmark & \xmark\\
	
	\hline \rowcolor{lightgray}
	{\bf{\name}} & XX $\times$ XXX & \$XX & \cmark & \cmark & \cmark\\
	
	\hline \rowcolor{lightgray}
	{\bf{\nameMini}} & XX $\times$ XXX & \$XX & \cmark & \cmark & \cmark\\
	
%     \hline \rowcolor{lightgray}
% 	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 30.72 & 61.44 & 12 & 70$\sim$6000 & 160 $\sim$ 490 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark &  & \$733\\
	
% 	\hline \rowcolor{lightgray}
% 	{bladeRF 2.0 micro xA9\cite{bladerf2, ad9361digikey}} & 30.72 & 61.44 & 12 & 47$\sim$6000 & 190 $\sim$ 410 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark & 5.0 x 2.5 & \$720\\
	
% 	\hline \rowcolor{lightgray}
% 	{LimeSDR USB \cite{limesdr, limesdrusb, lms7002m}} & 61.44 & 160 & 12 & 0.1$\sim$3800 & 420 & 350
% 	& -7 & 2 $\sim$ 2.5 & \cmark & 3.9 x 2.36 & \$300\\
	
% 	\hline \rowcolor{lightgray}
% 	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 160 & 12 & 10$\sim$3500 & 420 & 350
% 	& -7 & 2 $\sim$ 2.5 & \xmark & 2.71 x 1.23 & \$160\\
	
% 	\hline \rowcolor{lightgray}
% 	{HackRF One\cite{hackrfwiki, hackrfnoise, hackrfreview}} & 10 & 20 & 8 & 1$\sim$6000 &$>440$& 440 & 15 & 11 &
% 	\xmark & 4.72 x 2.95 & \$300\\
	
% 	\hline \rowcolor{lightgray}
% 	{GalioT\cite{galiot, rtl2832}} & 14.4 & 28.8 & 8 & 0.5$\sim$1766 & No TX & 280 & No TX & $\approx$3.5 & \xmark & 2.75 x 1.0 & \$60\\
	
% 	\hline \rowcolor{lightgray}
% 	{\bf{\name}}& 2 & 4 & 13 & \newline 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 \newline & 40 $\sim$ 62 & 28 & 14 & $<$5& \xmark & XXX x XXX & \$XX\\
	\hline
\end{tabular}
% \vskip -0.1in
\captionof{table}{\footnotesize{\bf SDR Platforms.}}
\label{tab:platforms}
}}

==> related-2.tex <==
\section{The Case for \name and Related Work}
To demonstrate that \name is the best fit for network research community to deploy large-scale IoT networks, we first need to understand what are the requirements in IoT communication protocol implementation and deployments and what are the performance parameters of currently available SDR designs in terms of these requirements. The determining performance metrics for SDR platforms used in IoT network research are power consumption, latency and deployability (xxxx why these three?). Next, we explain how previous SDR platforms perform with these metrics and argue that current they are not the optimal choice for supporting IoT wireless technologies' growth.


\squishlist
\item {\bf Latency.} 
    Many existing SDR platforms focused on designing a low-latency design. These efforts are only because of the need for processing high rate of information and supporting delay-bounded protocols such as Wi-Fi~\cite{}. However, IoT protocols have relaxed requirements in terms of latency and throughput. For example, LoRa MAC protocols requires to support receive windows for downlink message in XXX and XXX seconds after uplink message~\cite{}. \textcolor{red}{This requirement, however, is achievable with low-computation processing units which result in much simpler design compare to conventional platforms. seems weird}
    
    \item {\bf Power consumption.} Existing SDR platforms can operate at wide frequency spectrum and support up to 60~MHz bandwidth which results in using high sampling rate ADCs and DACs and more importantly high digital baseband throughput to the processing unit and computationally extensive processing unit. Moreover, they require to use radio front-ends with high sampling rate  and noise performance over large frequency spectrum and bandwidth. As a result, their whole system, radio front-end and processing unit, consumes several watts of power. Fig.~\ref{fig:platform_power} shows the power consumption of only radio module in existing SDR platforms. In contrast, IoT protocols such as LoRa, Sigfox use less than 500~kHz bandwidth and require low sampling rate of maximum 1~MHz. This means that there is an \textcolor{red}{over-designed} gap between the current SDR designs and what is required for IoT communication protocol implementation. Fig.~\ref{fig:platform_power} shows that these platforms use power-hungry RF front-ends which consumes in the order of few watts of power in transmit mode and few hundred milliwatts of power in receive mode. High power consuming radios are not suitable for a battery-powered SDR platform which is the our target for large-scale research deployments. These requirements lead us to rethink existing SDR solutions and optimize them for IoT protocols. We design and build \name that is low-power and last XXX years using only a XXX battery.
    
    % \item {\bf Bandwidth.} Conventional SDR platform are designed to support huge sampling rate and bandwidth. These platforms support wide-band frequency spectrum and more than 20~MHz bandwidth to support different 802.11 standards. In contrast, IoT protocols such as LoRa, Sigfox and etc. use less than 500~kHz bandwidth and operate at low sampling rate. This requirements lead us to redesigning existing SDR solutions and optimizing them for IoT protocols. We design \name platform based on requirements of existing IoT protocols.  

    \item {\bf Deployability.} IoT communication network protocols are needed to be implemented at large-scale to be fully evaluated and show their potential~\cite{choir, netscatter}. However, building large-scale IoT networks with existing SDR platforms involves multiple challenges because of their large form-factor, expensive hardware, high power and processing backbone infrastructure. With the advent of new IoT protocols~\cite{}, the demand for a universal inexpensive platform with processing capabilities supporting IoT protocols increases. Table~\ref{tab:platforms} shows existing platforms and compares them in terms of size, cost and power requirement. We define large-scale deployability of a platform in terms of form-factor size, cost and infrastructure requirements. As shown in the Table~\ref{tab:platforms}, none of the previous platforms satisfy the requirements of deployability while \name is cheap, small form-factor, battery-powered and without any need for backbone infrastructure which makes it deployable and optimal fit for IoT network research.    
\squishend

In summary, \name provides the smallest SDR solution which enables large-scale deployments for network research community at very low cost. XXX

Related work in SDR platform domain falls into two categories which we explain here.
\squishlist
    \item{\bf Commercial SDR platforms.} Ettus research is one of the world's leaders in SDR platform technologies. They provide a variety of platforms such as USRP N210~\cite{}, Embedded USRP~\cite{} and USRP networked series~\cite{}. USRP uses peripheral buses such as USB or Ethernet to connect to a computer with operating system for its controlling signal. Embedded USRP E310 benefits from a Dual Core ARM A9 processor for processing high data-rate information. Lime microsystems provides SDR platforms such as LimeSDR~\cite{} and LimeSDR Mini~\cite{}. Nuand is another commercial SDR provider which recently realsead bladeRF 2.0 micro SDR platform. More recently, Analog Devices has released PlutoSDR~\cite{} platform which uses AD9363~\cite{} radio front-end. Commercial SDR platforms are designed to support large spectrum frequency and provide flexibility for different applications. However, they are bulky in design, expensive and power-hungry in nature. Here, we target to build a platform for IoT network research community which provides flexibility in design while can it can be battery-powered.
    
    \item{\bf Research SDR platforms.} Over the past decade there has been multiple works on designing SDR platforms.  Tick~\cite{} achieves good programmability, high throughput and low latency by software-hardware co-design solutions. However, it uses a high power radio on the order of several watts~\cite{AD9371} and the whole design costs more than 3000 dollars. SORA~\cite{sora} is research platform that uses PCI-Express bus to provide sub 1~$\mu$s latency. However, it requires host PC for backbone processing and hence large form-factor. $\mu$SDR solves the latency challenge by using an advanced microcontroller bus architecture (AMBA) along with a Cortex-M3 ARM processor~\cite{musdr} and flash-based FPGA to process data. However, it is power-hungry for an IoT network deployment and relatively expensive. SODA~\cite{} proposed a fully programmable SDR architecture IC simulation which meets the requirements of high-end wireless protocols and consist of four SIMD cores. However, it has a slightly customized VLIW+SIMD ISA which needs users to hand-tune their program. KUAR~\cite{} is a research SDR platform that have large form-factor design and required PCI-Express connection to a host an embedded PC-like environment to operate. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio~\cite{rtl2832} connected to a Raspberry pi computer. This platform can only receive signal and the receiver RF front-end is power-hungry as shown in Fig.~\ref{fig:platform_power}. XXXX
\squishend


% Conventional SDR platforms follow similar trends in design such as providing large bandwidth, supporting huge frequency bands and optimizing RF front-end noise figure for all supported frequency bands. To achieve these requirements, conventional SDR platforms use expensive RF front-end with high sampling rate and optimized noise figure for all frequency bands. For instance, LimeSDR-USB~\cite{limesdrusb} uses LMS7002M~\cite{lms7002m} RF front-end which operates at 61.44~MHz sampling rate and generates 12 bits I and Q data. Running radio front-end at high sampling rate generates high data rate of more than 1.4~GHz which requires a high sampling-rate digital design for digital signal processing. In addition, optimizing noise figure to support large bandwidth over a wide frequency spectrum significantly increases the power consumption of the RF front-end. As a result, both analog front-end and digital design for conventional SDR platforms are power-hungry. In contrast, IoT protocols such as LoRa, SigFox and NB-IoT require less than 500~kHz bandwidth. Therefore, conventional SDR platforms are over designed for implementing IoT protocols and significantly less power efficient. GalioI~\cite{galiot} presents an SDR platform including a RTL2832U radio dongle~\cite{rtl2832} connected to a Raspberry pi computer. However, this platform can only receive signal and the receiver RF front-end is relatively power-hungry for a battery-free scenario.

% \noindent\name provide an SDR platform that satisfies requirements for IoT protocols. \name first version design can operate up to 2~MHz bandwidth, runs at 4~MHz sampling rate and provide 13 bits I/Q samples. Using low sampling rate with additional ADC resolution provides a low-power SDR platform which also has better sensitivity compare to existing SDR platforms. \name first design uses low-power RF front-end transceiver AT86RF215~\cite{at86rf215} from Atmel which supports three frequency bands including 900~MHz and 2.4~GHz ISM bands, consumes only 28~mA in receive mode and 40$\sim$62~mA in transmit mode. This chip cost only \$5~\cite{at86rf215digikey} while conventional SDR platforms use AD9361~\cite{ad9361digikey}, AD9364~\cite{ad9364digikey} or LMS7002M~\cite{lms7002m} RF front-ends which cost few hundred dollars.





% {\footnotesize{
% \centering
% \vskip 0.2in
% \begin{tabular}{|C{1cm}|C{0.8cm}|C{0.6cm}|C{1.5cm}|C{1cm}|C{0.6cm}|C{1cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
% 	\hline \rowcolor{black}
% 	\centering
% 	{\bf\color{white}Platform}
% 	& {\bf\color{white}Max BW}
% 	& {\bf\color{white}ADC}
% 	& {\bf\color{white}Frequency Spectrum}
% 	& {\bf\color{white}Size (inches)}
% 	& {\bf\color{white}Cost}
% 	& {\bf\color{white}Battery-Powered}
% 	& {\bf\color{white}Deployability}
% 	\\
	
%     \hline \rowcolor{lightgray}
% 	{USRP E310~\cite{usrpe310, ad9361digikey}} & XXX & XXX & XXX & 5.23 $\times$ 2.68 & \$3057 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{USRP B200mini~\cite{usrpb200mini, ad9364digikey}} & 3.26 $\times$ 2.0 & \$733 & \cmark & \xmark& \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{bladeRF 2.0~\cite{bladerf2, ad9361digikey}} & 5.0 $\times$ 2.5 & \$720 & \cmark & \xmark& \xmark\\

% 	\hline \rowcolor{lightgray}
% 	{LimeSDR Mini~\cite{limesdr, limesdrmini, lms7002m}} & 3.9 $\times$ 2.36 & \$159 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{PlutoSDR~\cite{XXX, XXX}} & XXX $\times$ XXX & \$149 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{$\mu$SDR~\cite{XXX, XXX}} & XXX $\times$ XXX & \$150 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{GalioT~\cite{galiot, rtl2832}} & 2.75 $\times$ 1.0 & \$60 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{\bf{\name}} & XX $\times$ XXX & \$XX & \cmark & \cmark & \cmark\\
	
% %     \hline \rowcolor{lightgray}
% % 	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 30.72 & 61.44 & 12 & 70$\sim$6000 & 160 $\sim$ 490 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark &  & \$733\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{bladeRF 2.0 micro xA9\cite{bladerf2, ad9361digikey}} & 30.72 & 61.44 & 12 & 47$\sim$6000 & 190 $\sim$ 410 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark & 5.0 x 2.5 & \$720\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{LimeSDR USB \cite{limesdr, limesdrusb, lms7002m}} & 61.44 & 160 & 12 & 0.1$\sim$3800 & 420 & 350
% % 	& -7 & 2 $\sim$ 2.5 & \cmark & 3.9 x 2.36 & \$300\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 160 & 12 & 10$\sim$3500 & 420 & 350
% % 	& -7 & 2 $\sim$ 2.5 & \xmark & 2.71 x 1.23 & \$160\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{HackRF One\cite{hackrfwiki, hackrfnoise, hackrfreview}} & 10 & 20 & 8 & 1$\sim$6000 &$>440$& 440 & 15 & 11 &
% % 	\xmark & 4.72 x 2.95 & \$300\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{GalioT\cite{galiot, rtl2832}} & 14.4 & 28.8 & 8 & 0.5$\sim$1766 & No TX & 280 & No TX & $\approx$3.5 & \xmark & 2.75 x 1.0 & \$60\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{\bf{\name}}& 2 & 4 & 13 & \newline 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 \newline & 40 $\sim$ 62 & 28 & 14 & $<$5& \xmark & XXX x XXX & \$XX\\
% 	\hline
% \end{tabular}
% % \vskip -0.1in
% \captionof{table}{\footnotesize{\bf SDR Platforms.}}
% \label{tab:platforms}
% }}

% \begin{figure*}

% \begin{minipage}[b]{\textwidth}

%   {\footnotesize{
% \centering
% \vskip 0.2in
% \begin{tabular}{|C{1cm}|C{0.8cm}|C{0.6cm}|C{1.5cm}|C{1cm}|C{0.6cm}|C{1cm}|C{1cm}|C{1cm}|} %c|c|>{\centering}m{2cm}|c|}
% 	\hline \rowcolor{black}
% 	\centering
% 	{\bf\color{white}Platform}
% 	& {\bf\color{white}Max BW}
% 	& {\bf\color{white}ADC}
% 	& {\bf\color{white}Frequency Spectrum}
% 	& {\bf\color{white}Size (inches)}
% 	& {\bf\color{white}Cost}
% 	& {\bf\color{white}Battery-Powered}
% 	& {\bf\color{white}Deployability}
% 	\\
	
%     \hline \rowcolor{lightgray}
% 	{USRP E310~\cite{usrpe310, ad9361digikey}} & XXX & XXX & XXX & 5.23 $\times$ 2.68 & \$3057 & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{USRP B200mini~\cite{usrpb200mini, ad9364digikey}} & 3.26 $\times$ 2.0 & \$733 & \cmark & \xmark& \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{bladeRF 2.0~\cite{bladerf2, ad9361digikey}} & 5.0 $\times$ 2.5 & \$720 & \cmark & \xmark& \xmark\\

% 	\hline \rowcolor{lightgray}
% 	{LimeSDR Mini~\cite{limesdr, limesdrmini, lms7002m}} & 3.9 $\times$ 2.36 & \$159 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{PlutoSDR~\cite{XXX, XXX}} & XXX $\times$ XXX & \$149 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{$\mu$SDR~\cite{XXX, XXX}} & XXX $\times$ XXX & \$150 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{GalioT~\cite{galiot, rtl2832}} & 2.75 $\times$ 1.0 & \$60 & \cmark & \xmark & \xmark\\
	
% 	\hline \rowcolor{lightgray}
% 	{\bf{\name}} & XX $\times$ XXX & \$XX & \cmark & \cmark & \cmark\\
	
% %     \hline \rowcolor{lightgray}
% % 	{USRP B200mini\cite{usrpb200mini, ad9364digikey}} & 30.72 & 61.44 & 12 & 70$\sim$6000 & 160 $\sim$ 490 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark &  & \$733\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{bladeRF 2.0 micro xA9\cite{bladerf2, ad9361digikey}} & 30.72 & 61.44 & 12 & 47$\sim$6000 & 190 $\sim$ 410 & 180 $\sim$ 260 & 7 & 2 $\sim$ 3 & \cmark & 5.0 x 2.5 & \$720\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{LimeSDR USB \cite{limesdr, limesdrusb, lms7002m}} & 61.44 & 160 & 12 & 0.1$\sim$3800 & 420 & 350
% % 	& -7 & 2 $\sim$ 2.5 & \cmark & 3.9 x 2.36 & \$300\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{LimeSDR Mini \cite{limesdr, limesdrmini, lms7002m}} & 30.72 & 160 & 12 & 10$\sim$3500 & 420 & 350
% % 	& -7 & 2 $\sim$ 2.5 & \xmark & 2.71 x 1.23 & \$160\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{HackRF One\cite{hackrfwiki, hackrfnoise, hackrfreview}} & 10 & 20 & 8 & 1$\sim$6000 &$>440$& 440 & 15 & 11 &
% % 	\xmark & 4.72 x 2.95 & \$300\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{GalioT\cite{galiot, rtl2832}} & 14.4 & 28.8 & 8 & 0.5$\sim$1766 & No TX & 280 & No TX & $\approx$3.5 & \xmark & 2.75 x 1.0 & \$60\\
	
% % 	\hline \rowcolor{lightgray}
% % 	{\bf{\name}}& 2 & 4 & 13 & \newline 389.5$\sim$510 779$\sim$1020 2400$\sim$2483 \newline & 40 $\sim$ 62 & 28 & 14 & $<$5& \xmark & XXX x XXX & \$XX\\
% 	\hline
% \end{tabular}
% % \vskip -0.1in
% \captionof{table}{\footnotesize{\bf SDR Platforms.}}
% \label{tab:platforms}
% }}

% \end{minipage}
% \end{figure*}

\begin{table}[htb]%\[!htb\]
    \caption{Global caption}
    \begin{subtable}[t]{.5\textwidth}
        \caption{This is a very very very long Caption}
        \raggedright
            \begin{tabular}{@{\extracolsep{1pt}}lcccc}
                \hline\hline \\
                Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\
                \hline \\
                A & 1.000 & 0.000 & 1     & 1 \\
                B & 0.968 & 0.76  & 0.138 & 1.000 \\
                C & 0.969 & 0.009 & 0.917 & 1.000 \\
                D & 0.966 & 0.070 & 0.495 & 0.83 \\
                \hline \\
            \end{tabular}
    \end{subtable}%
   \begin{subtable}[t]{.5\textwidth}
        \raggedleft
        \caption{This is a very very very long Caption}
        \begin{tabular}{@{\extracolsep{1pt}}lcccc}
            \hline\hline \\
        Statistic & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Max} \\
        \hline \\
                A & 1.000 & 0.000 & 1     & 1 \\
                B & 0.968 & 0.76  & 0.138 & 1.000 \\
                C & 0.969 & 0.009 & 0.917 & 1.000 \\
                D & 0.966 & 0.070 & 0.495 & 0.83 \\
        \hline \\
        \end{tabular}
    \end{subtable}
\end{table}

==> results-1.tex <==

\subsection{Network Deployments}\label{sec:deploy}
%Next, we describe our two deployment results.  
We evaluate three key network parameters: 
\squishlist
\item {\it Network PHY bit-rate.} This is the bit rate achieved across all the end-devices during the payload part of the packet.
\item {\it Link-layer data rate.} This is the data rate achieved in the network which is defined as the data rate for sending useful payload bits, after considering overheads including the AP's query message and the preamble of the packet transmission.
\item {\it Network latency.} This is the latency to successfully get the payload bits from all the end-devices in the network. 
\squishend

\subsubsection{Backscatter deployment}\label{sec:back_deploy}
 We set each \tagname bit-rate to 1~kbps, $BW_{agg}=500~KHz$, $SF=9$ and a payload size of five bytes. With the above settings and considering the $\Delta FFT_{bin}$ results shown in Fig.~\ref{fig:fft_var}, the number of empty cyclic shifts is one corresponding to $SKIP=2$ in our design. This means that our network supports {256} \tagnames talking concurrently. We deploy these backscatter end-devices across the floor of an office building with more than eight rooms.\footnote{{Note that RFID EPC-Gen2 readers' receiver decoding sensitivity is -85~dBm~\cite{rfidReader} for battery-powered backscatter tags. With BW=500~kHz and SF=9, the sensitivity for CSS modulation is -123~dBm. This 38~dB gain 
allows CSS-based backscatter systems to support long ranges and deployments that are not possible with EPC-Gen2.}}
%  \footnote{In Fig.~\ref{sec:related} we show throughput results in the same deployment for {\it battery-powered} RFID EPC-GEN2 protocol and show that XX\% of the locations achieve a zero throughput. This is because EPC-GEN2 cannot support the ranges in our deployment since they have a limited sensitivity of XX~dBm. In contrast, CSS modulation can operate at sensitivities as low as XX~dBm.}

\begin{figure*}[t]
	\begin{subfigure}{0.32\linewidth}
    	\centering
    	\includegraphics[width=1.05\linewidth]{./figs/12_active_dataRate_latency/phy_rate_bar.eps}
		\label{fig:active_phy}
        \vskip -0.25in
        \caption{Network Physical Rate}
	\end{subfigure}
    \begin{subfigure}{0.32\linewidth}
    	\centering
    	\includegraphics[width=1.05\linewidth]{./figs/12_active_dataRate_latency/link_rate_bar.eps}
		\label{fig:active_link}
        \vskip -0.25in
        \caption{Link-layer Data Rate}
	\end{subfigure}
    \begin{subfigure}{0.32\linewidth}
    	\centering
    	\includegraphics[width=1.05\linewidth]{./figs/12_active_dataRate_latency/latency_bar.eps}
		\label{fig:activ_latency}
        \vskip -0.25in
        \caption{Latency}
	\end{subfigure}
	\vskip -0.15in
\caption{{\bf Wide-Area Radio Deployment.} We evaluate network physical rate, link-layer data rate and latency for \nameDesign and compare it with Choir.}
	\label{fig:active_link_rate}
    \vskip -0.15in
\end{figure*}

We compare three schemes: i) LoRa backscatter~\cite{lorabackscatter}, ii) LoRa backscatter with rate adaptation and iii) \nameDesign.  Note that the authors of~\cite{lorabackscatter} did not publicly release the code and so, we replicate the implementation adding the missing details  and using  $BW=500~KHz$ and $SF=9$. We also note that ~\cite{lorabackscatter} is not designed to work with more than one user. Here, we use TDMA with scheduling when there are more users where the AP queries each end-devices. While LoRa backscatter does not support rate adaptation, we wanted to compare with an ideal approach  that maximizes the bit-rate of each end-device by picking the optimal SF and BW. To do so, we measure RSSI from each of the backscatter  \tagnames and compute the bit rate  using the SNR table in~\cite{lora1276}.

Fig.~\ref{fig:passive_link_rate} shows the results for our backscatter network deployment. The plots show that with 256 backscatter end-devices, \nameDesign increases the PHY bit-rate by 6.8x and 26.2x over LoRa backscatter with and without rate adaptation. The gains are lower with the ideal rate adaptation since  it could pick the maximum LoRa bit rate of 32~Kbps. We also note that \nameDesign sets the bit rate of each end-device to 1~kbps and hence has better gains as the number of end-devices increase.  Further, the gains at the link-layer are however higher for \nameDesign at 20x and 98.5x respectively. This is because, in \nameDesign, the added overhead of sending AP's query and \tagnames' preambles happen once and at the same time for all \tagnames. But the other schemes need to do TDMA which means that sending query and preamble will not happen concurrently for all \tagnames. 
Finally, \nameDesign has a latency reduction of 21.8x and 106x over the other approaches. %This is the key advantage of using concurrent transmissions in low-power networks. 


\subsubsection{Wide-Area Radio Deployment}\label{sec:wi}
Unlike backscatter devices which can be deployed within a single building, the logistics of deploying 256 radio end-devices across the campus is prohibitive in terms of {man-power as well as the time that it takes}. Instead we emulate a 256 node network across the campus by moving 10 radio \tagnames  across 256 different locations across the campus. Note that the actual technical feasibility of \nameDesign at scale has already been demonstrated in the backscatter experiments, so these set of experiments are for completeness.
%Next we deploy \nameDesign across a metropolitan area.


Specifically, to emulate a network of {256} \tagnames, we do 26 different deployments across campus and record the results using USRP. Each deployment involves all ten radio \tagnames. Moreover, the spatial locations and cyclic shifts assigned to the \tagnames in each deployment is different from other deployments. Note that, we assign \tagnames based on ~\xref{sec:nearfar} at different power levels and they use the power adjustment to stay within that power level after deployment. We then time-synchronize and combine the time-domain recordings across all these 26 deployments. We input this addition result to the \nameDesign decoder and decode all the concurrent 256 \tagnames. A question the reader might have is: If we have a network involving {256} \tagnames, would the result of the USRP recording be the same as our combined deployment results? For a linear system, adding two inputs will result in an output which is equal to adding their corresponding outputs. Since the end-devices are far from the AP and a have weak signal strength, the analog front-end of the USRP is far from being saturated and works in linear region. This means that, the addition of the USRP recordings of different deployments is functionally similar as a recording of deployment which involves all the \tagnames.

We compare \nameDesign with Choir~\cite{lorasigcomm17} which enables up to ten concurrent LoRa transmissions. To support more than 10 transmissions in Choir, we again use TDMA where the AP sends a query message to different sets of ten transmitters. Fig.~\ref{fig:active_link_rate} shows the results for our deployment. Note that each node in Choir transmits an average of 9~kbps and since it can support up to ten concurrent transmissions, our gains are more prominent with a large number of \tagnames. Further, when the number of \tagnames is less than 90, Choir can outperform \nameDesign since the latter requires a large number of users to fully utilizes the network capacity. With 256 \tagnames, the PHY and link-layer gains over Choir (LoRa TDMA with rate adaptation) for \nameDesign was 2.5x (4.1x) and 4.8x (27.8x) respectively. Also, with corresponding latency reduction is around 5.4x (30.1x) which is significant in practical networks. Note that, for clarity of comparison between \nameDesign and Choir, Fig.~\ref{fig:active_link_rate} does not include the results of the LoRa TDMA.


% In following sections, first we compare the performance of \nameshort~with other method. Then, we evaluate the overall throughput of our network and compare it with existing methods.
% \subsubsection{\nameshort Performance per \tagName}
% Here, we compare the performance of one \tagname~in \nameshort~with existing methods such as FlipTracer\cite{fliptracer} and LF-Backscatter\ref{lfbackscatter} which are using EPCglobal~Gen2 protocol at 100~Kbps. We assume that we have a deployment of 250 \tagnames, where we implement different methods. Then we evaluate throughput for each \tagname. Fig.~\ref{fig:throughput_tag} shows the CDF of PHY-Layer throughput per \tagname~for 250 \tagnames. As this figure shows, FlipTracer and LF-Backscatter only support up to five and sixteen concurrent transmissions, respectively. This result show that in existing methods, 98~\% and 93~\% of the \tagnames~has throughput of near to zero. However, \nameshort~can guarantee $\approx$~1~Kbps throughput for all \tagnames.

% \subsubsection{Operation Range}
% In this section, we evaluate the performance of \nameshort~at different ranges. 


% \subsection{Performance of \nameshort}

==> system-1.tex <==
\section{System Design}
% -whole view explanation of our design

% -block diagram

% -explain all components

% -design requirements and decisions: why we use such a low bandwidth, why SD card? why

% -Why this FPGA?

% -why this radio? BW, power, IQ output, compare with other radios in power and SR. Frequency bands

%

\begin{figure}[t]
    \centering
	\includegraphics[width=0.2\linewidth]{./figs/sdr_hardware.png}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}
\textcolor{red}{write it based on the Mobicom paper}
In this section, we go over the PHY and MAC layer design of the \name system and present design choices and considerations.

\subsection{PHY Layer}
In this section, we go over the different parts of the \name system and present design choices and considerations. \name platform is composed of analog front-end, FPGA, MCU, sensor interface and microSD card interface. Fig.~\ref{fig:block_diagram} shows the block diagram of the \name platform. 
In the receive chain, analog front-end receives RF signal and provides I/Q signal to the FPGA for base-band processing. The transmit chain works in the opposite direction meaning that the I/Q signal will be upconverted to RF frequency to send it over the antenna. FPGA does baseband modulation and demodulation. MCU provides sensor interface, controls the analog front-end and power management unit (PMU). We provision microSD card to record raw I/Q samples and packet information for research projects that need data collection.

\subsection{Analog Front-End}
The RF front-end is based on AT86RF215~\cite{ref:AT86RF215} from Microchip which can operate in 400~MHz, 900~MHz and 2.4~GHz frequency bands which makes this design suitable for these ISM bands xxxx and is capable of exchanging digitized raw I/Q samples with the baseband processing unit. This chip provides all the necessary blocks of the transceiver chain from the antenna to the digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, synthesizer and voltage-controlled oscillator. To exchange digitized I/Q baseband data between the baseband processing block, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. Note that, most IoT communication protocols have low bandwidth xxxx (e.g. LoRa, SigFox \cite{xxxx}). Moreover, the digital analog baseband front-end, ADC/DAC, has 13 bits which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP \cite{xxxx}. In addition, the low bandwidth and sampling rate of this chip makes it low power so that it can be run out of a battery. Fig. \ref{fig:} shows the power consumption comparison of this transceiver compared to other transceivers that are used in similar products. As mentioned in ~\xref{sec:case}, our goal is to enable inexpensive SDR platform. Our other consideration in choosing this chip is its very low price of less than 5 dollars. In summary, AT86RF215 satisfies all the requirements of the wide-spread inexpensive SDR for IoT applications.
- explain the LVDS part
- explain different options for control

\subsection{Processing Unit}
The processing is composed of FPGA and MCU and is responsible for communication protocol implementation including modulation and demodulation and MAC layer. FPGA is responsible for doing modulationa and demodulation and MCU for MAC layer implementation. We selected FPGA by analyzing different IoT communication protocols’ receiver algorithm, FPGA computational resource needed to enable these algorithms and also computational resource needed to do localization xxxx. Moreover, it needs to support LVDS interface to be able to talk to the transceiver chip. We have used M2GL010T from IGLOO 2 series of Microsemi for our first prototype. We chose MSP430FR5969 from TI MSP430 series for MCU because of its power performance.

\subsection{Control Unit}
As shown in Fig. \ref{xx}, the other block that we have used in our design is control unit which is implemented on a low power MSP430~\cite{xxxx} MCU. This unit serves multiple purposes. First, it talks to the radio to adjust its settings including synthesizer frequency, analog front-end gain, TX transmit power,sampling rate, filtering parameters and etc. depending on the application and communication protocol. Moreover, it talks to the power management unit to set voltage supply of different blocks and optimize them to minimize power consumption. In addition, it provides different communication interfaces (SPI, I2C and ...) to talk to different sensors that may need to be added.

\subsection{MicroSD Card}
The purpose of this unit is to enable recording high amounts of data (e.g. raw I/Q data or baseband bits) for later post-processing. MicroSD cards provide two modes of communication to the host: 1- xxxx 2- SPI based communication. The SPI-based communication is much simpler than the first option and can provide around xxxx~Mbps. To fast prototype our design, we have implemented the SPI-based communication between the FPGA and the MicroSD card.




==> system-2.tex <==
\section{System Design}
% -whole view explanation of our design

% -block diagram

% -explain all components

% -design requirements and decisions: why we use such a low bandwidth, why SD card? why

% -Why this FPGA?

% -why this radio? BW, power, IQ output, compare with other radios in power and SR. Frequency bands

%

\begin{figure}[t]
    \centering
	\includegraphics[width=0.2\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}
In this section, first, we go over the PHY and MAC layer design and implementations of the \name system and present design choices and considerations. Next, we explain the microSD card interface and sensor interface that has been added to enable the system to act as a sensor node and increase its functionality. Fig.~\ref{fig:block_diagram} shows the block diagram of the \name platform.

\subsection{PHY Layer}
\name platform's PHY layer is composed of analog front-end and FPGA. In the receive chain, analog front-end receives RF signal and provides I/Q signal to the FPGA for base-band processing, modulation and demodulation. The transmit chain works in the opposite direction meaning that the I/Q signal will be upconverted to RF frequency to send it over the antenna. 


\squishlist
    \item {\bf Analog Front-End.} 
    The RF front-end is based on AT86RF215~\cite{ref:AT86RF215} from Microchip which can operate in 400~MHz, 900~MHz and 2.4~GHz frequency bands which makes this design suitable for these ISM bands xxxx and is capable of exchanging digitized raw I/Q samples with the baseband processing unit. This chip provides all the necessary blocks of the transceiver chain from the antenna to the digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, synthesizer and voltage-controlled oscillator. To exchange digitized I/Q baseband data between the baseband processing block, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. Note that, most IoT communication protocols have low bandwidth of 500~KHz (e.g. LoRa, SigFox \cite{xxxx}). Moreover, the digital analog baseband front-end, ADC/DAC, has 13 bits which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP \cite{xxxx}. \textcolor{red}{the low bandwidth and sampling rate xxxx, mention it or not?}. Fig. \ref{fig:} compares power consumption this transceiver with other transceivers that are used in existing products. As can be seen, power consumption is more than \textcolor{red}{5 xxx} times less than the closest SDR platform. \textcolor{red}{Moreover, the price of this transceiver chip is less than 5 dollars which makes this design very low cost.} In summary, AT86RF215 satisfies all the requirements of the wide-spread cheap SDR for IoT applications.

    \item {\bf Baseband-Processing Unit.}
    The processing is composed of FPGA and MCU and is responsible for communication protocol implementation including modulation and demodulation and MAC layer. FPGA is responsible for doing modulationa and demodulation and MCU for MAC layer implementation. We selected FPGA by analyzing different IoT communication protocols’ receiver algorithm, FPGA computational resource needed to enable these algorithms and also computational resource needed to do localization xxxx. Moreover, it needs to support LVDS interface to be able to talk to the transceiver chip. We have used M2GL010T from IGLOO 2 series of Microsemi for our first prototype. We chose MSP430FR5969 from TI MSP430 series for MCU because of its power performance.
\squishend

MCU provides sensor interface, controls the analog front-end and power management unit (PMU). We provision microSD card to record raw I/Q samples and packet information for research projects that need data collection.


\subsection{MAC Layer}
As shown in Fig. \ref{xx}, the other block that we have used in our design is control unit which is implemented on a low power MSP430~\cite{xxxx} MCU. This unit serves multiple purposes. First, it talks to the radio to adjust its settings including synthesizer frequency, analog front-end gain, TX transmit power,sampling rate, filtering parameters and etc. depending on the application and communication protocol. Moreover, it talks to the power management unit to set voltage supply of different blocks and optimize them to minimize power consumption. In addition, it provides different communication interfaces (SPI, I2C and ...) to talk to different sensors that may need to be added.

\subsection{MicroSD Card}
The purpose of this unit is to enable recording high amounts of data (e.g. raw I/Q data or baseband bits) for later post-processing. MicroSD cards provide two modes of communication to the host: 1- xxxx 2- SPI based communication. The SPI-based communication is much simpler than the first option and can provide around xxxx~Mbps. To fast prototype our design, we have implemented the SPI-based communication between the FPGA and the MicroSD card.




==> system-3.tex <==
\section{System Design}
% -whole view explanation of our design

% -block diagram

% -explain all components

% -design requirements and decisions: why we use such a low bandwidth, why SD card? why

% -Why this FPGA?

% -why this radio? BW, power, IQ output, compare with other radios in power and SR. Frequency bands

%

\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}
In this section, first, we go over the PHY and MAC layer design and implementations of the \name system and present design choices and considerations. Next, we explain the microSD card interface and sensor interface that has been added to enable the system to act as a sensor node and increase its functionality. Fig.~\ref{fig:block_diagram} shows the block diagram of the \name platform.

\subsection{PHY Layer}
\name platform's PHY layer is composed of analog front-end and FPGA. In the receive chain, analog front-end receives RF signal and provides I/Q signal to the FPGA for base-band processing, modulation and demodulation. The transmit chain works in the opposite direction meaning that the I/Q signal will be upconverted to RF frequency to send it over the antenna. 


\squishlist
    \item {\bf Analog Front-End.} 
    The RF front-end is based on AT86RF215~\cite{ref:AT86RF215} from Microchip which can operate in 400~MHz, 900~MHz and 2.4~GHz frequency bands which makes this design suitable for these ISM bands xxxx and is capable of exchanging digitized raw I/Q samples with the baseband processing unit. This chip provides all the necessary blocks of the transceiver chain from the antenna to the digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, synthesizer and voltage-controlled oscillator. To exchange digitized I/Q baseband data between the baseband processing block, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. Note that, most IoT communication protocols have low bandwidth of 500~KHz (e.g. LoRa, SigFox \cite{xxxx}). Moreover, the digital analog baseband front-end, ADC/DAC, has 13 bits which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP \cite{xxxx}. \textcolor{red}{the low bandwidth and sampling rate xxxx, mention it or not?}. Fig. \ref{fig:} compares power consumption this transceiver with other transceivers that are used in existing products. As can be seen, power consumption is more than \textcolor{red}{5 xxx} times less than the closest SDR platform. \textcolor{red}{Moreover, the price of this transceiver chip is less than 5 dollars which makes this design very low cost.} In summary, AT86RF215 satisfies all the requirements of the wide-spread cheap SDR for IoT applications.

    \item {\bf Baseband-Processing Unit.}
    The processing is composed of FPGA and MCU and is responsible for communication protocol implementation including modulation and demodulation and MAC layer. FPGA is responsible for doing modulationa and demodulation and MCU for MAC layer implementation. We selected FPGA by analyzing different IoT communication protocols’ receiver algorithm, FPGA computational resource needed to enable these algorithms and also computational resource needed to do localization xxxx. Moreover, it needs to support LVDS interface to be able to talk to the transceiver chip. We have used M2GL010T from IGLOO 2 series of Microsemi for our first prototype. We chose MSP430FR5969 from TI MSP430 series for MCU because of its power performance.
\squishend

MCU provides sensor interface, controls the analog front-end and power management unit (PMU). We provision microSD card to record raw I/Q samples and packet information for research projects that need data collection.


\subsection{MAC Layer}
As shown in Fig. \ref{xx}, the other block that we have used in our design is control unit which is implemented on a low power MSP430~\cite{xxxx} MCU. This unit serves multiple purposes. First, it talks to the radio to adjust its settings including synthesizer frequency, analog front-end gain, TX transmit power,sampling rate, filtering parameters and etc. depending on the application and communication protocol. Moreover, it talks to the power management unit to set voltage supply of different blocks and optimize them to minimize power consumption. In addition, it provides different communication interfaces (SPI, I2C and ...) to talk to different sensors that may need to be added.

\subsection{MicroSD Card}
The purpose of this unit is to enable recording high amounts of data (e.g. raw I/Q data or baseband bits) for later post-processing. MicroSD cards provide two modes of communication to the host: 1- xxxx 2- SPI based communication. The SPI-based communication is much simpler than the first option and can provide around xxxx~Mbps. To fast prototype our design, we have implemented the SPI-based communication between the FPGA and the MicroSD card.

\subsection{Over-the-Air Update}

\subsection{Protocols}

\subsubsection{LoRa}

\subsubsection{Zigbee}


==> system-4.tex <==
\section{System Design}\label{sec:system}
%Explain more on the high-level: - Why are we doing this having IoTLab in mind?: --Duty-cycling --over the air update --flexibility
% -whole view explanation of our design

% -block diagram

% -explain all components

% -design requirements and decisions: why we use such a low bandwidth, why SD card? why

% -Why this FPGA?

% -why this radio? BW, power, IQ output, compare with other radios in power and SR. Frequency bands

%

\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}

The \name system is designed to fulfill the vision of an SDR based IoT testbed. In particular, \name system has flexible PHY and MAC layer, is capable of updating over the air (OTA) and low power. In this section, we explain the design of the \name system and present design choices and considerations. As shown in fig.~\ref{fig:system}, the system is divided to six different functional blocks: i) PHY layer, ii) MAC layer and central control, iii) Power Management Unit (PMU), iv) storage devices, v) sensor interface, and vi) OTA update unit.


\begin{figure}[t]
    \centering
	\includegraphics[width=1\linewidth]{figs/block_diagram/system.eps}
	\caption{\footnotesize{\name system block diagram.}}
	\label{fig:system}
\end{figure}

% This subsection should go to the end since it controls all
% Explain duty-cycling
\subsection{MAC Layer and Central Control Unit}
The MAC layer controls channel access between different transceivers on the medium. In \name design, it is implemented on an MCU. Note that, since \name is designed for IoT protocols testing and implementation, it has relaxed latency requirements. This means there is no stringent timing requirement on the communication link between the PHY and MAC layer. MCU is the central controller of the system and in addition to hosting the MAC layer it controls sensor interfaces, OTA update process and all necessary functions to increase the battery life-time including duty-cycling and power-gating of different blocks.

transforms information bits into a radio waveform,
or vice versa. PHY has both control and data flows. The control
flow is relatively simple. It sets configuration parameters. 

\subsection{PHY Layer}
The job of PHY layer is to convert data to RF signal on the transmit side and vice versa on the receive side. It is composed of RF front-end and baseband processing. On the transmit chain, FPGA gets data, does encoding and modulation and feeds it to the RF front-end to transfrom it to RF signal. On the receive side, RF front-end receives RF signal and sends it FPGA for decoding and demodualtion. The combination of a RF front-end capable of exchanging I/Q samples with an FPGA provides us with a flexible PHY layer. MCU controls the settings of this layer.


% The RF front-end IC does all the necessary functions to tra. This RF IC exchanges digitized baseband raw I/Q data with the baseband processing unit which is implemented on an FPGA and does modulation, demodulation, source and channel encoder and decoder.
% in RF side including low noise amplification, power amplification, upconversion and downconversion mixing and also A/D and D/A conversion




% \squishlist
%     \item {\bf Analog Front-End.} 
%     The RF front-end is based on AT86RF215~\cite{ref:AT86RF215} from Microchip which can operate in 400~MHz, 900~MHz and 2.4~GHz frequency bands which makes this design suitable for these ISM bands xxxx and is capable of exchanging digitized raw I/Q samples with the baseband processing unit. This chip provides all the necessary blocks of the transceiver chain from the antenna to the digital baseband data including LNA/PA, downconversion/upconversion mixers, band-pass/low-pass filters, ADC/DAC, synthesizer and voltage-controlled oscillator. To exchange digitized I/Q baseband data between the baseband processing block, it uses 64~MHz double data-rate low voltage differential signaling (LVDS). The maximum sampling frequency for the I/Q data is 4~MHz which means that it can support modulations with maximum of 2~MHz bandwidth. Note that, most IoT communication protocols have low bandwidth of 500~KHz (e.g. LoRa, SigFox \cite{xxxx}). Moreover, the digital analog baseband front-end, ADC/DAC, has 13 bits which is even better than the analog front-end (AD93XX~\cite{xxxx}) used by USRP \cite{xxxx}. \textcolor{red}{the low bandwidth and sampling rate xxxx, mention it or not?}. Fig. \ref{fig:} compares power consumption this transceiver with other transceivers that are used in existing products. As can be seen, power consumption is more than \textcolor{red}{5 xxx} times less than the closest SDR platform. \textcolor{red}{Moreover, the price of this transceiver chip is less than 5 dollars which makes this design very low cost.} In summary, AT86RF215 satisfies all the requirements of the wide-spread cheap SDR for IoT applications.

%     \item {\bf Baseband-Processing Unit.}
%     The processing is composed of FPGA and MCU and is responsible for communication protocol implementation including modulation and demodulation and MAC layer. FPGA is responsible for doing modulationa and demodulation and MCU for MAC layer implementation. We selected FPGA by analyzing different IoT communication protocols’ receiver algorithm, FPGA computational resource needed to enable these algorithms and also computational resource needed to do localization xxxx. Moreover, it needs to support LVDS interface to be able to talk to the transceiver chip. We have used M2GL010T from IGLOO 2 series of Microsemi for our first prototype. We chose MSP430FR5969 from TI MSP430 series for MCU because of its power performance.
% \squishend

% MCU provides sensor interface, controls the analog front-end and power management unit (PMU). We provision microSD card to record raw I/Q samples and packet information for research projects that need data collection.


\subsection{Power Management Unit (PMU)}
%-power gating -> granular and composed multiple regulators - controllable
PMU is designed to meet the expectations of the IoT testbed which are being power-optimized and programmable. To this end, we used high-efficiency programmable switching regulators controlled by the MCU. Moreover, the system is divided to different power domains based on the voltage requirements of the blocks of the system each powered by a separate regulator. The granular power distribution design in combination with the programmable regulators enables power-gating functionality and saves power as a result. 

% As shown in Fig. \ref{xx}, the other block that we have used in our design is control unit which is implemented on a low power MSP430~\cite{xxxx} MCU. This unit serves multiple purposes. First, it talks to the radio to adjust its settings including synthesizer frequency, analog front-end gain, TX transmit power,sampling rate, filtering parameters and etc. depending on the application and communication protocol. Moreover, it talks to the power management unit to set voltage supply of different blocks and optimize them to minimize power consumption. In addition, it provides different communication interfaces (SPI, I2C and ...) to talk to different sensors that may need to be added.

\subsection{Storage Devices}
We provisioned two storage devices in \name design: - Flash memory - microSD card. Flash memory is used to save the programming data of the FPGA and also programming data of the MCU in the case of multi-boot design. microSD card is several Gigabyte memory used to record I/Q samples to be post-processed offline.


\subsection{Over-the-Air Update}
%-backbone radio - controlled by MCU -sometime during the day  -maybe explain the update strategy that we were thinking about  - talks to storage devices -Explain the whole update process (copying into memory, changing FPGA state and update)
One of the key features of our design is the OTA functionality. OTA is enabled by adding a second dedicated RF chip talking to the MCU as backbone. In \name design, after every preset time duration, \name's backbone radio talks to the IoT testbed central access point and checks if there is an update. If the answer is yes, first, it receives the compressed programming data of the FPGA and MCU itself and saves it in the flash memory. Then, MCU reads the data from flash memory, uncompresses and saves it in the flash memory again. Then, MCU activates the FPGA programming mode and FPGA code will be updated. As the last step, the MCU activates its boot loader and updates its own code if necessary. Note that during the update process, all the blocks except the backbone radio, MCU and flash memory are power-gated to save the energy.

\subsection{Sensor Interface}
To enable testing of different application scenarios, \name is utilized with common sensor interfaces like ADC, I2C and SPI. These interfaces are handled by the MCU.





==> system-5.tex <==
\section{System Design}\label{sec:system}
%   Explain in detail with a right flow
%   have a detailed block diagram
% 

\begin{figure}[t]
    \centering
	\includegraphics[width=0.8\linewidth]{./figs/foo.eps}
	\caption{\footnotesize{{\bf \name Hardware Design.}}}
	\label{fig:sdr_hardware}
\end{figure}

The \name system is designed to fulfill the vision of an SDR based IoT testbed. In particular, \name system has flexible PHY and MAC layer, is capable of updating over the air (OTA) and low power. In this section, we explain the design of the \name system and present design choices and considerations. As shown in fig.~\ref{fig:system}, the system is divided to six different functional blocks: i) PHY layer, ii) MAC layer and central control, iii) Power Management Unit (PMU), iv) storage devices, v) sensor interface, and vi) OTA update unit.

